Soft-Coherent Direct Multipath SLAM

Challenging indoor and urban environments with severe multipath propagation and obstructed line-of-sight degrade classical radio positioning. Multipath-based simultaneous localization and mapping (MP-SLAM) addresses this by building and exploiting propagation maps for robust localization. Emerging distributed multiple-input multiple-output (D-MIMO)/extremely large-scale MIMO (XL-MIMO) infrastructures provide large spatial apertures and high-resolution sensing, especially when phase coherence is maintained across base stations, subarrays, or distributed arrays. We propose a scalable Bayesian direct MP-SLAM method for coherent data fusion in D-MIMO/XL-MIMO systems that jointly infers the environment while performing robust, high-accuracy localization directly from raw radio signals. While commonly used zero-mean Type-II likelihood functions inherently lead to noncoherent processing across distributed arrays and thus to aperture loss, the proposed phase-preserving nonzero-mean Type-II likelihood shares a complex mean across distributed arrays. This enables coherent fusion and preserves the distributed aperture gain, while the variance captures noncoherent signal power. The method is combined with a surface model that enables map-feature fusion across the distributed infrastructure and supports near-field propagation and visibility effects. Bayesian inference is performed using belief propagation by means of the sum-product algorithm on a factor graph with particle-based messages. Parallelizing over particles and arrays, the GPU-accelerated implementation achieves millisecond-level runtimes even in large or distributed infrastructures. Simulation results show that the proposed method achieves performance gains over existing noncoherent methods and approaches the corresponding posterior CRLB, highlighting the potential of coherent processing for high-resolution sensing and localization.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}


==> figures/results/scenario-det-rays-background-N.tex <==

\addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.121431144606923	-0.305973920991947\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.112135907853868	-0.279815295362446\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.102810100110852	-0.253570636950484\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0934535703126276	-0.227239520628721\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.115390696823291	-0.313896027611391\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.106023713566285	-0.287576679154121\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0966257183123387	-0.261170193191485\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0871965567953521	-0.234676136266612\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.10926957279128	-0.32192394192328\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0998297489677462	-0.295441896485149\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.090358462584103	-0.268871587435112\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0808555560825777	-0.242212572767877\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.103066145376365	-0.330059797930529\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0935523620956501	-0.303413045049934\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0840066558587743	-0.276676880512702\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0744288657222368	-0.249850853538991\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0637884020032	-0.101769000151684\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06213096187395	-0.0861229589818673\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06047771430575	-0.0705164950986124\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.05882864341084	-0.0549494585231152\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0748989533857	-0.103085499152609\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0732359106856	-0.0875170587799596\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.07157705343489	-0.0719878001548322\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06992236585288	-0.0564975755476025\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08589736415929	-0.1043887105142\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08422891594527	-0.0888971053405379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08256464564711	-0.0734442922747162\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08090453759173	-0.0580301257915418\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09678532357923	-0.105678834397793\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09511166183643	-0.0902633100936512\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09344217007312	-0.0748861940403021\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09177683272422	-0.0595473428733455\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.275016741636257	0.318464099554947\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.281649014588661	0.340712214916542\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.288238233874936	0.362815905744093\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.294784817365672	0.384776573794313\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.263426192772478	0.332561041575443\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.27013404172854	0.354889186490687\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.276798100230945	0.377071567897901\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.283418795696495	0.399109608522073\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.251702970525635	0.346819346876548\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.258487694689603	0.369227902953099\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.265227874704238	0.391489338816052\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.271923947806723	0.413605098570382\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.239844783776866	0.361241802019117\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.246707712303528	0.383731148202568\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.253525325589217	0.406071999448667\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.260298070975166	0.428265821663957\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.3227256843839	3.1772743156161	0.22618755589019\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32576102520213	3.17423897479787	0.23510310099458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32881066571741	3.17118933428259	0.244060647838386\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.33187470721861	3.16812529278139	0.253060493931981\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31750185847795	3.18249814152205	0.230991883124655\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32051266836299	3.17948733163701	0.239882530638814\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32353760474344	3.17646239525656	0.248814892407969\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32657676727378	3.17342323272622	0.257789262702725\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31232011633952	3.18767988366048	0.235757506123176\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31530669147439	3.18469330852561	0.244623366872182\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31830722268891	3.18169277731109	0.253530657236472\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32132180803603	3.17867819196397	0.262479668293158\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.30717995146103	3.19282004853897	0.240484890718297\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31014258327976	3.18985741672024	0.249326075271772\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31311900349251	3.18688099650749	0.258208407609945\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31610930858271	3.18389069141729	0.267132175661891\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.991159848539033	0.265789947524383\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.987350755178758	0.280902581875283\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.983519624341664	0.296102650242015\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.979666264226472	0.311390913599003\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.99770580743776	0.273805047871219\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.993934436759458	0.288865559721062\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.990141355626273	0.304012769641958\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.986326376027868	0.319247428430406\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00418719150682	0.28174108054475\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00045298590247	0.296749759735325\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.996697390426655	0.311844410013976\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.992920220766769	0.32702577217777\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0106049515867	0.289599209787227\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00690736438431	0.304556345188937\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.003188701613	0.3195987335193\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.99944878256747	0.334727105750607\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.565174253005492	-0.219946772743362\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.561583398965443	-0.197491275200431\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.557993766058512	-0.175043414044675\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.554405353661905	-0.152603185381425\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.551447055534443	-0.222117578774727\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.547838493367619	-0.199536291477689\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.544231165208612	-0.176962726227206\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.540625070424547	-0.154396879062932\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.537565631927174	-0.224312773981479\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.533939189238341	-0.201604279721379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.530313993635908	-0.178903594616633\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.526690044476699	-0.156210714639732\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.523527368386541	-0.226532771707029\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.519882870311289	-0.203695629188974\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.51623963260921	-0.180866384417376\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.512597654626605	-0.158045033296036\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.912118731001735	4	-0.016708731386001\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.912576001584169	4	-0.00583533410247139\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.913032269580855	4	0.0050142227820611\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.913487538285504	4	0.0158400175884114\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.901581529845063	4	-0.0165021615844915\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.90204984285177	4	-0.00564109463688522\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.902517130203475	4	0.00519618542569555\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.90298339526593	4	0.0160097566614629\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.891067787574463	4	-0.0162960516676675\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.891547092760417	4	-0.00544728713152698\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.892025349383278	4	0.00537774385359263\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.892502560880158	4	0.0161791190844736\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.880577425937548	4	-0.0160904001014801\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.881067673310735	4	-0.00525391014707255\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.881556849372818	4	0.00555889941115834\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.882044957631581	4	0.0163481061097306\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48638224524632	3.01361775475368	-0.0269007603290558\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48725106831988	3.01274893168012	-0.0154941673743061\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48811859499174	3.01188140500826	-0.00410459460103307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48898482816137	3.01101517183863	0.00726799605698714\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47946882760321	3.02053117239679	-0.0257063717054005\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48033747843498	3.01966252156502	-0.0143702800433674\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48120484102663	3.01879515897337	-0.00305100020893773\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.4820709182418	3.0179290817582	0.00825150516898576\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47263934580998	3.02736065419002	-0.0245264841620204\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47350776458132	3.02649223541868	-0.0132600277718489\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47437490326335	3.02562509673665	-0.00201017865785913\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47524076468436	3.02475923531564	0.00922309987274139\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46589228049144	3.03410771950856	-0.0233608352058118\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46676040957962	3.03323959042038	-0.0121631639239768\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.4676272667155	3.0323727332845	-0.000981899077390547\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46849285469248	3.03150714530752	0.0101829953647518\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.787528431992443	-0.170473881302008\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.783826995472351	-0.15099594786531\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.780124066348989	-0.131510159957258\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.776419643719339	-0.112016512825924\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.794072405600304	-0.168256201303825\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.790396489233142	-0.148905221131802\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.786719100250862	-0.129546488730641\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.783040237768365	-0.110179999440959\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.800531349343121	-0.166067336982822\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.79688060454599	-0.146841665898882\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.79322840672333	-0.1276083428446\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.789574755007493	-0.10836736325075\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.806906909791271	-0.16390673033458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.803280995058272	-0.14480475589696\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.799653646501292	-0.125695227815348\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.796024863269679	-0.106578141608363\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.668017536654152	0.308394121583095\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.670277019654357	0.328850481456709\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.672542095904788	0.349357480144355\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.674812786199945	0.36991530591027\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.6534326670454	0.305501297516042\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.655685316523917	0.326056244797117\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.65794357022552	0.346662329421666\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.660207449089842	0.367319742459371\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.638701543091929	0.302579464750271\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.640947107823332	0.323233953068746\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.643198287232844	0.343940084656196\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.645455102404742	0.364698053443761\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.623821953791154	0.299628184746278\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.62606017597274	0.320383181616372\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.62830402274524	0.341190335223985\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.630553515336993	0.36204984241913\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04227938154491	4	0.239656183297002\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03976177254897	4	0.250054333129968\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03723765163295	4	0.26047937829135\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03470699349902	4	0.270931423265417\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03211014702548	4	0.23770920261751\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02958423893929	4	0.248084974596827\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02705180996657	4	0.258487532678155\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0245128348232	4	0.268916980722096\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02197964962768	4	0.235769638467478\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01944552394739	4	0.246123127488271\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01690486865836	4	0.256503294046329\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01435765849107	4	0.266910241383528\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0118876684334	4	0.233837448550379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00934540590608	4	0.244168748911575\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00679660528874	4	0.254526618901629\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0042412413273	4	0.264911161148586\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58660640495456	2.91339359504544	0.248675686375164\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58386720830482	2.91613279169517	0.260259659541907\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58112901607392	2.91887098392608	0.271839385054236\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57839182770948	2.92160817229052	0.283414865248042\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57940846507169	2.92059153492831	0.246088265093267\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57668961253085	2.92331038746915	0.257592217997309\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57397175002286	2.92602824997714	0.269091981894744\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57125487700705	2.92874512299295	0.280587559073209\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57230988290969	2.92769011709031	0.243536559625293\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56961107573759	2.93038892426241	0.254961590178205\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.5669132445189	2.9330867554811	0.266382489166026\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56421638872432	2.93578361127567	0.277799258829458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56530861532367	2.93469138467633	0.241019835528246\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56262956128918	2.93737043871082	0.252367019200635\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.55995146942656	2.94004853057344	0.263710127576012\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.55727433921756	2.94272566078244	0.275049162849424\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.646569565148188	0.310217457064253\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.653727408850739	0.33046557935495\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.660861022922039	0.350645160817288\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.667970530181842	0.370756548884028\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.651470344886514	0.305663228148336\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.65857147495637	0.325781932400888\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.665648729843089	0.345832994215716\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.672702229753112	0.36581675415803\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.656305100419357	0.30117035464152\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.663350390066484	0.321161278860841\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.670372151303177	0.341085441499938\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.677370501795982	0.360943176436209\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.661075157054671	0.296737604952891\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.668065459788268	0.316602356364934\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.675032573427637	0.336401209973997\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.681976613170287	0.35613449314357\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};


==> figures/results/scenario-det-rays-background.tex <==

\addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.121431144606923	-0.305973920991947\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.112135907853868	-0.279815295362446\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.102810100110852	-0.253570636950484\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0934535703126276	-0.227239520628721\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.115390696823291	-0.313896027611391\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.106023713566285	-0.287576679154121\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0966257183123387	-0.261170193191485\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0871965567953521	-0.234676136266612\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.10926957279128	-0.32192394192328\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0998297489677462	-0.295441896485149\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.090358462584103	-0.268871587435112\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0808555560825777	-0.242212572767877\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.103066145376365	-0.330059797930529\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0935523620956501	-0.303413045049934\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0840066558587743	-0.276676880512702\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0744288657222368	-0.249850853538991\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.537886583448956	4	-0.0126620261638558\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.53599994549364	4	-0.00216809897884307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.534118153288	4	0.00829887499868598\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.532241188186827	4	0.0187389994778027\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.526775827752169	4	-0.014823752471844\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.5248999015857	4	-0.00430700177994603\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523028802844864	4	0.00618268556970353\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521162512919582	4	0.0166454139082803\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.515622503264112	4	-0.0169937610315976\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.513757384821553	4	-0.0064540888109369\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.511897075163215	4	0.00405840925911061\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.510041555715506	4	0.0145438381368011\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.504426364873643	4	-0.0191720995323307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.502572150958734	4	-0.00860940713567449\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.500722726865196	4	0.00192599962292006\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.498878074057307	4	0.0124342263338147\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0637884020032	-0.101769000151684\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06213096187395	-0.0861229589818673\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06047771430575	-0.0705164950986124\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.05882864341084	-0.0549494585231152\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0748989533857	-0.103085499152609\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0732359106856	-0.0875170587799596\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.07157705343489	-0.0719878001548322\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06992236585288	-0.0564975755476025\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08589736415929	-0.1043887105142\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08422891594527	-0.0888971053405379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08256464564711	-0.0734442922747162\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08090453759173	-0.0580301257915418\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09678532357923	-0.105678834397793\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09511166183643	-0.0902633100936512\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09344217007312	-0.0748861940403021\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09177683272422	-0.0595473428733455\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.275016741636257	0.318464099554947\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.281649014588661	0.340712214916542\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.288238233874936	0.362815905744093\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.294784817365672	0.384776573794313\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.263426192772478	0.332561041575443\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.27013404172854	0.354889186490687\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.276798100230945	0.377071567897901\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.283418795696495	0.399109608522073\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.251702970525635	0.346819346876548\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.258487694689603	0.369227902953099\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.265227874704238	0.391489338816052\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.271923947806723	0.413605098570382\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.239844783776866	0.361241802019117\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.246707712303528	0.383731148202568\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.253525325589217	0.406071999448667\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.260298070975166	0.428265821663957\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.3227256843839	3.1772743156161	0.22618755589019\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32576102520213	3.17423897479787	0.23510310099458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32881066571741	3.17118933428259	0.244060647838386\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.33187470721861	3.16812529278139	0.253060493931981\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31750185847795	3.18249814152205	0.230991883124655\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32051266836299	3.17948733163701	0.239882530638814\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32353760474344	3.17646239525656	0.248814892407969\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32657676727378	3.17342323272622	0.257789262702725\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31232011633952	3.18767988366048	0.235757506123176\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31530669147439	3.18469330852561	0.244623366872182\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31830722268891	3.18169277731109	0.253530657236472\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32132180803603	3.17867819196397	0.262479668293158\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31311900349251	3.18688099650749	0.258208407609945\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31610930858271	3.18389069141729	0.267132175661891\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.991159848539033	0.265789947524383\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.987350755178758	0.280902581875283\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.983519624341664	0.296102650242015\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.979666264226472	0.311390913599003\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.99770580743776	0.273805047871219\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.993934436759458	0.288865559721062\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.990141355626273	0.304012769641958\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.986326376027868	0.319247428430406\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00418719150682	0.28174108054475\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00045298590247	0.296749759735325\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.996697390426655	0.311844410013976\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.992920220766769	0.32702577217777\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0106049515867	0.289599209787227\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00690736438431	0.304556345188937\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.003188701613	0.3195987335193\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.99944878256747	0.334727105750607\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.565174253005492	-0.219946772743362\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.561583398965443	-0.197491275200431\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.557993766058512	-0.175043414044675\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.554405353661905	-0.152603185381425\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.551447055534443	-0.222117578774727\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.547838493367619	-0.199536291477689\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.544231165208612	-0.176962726227206\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.540625070424547	-0.154396879062932\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.537565631927174	-0.224312773981479\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.533939189238341	-0.201604279721379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.530313993635908	-0.178903594616633\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.526690044476699	-0.156210714639732\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.523527368386541	-0.226532771707029\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.519882870311289	-0.203695629188974\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.51623963260921	-0.180866384417376\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.512597654626605	-0.158045033296036\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.912118731001735	4	-0.016708731386001\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.912576001584169	4	-0.00583533410247139\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.913032269580855	4	0.0050142227820611\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.913487538285504	4	0.0158400175884114\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.901581529845063	4	-0.0165021615844915\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.90204984285177	4	-0.00564109463688522\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.902517130203475	4	0.00519618542569555\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.90298339526593	4	0.0160097566614629\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.891067787574463	4	-0.0162960516676675\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.891547092760417	4	-0.00544728713152698\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.892025349383278	4	0.00537774385359263\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.892502560880158	4	0.0161791190844736\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.880577425937548	4	-0.0160904001014801\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.881067673310735	4	-0.00525391014707255\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.881556849372818	4	0.00555889941115834\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.882044957631581	4	0.0163481061097306\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48638224524632	3.01361775475368	-0.0269007603290558\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48725106831988	3.01274893168012	-0.0154941673743061\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48811859499174	3.01188140500826	-0.00410459460103307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48898482816137	3.01101517183863	0.00726799605698714\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47946882760321	3.02053117239679	-0.0257063717054005\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48033747843498	3.01966252156502	-0.0143702800433674\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48120484102663	3.01879515897337	-0.00305100020893773\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.4820709182418	3.0179290817582	0.00825150516898576\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47263934580998	3.02736065419002	-0.0245264841620204\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47350776458132	3.02649223541868	-0.0132600277718489\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47437490326335	3.02562509673665	-0.00201017865785913\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47524076468436	3.02475923531564	0.00922309987274139\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46589228049144	3.03410771950856	-0.0233608352058118\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46676040957962	3.03323959042038	-0.0121631639239768\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.4676272667155	3.0323727332845	-0.000981899077390547\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46849285469248	3.03150714530752	0.0101829953647518\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.787528431992443	-0.170473881302008\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.783826995472351	-0.15099594786531\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.780124066348989	-0.131510159957258\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.776419643719339	-0.112016512825924\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.794072405600304	-0.168256201303825\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.790396489233142	-0.148905221131802\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.786719100250862	-0.129546488730641\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.783040237768365	-0.110179999440959\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.800531349343121	-0.166067336982822\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.79688060454599	-0.146841665898882\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.79322840672333	-0.1276083428446\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.789574755007493	-0.10836736325075\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.806906909791271	-0.16390673033458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.803280995058272	-0.14480475589696\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.799653646501292	-0.125695227815348\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.796024863269679	-0.106578141608363\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.668017536654152	0.308394121583095\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.670277019654357	0.328850481456709\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.672542095904788	0.349357480144355\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.674812786199945	0.36991530591027\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.6534326670454	0.305501297516042\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.655685316523917	0.326056244797117\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.65794357022552	0.346662329421666\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.660207449089842	0.367319742459371\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.638701543091929	0.302579464750271\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.640947107823332	0.323233953068746\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.643198287232844	0.343940084656196\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.645455102404742	0.364698053443761\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.623821953791154	0.299628184746278\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.62606017597274	0.320383181616372\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.62830402274524	0.341190335223985\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.630553515336993	0.36204984241913\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04227938154491	4	0.239656183297002\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03976177254897	4	0.250054333129968\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03723765163295	4	0.26047937829135\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03470699349902	4	0.270931423265417\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03211014702548	4	0.23770920261751\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02958423893929	4	0.248084974596827\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02705180996657	4	0.258487532678155\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0245128348232	4	0.268916980722096\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02197964962768	4	0.235769638467478\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01944552394739	4	0.246123127488271\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01690486865836	4	0.256503294046329\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01435765849107	4	0.266910241383528\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0118876684334	4	0.233837448550379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00934540590608	4	0.244168748911575\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00679660528874	4	0.254526618901629\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0042412413273	4	0.264911161148586\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58660640495456	2.91339359504544	0.248675686375164\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58386720830482	2.91613279169517	0.260259659541907\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58112901607392	2.91887098392608	0.271839385054236\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57839182770948	2.92160817229052	0.283414865248042\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57940846507169	2.92059153492831	0.246088265093267\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57668961253085	2.92331038746915	0.257592217997309\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57397175002286	2.92602824997714	0.269091981894744\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57125487700705	2.92874512299295	0.280587559073209\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57230988290969	2.92769011709031	0.243536559625293\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56961107573759	2.93038892426241	0.254961590178205\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.5669132445189	2.9330867554811	0.266382489166026\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56421638872432	2.93578361127567	0.277799258829458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56530861532367	2.93469138467633	0.241019835528246\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56262956128918	2.93737043871082	0.252367019200635\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.55995146942656	2.94004853057344	0.263710127576012\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.55727433921756	2.94272566078244	0.275049162849424\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.646569565148188	0.310217457064253\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.653727408850739	0.33046557935495\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.660861022922039	0.350645160817288\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.667970530181842	0.370756548884028\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.651470344886514	0.305663228148336\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.65857147495637	0.325781932400888\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.665648729843089	0.345832994215716\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.672702229753112	0.36581675415803\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.656305100419357	0.30117035464152\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.663350390066484	0.321161278860841\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.670372151303177	0.341085441499938\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.677370501795982	0.360943176436209\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.661075157054671	0.296737604952891\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.668065459788268	0.316602356364934\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.675032573427637	0.336401209973997\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.681976613170287	0.35613449314357\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
























 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
0.912118731001735	4	-0.016708731386001\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
0.912576001584169	4	-0.00583533410247139\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
0.913032269580855	4	0.0050142227820611\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
0.913487538285504	4	0.0158400175884114\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
0.901581529845063	4	-0.0165021615844915\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
0.90204984285177	4	-0.00564109463688522\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
0.902517130203475	4	0.00519618542569555\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
0.90298339526593	4	0.0160097566614629\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
0.891067787574463	4	-0.0162960516676675\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
0.891547092760417	4	-0.00544728713152698\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
0.892025349383278	4	0.00537774385359263\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
0.892502560880158	4	0.0161791190844736\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
0.880577425937548	4	-0.0160904001014801\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
0.881067673310735	4	-0.00525391014707255\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
0.881556849372818	4	0.00555889941115834\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
0.882044957631581	4	0.0163481061097306\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
2.48638224524632	3.01361775475368	-0.0269007603290558\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
2.48725106831988	3.01274893168012	-0.0154941673743061\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
2.48811859499174	3.01188140500826	-0.00410459460103307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
2.48898482816137	3.01101517183863	0.00726799605698714\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
2.47946882760321	3.02053117239679	-0.0257063717054005\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
2.48033747843498	3.01966252156502	-0.0143702800433674\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
2.48120484102663	3.01879515897337	-0.00305100020893773\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
2.4820709182418	3.0179290817582	0.00825150516898576\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
2.47263934580998	3.02736065419002	-0.0245264841620204\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
2.47350776458132	3.02649223541868	-0.0132600277718489\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
2.47437490326335	3.02562509673665	-0.00201017865785913\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
2.47524076468436	3.02475923531564	0.00922309987274139\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
2.46589228049144	3.03410771950856	-0.0233608352058118\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
2.46676040957962	3.03323959042038	-0.0121631639239768\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
2.4676272667155	3.0323727332845	-0.000981899077390547\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
2.46849285469248	3.03150714530752	0.0101829953647518\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
4	0.787528431992443	-0.170473881302008\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
4	0.783826995472351	-0.15099594786531\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
4	0.780124066348989	-0.131510159957258\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
4	0.776419643719339	-0.112016512825924\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
4	0.794072405600304	-0.168256201303825\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
4	0.790396489233142	-0.148905221131802\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
4	0.786719100250862	-0.129546488730641\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
4	0.783040237768365	-0.110179999440959\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
4	0.800531349343121	-0.166067336982822\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
4	0.79688060454599	-0.146841665898882\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
4	0.79322840672333	-0.1276083428446\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
4	0.789574755007493	-0.10836736325075\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
4	0.806906909791271	-0.16390673033458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
4	0.803280995058272	-0.14480475589696\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
4	0.799653646501292	-0.125695227815348\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
4	0.796024863269679	-0.106578141608363\\
};





 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
1.04227938154491	4	0.239656183297002\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
1.03976177254897	4	0.250054333129968\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
1.03723765163295	4	0.26047937829135\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
1.03470699349902	4	0.270931423265417\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
1.03211014702548	4	0.23770920261751\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
1.02958423893929	4	0.248084974596827\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
1.02705180996657	4	0.258487532678155\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
1.0245128348232	4	0.268916980722096\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
1.02197964962768	4	0.235769638467478\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
1.01944552394739	4	0.246123127488271\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
1.01690486865836	4	0.256503294046329\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
1.01435765849107	4	0.266910241383528\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
1.0118876684334	4	0.233837448550379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
1.00934540590608	4	0.244168748911575\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
1.00679660528874	4	0.254526618901629\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
1.0042412413273	4	0.264911161148586\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
2.58660640495456	2.91339359504544	0.248675686375164\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
2.58386720830482	2.91613279169517	0.260259659541907\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
2.58112901607392	2.91887098392608	0.271839385054236\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
2.57839182770948	2.92160817229052	0.283414865248042\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
2.57940846507169	2.92059153492831	0.246088265093267\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
2.57668961253085	2.92331038746915	0.257592217997309\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
2.57397175002286	2.92602824997714	0.269091981894744\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
2.57125487700705	2.92874512299295	0.280587559073209\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
2.57230988290969	2.92769011709031	0.243536559625293\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
2.56961107573759	2.93038892426241	0.254961590178205\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
2.5669132445189	2.9330867554811	0.266382489166026\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
2.56421638872432	2.93578361127567	0.277799258829458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
2.56530861532367	2.93469138467633	0.241019835528246\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
2.56262956128918	2.93737043871082	0.252367019200635\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
2.55995146942656	2.94004853057344	0.263710127576012\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
2.55727433921756	2.94272566078244	0.275049162849424\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
4	0.646569565148188	0.310217457064253\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
4	0.653727408850739	0.33046557935495\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
4	0.660861022922039	0.350645160817288\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
4	0.667970530181842	0.370756548884028\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
4	0.651470344886514	0.305663228148336\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
4	0.65857147495637	0.325781932400888\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
4	0.665648729843089	0.345832994215716\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
4	0.672702229753112	0.36581675415803\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
4	0.656305100419357	0.30117035464152\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
4	0.663350390066484	0.321161278860841\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
4	0.670372151303177	0.341085441499938\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
4	0.677370501795982	0.360943176436209\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
4	0.661075157054671	0.296737604952891\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
4	0.668065459788268	0.316602356364934\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
4	0.675032573427637	0.336401209973997\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
4	0.681976613170287	0.35613449314357\\
};

==> figures/results/scenario-det-rays-foreground-N.tex <==

\addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
-3	0.121431144606923	-0.305973920991947\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
-3	0.112135907853868	-0.279815295362446\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
-3	0.102810100110852	-0.253570636950484\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
-3	0.0934535703126276	-0.227239520628721\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
-3	0.115390696823291	-0.313896027611391\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
-3	0.106023713566285	-0.287576679154121\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
-3	0.0966257183123387	-0.261170193191485\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
-3	0.0871965567953521	-0.234676136266612\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
-3	0.10926957279128	-0.32192394192328\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
-3	0.0998297489677462	-0.295441896485149\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
-3	0.090358462584103	-0.268871587435112\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
-3	0.0808555560825777	-0.242212572767877\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
-3	0.103066145376365	-0.330059797930529\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
-3	0.0935523620956501	-0.303413045049934\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
-3	0.0840066558587743	-0.276676880512702\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
-3	0.0744288657222368	-0.249850853538991\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
4	1.0637884020032	-0.101769000151684\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
4	1.06213096187395	-0.0861229589818673\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
4	1.06047771430575	-0.0705164950986124\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
4	1.05882864341084	-0.0549494585231152\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
4	1.0748989533857	-0.103085499152609\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
4	1.0732359106856	-0.0875170587799596\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
4	1.07157705343489	-0.0719878001548322\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
4	1.06992236585288	-0.0564975755476025\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
4	1.08589736415929	-0.1043887105142\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
4	1.08422891594527	-0.0888971053405379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
4	1.08256464564711	-0.0734442922747162\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
4	1.08090453759173	-0.0580301257915418\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
4	1.09678532357923	-0.105678834397793\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
4	1.09511166183643	-0.0902633100936512\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
4	1.09344217007312	-0.0748861940403021\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
4	1.09177683272422	-0.0595473428733455\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
-3	0.275016741636257	0.318464099554947\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
-3	0.281649014588661	0.340712214916542\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
-3	0.288238233874936	0.362815905744093\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
-3	0.294784817365672	0.384776573794313\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
-3	0.263426192772478	0.332561041575443\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
-3	0.27013404172854	0.354889186490687\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
-3	0.276798100230945	0.377071567897901\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
-3	0.283418795696495	0.399109608522073\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
-3	0.251702970525635	0.346819346876548\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
-3	0.258487694689603	0.369227902953099\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
-3	0.265227874704238	0.391489338816052\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
-3	0.271923947806723	0.413605098570382\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
-3	0.239844783776866	0.361241802019117\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
-3	0.246707712303528	0.383731148202568\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
-3	0.253525325589217	0.406071999448667\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
-3	0.260298070975166	0.428265821663957\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
2.3227256843839	3.1772743156161	0.22618755589019\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
2.32576102520213	3.17423897479787	0.23510310099458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
2.32881066571741	3.17118933428259	0.244060647838386\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
2.33187470721861	3.16812529278139	0.253060493931981\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
2.31750185847795	3.18249814152205	0.230991883124655\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
2.32051266836299	3.17948733163701	0.239882530638814\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
2.32353760474344	3.17646239525656	0.248814892407969\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
2.32657676727378	3.17342323272622	0.257789262702725\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
2.31232011633952	3.18767988366048	0.235757506123176\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
2.31530669147439	3.18469330852561	0.244623366872182\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
2.31830722268891	3.18169277731109	0.253530657236472\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
2.32132180803603	3.17867819196397	0.262479668293158\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
2.30717995146103	3.19282004853897	0.240484890718297\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
2.31014258327976	3.18985741672024	0.249326075271772\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
2.31311900349251	3.18688099650749	0.258208407609945\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
2.31610930858271	3.18389069141729	0.267132175661891\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
4	0.991159848539033	0.265789947524383\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
4	0.987350755178758	0.280902581875283\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
4	0.983519624341664	0.296102650242015\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
4	0.979666264226472	0.311390913599003\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
4	0.99770580743776	0.273805047871219\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
4	0.993934436759458	0.288865559721062\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
4	0.990141355626273	0.304012769641958\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
4	0.986326376027868	0.319247428430406\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
4	1.00418719150682	0.28174108054475\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
4	1.00045298590247	0.296749759735325\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
4	0.996697390426655	0.311844410013976\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
4	0.992920220766769	0.32702577217777\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
4	1.0106049515867	0.289599209787227\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
4	1.00690736438431	0.304556345188937\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
4	1.003188701613	0.3195987335193\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
4	0.99944878256747	0.334727105750607\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
-3	0.565174253005492	-0.219946772743362\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
-3	0.561583398965443	-0.197491275200431\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
-3	0.557993766058512	-0.175043414044675\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
-3	0.554405353661905	-0.152603185381425\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
-3	0.551447055534443	-0.222117578774727\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
-3	0.547838493367619	-0.199536291477689\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
-3	0.544231165208612	-0.176962726227206\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
-3	0.540625070424547	-0.154396879062932\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
-3	0.537565631927174	-0.224312773981479\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
-3	0.533939189238341	-0.201604279721379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
-3	0.530313993635908	-0.178903594616633\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
-3	0.526690044476699	-0.156210714639732\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
-3	0.523527368386541	-0.226532771707029\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
-3	0.519882870311289	-0.203695629188974\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
-3	0.51623963260921	-0.180866384417376\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
-3	0.512597654626605	-0.158045033296036\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
0.912118731001735	4	-0.016708731386001\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
0.912576001584169	4	-0.00583533410247139\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
0.913032269580855	4	0.0050142227820611\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
0.913487538285504	4	0.0158400175884114\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
0.901581529845063	4	-0.0165021615844915\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
0.90204984285177	4	-0.00564109463688522\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
0.902517130203475	4	0.00519618542569555\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
0.90298339526593	4	0.0160097566614629\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
0.891067787574463	4	-0.0162960516676675\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
0.891547092760417	4	-0.00544728713152698\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
0.892025349383278	4	0.00537774385359263\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
0.892502560880158	4	0.0161791190844736\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
0.880577425937548	4	-0.0160904001014801\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
0.881067673310735	4	-0.00525391014707255\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
0.881556849372818	4	0.00555889941115834\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
0.882044957631581	4	0.0163481061097306\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
2.48638224524632	3.01361775475368	-0.0269007603290558\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
2.48725106831988	3.01274893168012	-0.0154941673743061\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
2.48811859499174	3.01188140500826	-0.00410459460103307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
2.48898482816137	3.01101517183863	0.00726799605698714\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
2.47946882760321	3.02053117239679	-0.0257063717054005\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
2.48033747843498	3.01966252156502	-0.0143702800433674\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
2.48120484102663	3.01879515897337	-0.00305100020893773\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
2.4820709182418	3.0179290817582	0.00825150516898576\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
2.47263934580998	3.02736065419002	-0.0245264841620204\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
2.47350776458132	3.02649223541868	-0.0132600277718489\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
2.47437490326335	3.02562509673665	-0.00201017865785913\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
2.47524076468436	3.02475923531564	0.00922309987274139\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
2.46589228049144	3.03410771950856	-0.0233608352058118\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
2.46676040957962	3.03323959042038	-0.0121631639239768\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
2.4676272667155	3.0323727332845	-0.000981899077390547\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
2.46849285469248	3.03150714530752	0.0101829953647518\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
4	0.787528431992443	-0.170473881302008\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
4	0.783826995472351	-0.15099594786531\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
4	0.780124066348989	-0.131510159957258\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
4	0.776419643719339	-0.112016512825924\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
4	0.794072405600304	-0.168256201303825\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
4	0.790396489233142	-0.148905221131802\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
4	0.786719100250862	-0.129546488730641\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
4	0.783040237768365	-0.110179999440959\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
4	0.800531349343121	-0.166067336982822\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
4	0.79688060454599	-0.146841665898882\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
4	0.79322840672333	-0.1276083428446\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
4	0.789574755007493	-0.10836736325075\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
4	0.806906909791271	-0.16390673033458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
4	0.803280995058272	-0.14480475589696\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
4	0.799653646501292	-0.125695227815348\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
4	0.796024863269679	-0.106578141608363\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
-3	0.668017536654152	0.308394121583095\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
-3	0.670277019654357	0.328850481456709\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
-3	0.672542095904788	0.349357480144355\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
-3	0.674812786199945	0.36991530591027\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
-3	0.6534326670454	0.305501297516042\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
-3	0.655685316523917	0.326056244797117\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
-3	0.65794357022552	0.346662329421666\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
-3	0.660207449089842	0.367319742459371\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
-3	0.638701543091929	0.302579464750271\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
-3	0.640947107823332	0.323233953068746\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
-3	0.643198287232844	0.343940084656196\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
-3	0.645455102404742	0.364698053443761\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
-3	0.623821953791154	0.299628184746278\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
-3	0.62606017597274	0.320383181616372\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
-3	0.62830402274524	0.341190335223985\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
-3	0.630553515336993	0.36204984241913\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
1.04227938154491	4	0.239656183297002\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
1.03976177254897	4	0.250054333129968\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
1.03723765163295	4	0.26047937829135\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
1.03470699349902	4	0.270931423265417\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
1.03211014702548	4	0.23770920261751\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
1.02958423893929	4	0.248084974596827\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
1.02705180996657	4	0.258487532678155\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
1.0245128348232	4	0.268916980722096\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
1.02197964962768	4	0.235769638467478\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
1.01944552394739	4	0.246123127488271\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
1.01690486865836	4	0.256503294046329\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
1.01435765849107	4	0.266910241383528\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
1.0118876684334	4	0.233837448550379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
1.00934540590608	4	0.244168748911575\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
1.00679660528874	4	0.254526618901629\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
1.0042412413273	4	0.264911161148586\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
2.58660640495456	2.91339359504544	0.248675686375164\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
2.58386720830482	2.91613279169517	0.260259659541907\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
2.58112901607392	2.91887098392608	0.271839385054236\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
2.57839182770948	2.92160817229052	0.283414865248042\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
2.57940846507169	2.92059153492831	0.246088265093267\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
2.57668961253085	2.92331038746915	0.257592217997309\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
2.57397175002286	2.92602824997714	0.269091981894744\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
2.57125487700705	2.92874512299295	0.280587559073209\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
2.57230988290969	2.92769011709031	0.243536559625293\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
2.56961107573759	2.93038892426241	0.254961590178205\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
2.5669132445189	2.9330867554811	0.266382489166026\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
2.56421638872432	2.93578361127567	0.277799258829458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
2.56530861532367	2.93469138467633	0.241019835528246\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
2.56262956128918	2.93737043871082	0.252367019200635\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
2.55995146942656	2.94004853057344	0.263710127576012\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
2.55727433921756	2.94272566078244	0.275049162849424\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
4	0.646569565148188	0.310217457064253\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
4	0.653727408850739	0.33046557935495\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
4	0.660861022922039	0.350645160817288\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
4	0.667970530181842	0.370756548884028\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
4	0.651470344886514	0.305663228148336\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
4	0.65857147495637	0.325781932400888\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
4	0.665648729843089	0.345832994215716\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
4	0.672702229753112	0.36581675415803\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
4	0.656305100419357	0.30117035464152\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
4	0.663350390066484	0.321161278860841\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
4	0.670372151303177	0.341085441499938\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
4	0.677370501795982	0.360943176436209\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
4	0.661075157054671	0.296737604952891\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
4	0.668065459788268	0.316602356364934\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
4	0.675032573427637	0.336401209973997\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
4	0.681976613170287	0.35613449314357\\
};


==> figures/results/scenario-det-rays-foreground.tex <==

\addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
-3	0.121431144606923	-0.305973920991947\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
-3	0.112135907853868	-0.279815295362446\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
-3	0.102810100110852	-0.253570636950484\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
-3	0.0934535703126276	-0.227239520628721\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
-3	0.115390696823291	-0.313896027611391\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
-3	0.106023713566285	-0.287576679154121\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
-3	0.0966257183123387	-0.261170193191485\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
-3	0.0871965567953521	-0.234676136266612\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
-3	0.10926957279128	-0.32192394192328\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
-3	0.0998297489677462	-0.295441896485149\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
-3	0.090358462584103	-0.268871587435112\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
-3	0.0808555560825777	-0.242212572767877\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
-3	0.103066145376365	-0.330059797930529\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
-3	0.0935523620956501	-0.303413045049934\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
-3	0.0840066558587743	-0.276676880512702\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
-3	0.0744288657222368	-0.249850853538991\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
0.537886583448956	4	-0.0126620261638558\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
0.53599994549364	4	-0.00216809897884307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
0.534118153288	4	0.00829887499868598\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
0.532241188186827	4	0.0187389994778027\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
0.526775827752169	4	-0.014823752471844\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
0.5248999015857	4	-0.00430700177994603\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
0.523028802844864	4	0.00618268556970353\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
0.521162512919582	4	0.0166454139082803\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
0.515622503264112	4	-0.0169937610315976\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
0.513757384821553	4	-0.0064540888109369\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
0.511897075163215	4	0.00405840925911061\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
0.510041555715506	4	0.0145438381368011\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
0.504426364873643	4	-0.0191720995323307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
0.502572150958734	4	-0.00860940713567449\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
0.500722726865196	4	0.00192599962292006\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
0.498878074057307	4	0.0124342263338147\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
4	1.0637884020032	-0.101769000151684\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
4	1.06213096187395	-0.0861229589818673\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
4	1.06047771430575	-0.0705164950986124\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
4	1.05882864341084	-0.0549494585231152\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
4	1.0748989533857	-0.103085499152609\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
4	1.0732359106856	-0.0875170587799596\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
4	1.07157705343489	-0.0719878001548322\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
4	1.06992236585288	-0.0564975755476025\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
4	1.08589736415929	-0.1043887105142\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
4	1.08422891594527	-0.0888971053405379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
4	1.08256464564711	-0.0734442922747162\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
4	1.08090453759173	-0.0580301257915418\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
4	1.09678532357923	-0.105678834397793\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
4	1.09511166183643	-0.0902633100936512\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
4	1.09344217007312	-0.0748861940403021\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
4	1.09177683272422	-0.0595473428733455\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
-3	0.275016741636257	0.318464099554947\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
-3	0.281649014588661	0.340712214916542\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
-3	0.288238233874936	0.362815905744093\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
-3	0.294784817365672	0.384776573794313\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
-3	0.263426192772478	0.332561041575443\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
-3	0.27013404172854	0.354889186490687\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
-3	0.276798100230945	0.377071567897901\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
-3	0.283418795696495	0.399109608522073\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
-3	0.251702970525635	0.346819346876548\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
-3	0.258487694689603	0.369227902953099\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
-3	0.265227874704238	0.391489338816052\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
-3	0.271923947806723	0.413605098570382\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
-3	0.239844783776866	0.361241802019117\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
-3	0.246707712303528	0.383731148202568\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
-3	0.253525325589217	0.406071999448667\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
-3	0.260298070975166	0.428265821663957\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
2.3227256843839	3.1772743156161	0.22618755589019\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
2.32576102520213	3.17423897479787	0.23510310099458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
2.32881066571741	3.17118933428259	0.244060647838386\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
2.33187470721861	3.16812529278139	0.253060493931981\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
2.31750185847795	3.18249814152205	0.230991883124655\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
2.32051266836299	3.17948733163701	0.239882530638814\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
2.32353760474344	3.17646239525656	0.248814892407969\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
2.32657676727378	3.17342323272622	0.257789262702725\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
2.31232011633952	3.18767988366048	0.235757506123176\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
2.31530669147439	3.18469330852561	0.244623366872182\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
2.31830722268891	3.18169277731109	0.253530657236472\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
2.32132180803603	3.17867819196397	0.262479668293158\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
2.31311900349251	3.18688099650749	0.258208407609945\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
2.31610930858271	3.18389069141729	0.267132175661891\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
4	0.991159848539033	0.265789947524383\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
4	0.987350755178758	0.280902581875283\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
4	0.983519624341664	0.296102650242015\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
4	0.979666264226472	0.311390913599003\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
4	0.99770580743776	0.273805047871219\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
4	0.993934436759458	0.288865559721062\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
4	0.990141355626273	0.304012769641958\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
4	0.986326376027868	0.319247428430406\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
4	1.00418719150682	0.28174108054475\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
4	1.00045298590247	0.296749759735325\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
4	0.996697390426655	0.311844410013976\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
4	0.992920220766769	0.32702577217777\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
4	1.0106049515867	0.289599209787227\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
4	1.00690736438431	0.304556345188937\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
4	1.003188701613	0.3195987335193\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
4	0.99944878256747	0.334727105750607\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
-3	0.565174253005492	-0.219946772743362\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
-3	0.561583398965443	-0.197491275200431\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
-3	0.557993766058512	-0.175043414044675\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
-3	0.554405353661905	-0.152603185381425\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
-3	0.551447055534443	-0.222117578774727\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
-3	0.547838493367619	-0.199536291477689\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
-3	0.544231165208612	-0.176962726227206\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
-3	0.540625070424547	-0.154396879062932\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
-3	0.537565631927174	-0.224312773981479\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
-3	0.533939189238341	-0.201604279721379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
-3	0.530313993635908	-0.178903594616633\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
-3	0.526690044476699	-0.156210714639732\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
-3	0.523527368386541	-0.226532771707029\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
-3	0.519882870311289	-0.203695629188974\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
-3	0.51623963260921	-0.180866384417376\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
-3	0.512597654626605	-0.158045033296036\\
};

 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
-3	0.668017536654152	0.308394121583095\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
-3	0.670277019654357	0.328850481456709\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
-3	0.672542095904788	0.349357480144355\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
-3	0.674812786199945	0.36991530591027\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
-3	0.6534326670454	0.305501297516042\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
-3	0.655685316523917	0.326056244797117\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
-3	0.65794357022552	0.346662329421666\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
-3	0.660207449089842	0.367319742459371\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
-3	0.638701543091929	0.302579464750271\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
-3	0.640947107823332	0.323233953068746\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
-3	0.643198287232844	0.343940084656196\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
-3	0.645455102404742	0.364698053443761\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
-3	0.623821953791154	0.299628184746278\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
-3	0.62606017597274	0.320383181616372\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
-3	0.62830402274524	0.341190335223985\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
-3	0.630553515336993	0.36204984241913\\
};



==> figures/results/scenario-det-traj-ground.tex <==

\addplot3 [dashed,color=black,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.6	1	-1\\
-1.61492701767606	1.02367352612917	-1\\
-1.62956806850822	1.04741738951433	-1\\
-1.64390795843697	1.07122488683752	-1\\
-1.657931288255	1.09508913824079	-1\\
-1.67162246539232	1.11900309002269	-1\\
-1.68496571655508	1.14295951771515	-1\\
-1.69794510123443	1.16695102955143	-1\\
-1.71054452610028	1.19097007033569	-1\\
-1.72274776029341	1.21500892572435	-1\\
-1.7345384516276	1.23905972692839	-1\\
-1.74590014371191	1.26311445584568	-1\\
-1.75681629400107	1.28716495063131	-1\\
-1.76727029278012	1.31120291171342	-1\\
-1.77724548308712	1.33521990826106	-1\\
-1.78672518157534	1.35920738510974	-1\\
-1.79569270031421	1.3831566701496	-1\\
-1.80413136952528	1.4070589821797	-1\\
-1.81202456124688	1.43090543923133	-1\\
-1.81935571391849	1.45468706736173	-1\\
-1.82610835787233	1.47839480991855	-1\\
-1.83226614171705	1.50201953727407	-1\\
-1.83781285959478	1.52555205702697	-1\\
-1.84273247928951	1.54898312466778	-1\\
-1.8470091711614	1.57230345470285	-1\\
-1.85062733787781	1.59550373223033	-1\\
-1.85357164490822	1.61857462495954	-1\\
-1.85582705174657	1.64150679566409	-1\\
-1.85737884382043	1.66429091505706	-1\\
-1.85821266504271	1.68691767507487	-1\\
-1.85831455095748	1.70937780255479	-1\\
-1.85767096242771	1.73166207328932	-1\\
-1.85626881980827	1.75376132643855	-1\\
-1.85409553754411	1.77566647928017	-1\\
-1.85113905912881	1.79736854227458	-1\\
-1.84738789235537	1.81885863442087	-1\\
-1.8428311447867	1.84012799887767	-1\\
-1.83745855936947	1.8611680188207	-1\\
-1.83126055011146	1.88197023350729	-1\\
-1.82422823773844	1.90252635451629	-1\\
-1.81635348524341	1.92282828212979	-1\\
-1.80762893323742	1.94286812182162	-1\\
-1.79804803500809	1.96263820081579	-1\\
-1.78760509118871	1.98213108467621	-1\\
-1.77629528393836	2.00133959388799	-1\\
-1.76411471053047	2.02025682038854	-1\\
-1.75106041624528	2.03887614400575	-1\\
-1.73713042645954	2.05719124875916	-1\\
-1.72232377782498	2.07519613897878	-1\\
-1.70664054842597	2.09288515519529	-1\\
-1.69008188680547	2.11025298975438	-1\\
-1.67265003974802	2.12729470210736	-1\\
-1.65434837870809	2.14400573372947	-1\\
-1.63518142477238	2.16038192261691	-1\\
-1.61515487204521	2.17641951731331	-1\\
-1.59427560934735	2.19211519041652	-1\\
-1.57255174011986	2.20746605151621	-1\\
-1.54999260042676	2.22246965951371	-1\\
-1.52660877495285	2.23712403427541	-1\\
-1.50241211089556	2.25142766757216	-1\\
-1.47741572965375	2.26537953325792	-1\\
-1.45163403621978	2.2789790966418	-1\\
-1.42508272618601	2.29222632300941	-1\\
-1.39777879028168	2.30512168525059	-1\\
-1.3697405163614	2.31766617055255	-1\\
-1.34098748877277	2.3298612861194	-1\\
-1.31154058503666	2.34170906388134	-1\\
-1.28142196978071	2.35321206415888	-1\\
-1.25065508587391	2.36437337825049	-1\\
-1.2192646427176	2.37519662991453	-1\\
-1.18727660165669	2.38568597571944	-1\\
-1.15471815848291	2.39584610423936	-1\\
-1.12161772301113	2.40568223407566	-1\\
-1.08800489571855	2.4152001106883	-1\\
-1.05391044144608	2.42440600202462	-1\\
-1.01936626017099	2.43330669293703	-1\\
-0.984405354869354	2.44190947838472	-1\\
-0.949061796497066	2.45022215541877	-1\\
-0.913370686128259	2.45825301395389	-1\\
-0.877368114299888	2.46601082633426	-1\\
-0.841091117621584	2.47350483570512	-1\\
-0.804577632719929	2.480744743206	-1\\
-0.767866447596321	2.48774069400549	-1\\
-0.730997150487555	2.49450326220197	-1\\
-0.694010047301835	2.50104341262928	-1\\
-0.656935457035713	2.50736441633996	-1\\
-0.619777520270327	2.5134496099399	-1\\
-0.582536318257329	2.51927917865116	-1\\
-0.545211899255917	2.52483323324306	-1\\
-0.507804284604308	2.53009184174375	-1\\
-0.470313475000259	2.5350350616835	-1\\
-0.432739456970332	2.53964297279017	-1\\
-0.395082209506679	2.54389571005412	-1\\
-0.357341710849184	2.54777349707817	-1\\
-0.319517945390002	2.5512566796259	-1\\
-0.281610910676834	2.55432575928014	-1\\
-0.243620624490687	2.55696142712238	-1\\
-0.205547131973324	2.55914459734267	-1\\
-0.167390512779263	2.56085644068927	-1\\
-0.129150888226862	2.56207841766708	-1\\
-0.0908284284229049	2.56279231139396	-1\\
-0.0524233593349995	2.56298026002488	-1\\
-0.0139359697862137	2.56262478865443	-1\\
0.0246333816535292	2.56170884060986	-1\\
0.0632842599043112	2.56021580804812	-1\\
0.102016146766199	2.55812956177286	-1\\
0.140828434486415	2.55543448018915	-1\\
0.179720419527332	2.55211547731679	-1\\
0.218691296558149	2.54815802978598	-1\\
0.257740152692138	2.54354820274227	-1\\
0.296865961990646	2.53827267459164	-1\\
0.336067580253821	2.53231876052004	-1\\
0.375343740116939	2.52567443472627	-1\\
0.414693046470169	2.51832835131109	-1\\
0.454113972218082	2.51026986377024	-1\\
0.493604854394156	2.5014890430437	-1\\
0.533158773651777	2.49197973990717	-1\\
0.57273540668769	2.48175635265393	-1\\
0.61228163765447	2.47084157024566	-1\\
0.651745186265494	2.45925827084859	-1\\
0.691074717001968	2.44702946597036	-1\\
0.730219908350317	2.43417826701284	-1\\
0.769131518876106	2.42072785232418	-1\\
0.807761450011153	2.40670143481929	-1\\
0.846062805443338	2.3921222302348	-1\\
0.883989947011599	2.37701342608126	-1\\
0.921498547021819	2.36139815135147	-1\\
0.958545636912577	2.34529944704013	-1\\
0.995089652212923	2.32874023752638	-1\\
1.03109047374758	2.31174330286659	-1\\
1.06650946505803	2.2943312520407	-1\\
1.10130950602072	2.27652649719175	-1\\
1.13545502265651	2.25835122889351	-1\\
1.16891201313757	2.23982739247768	-1\\
1.20164807001019	2.22097666544736	-1\\
1.23363239866342	2.20182043600001	-1\\
1.26483583208486	2.18237978267863	-1\\
1.29523084195547	2.16267545516612	-1\\
1.32479154614572	2.14272785623386	-1\\
1.35349371268491	2.12255702485175	-1\\
1.38131476028487	2.10218262046302	-1\\
1.40823375550753	2.08162390842395	-1\\
1.43423140667408	2.06089974660476	-1\\
1.45929005462075	2.0400285731448	-1\\
1.48339366041264	2.019028395352	-1\\
1.50652779013353	1.99791677973342	-1\\
1.52867959687476	1.976710843141	-1\\
1.54983780005108	1.9554272450138	-1\\
1.56999266217555	1.93408218069554	-1\\
1.58913596322893	1.91269137580401	-1\\
1.60726097276223	1.89127008162656	-1\\
1.62436241987267	1.8698330715141	-1\\
1.64043646119571	1.84839463824412	-1\\
1.65548064705622	1.82696859232169	-1\\
1.6694938859228	1.80556826118582	-1\\
1.68247640730885	1.78420648928759	-1\\
1.69442972326371	1.76289563900515	-1\\
1.70535658859587	1.74164759235964	-1\\
1.71526095996887	1.72047375349588	-1\\
1.72414795400839	1.69938505189043	-1\\
1.73202380455672	1.67839194624969	-1\\
1.7388958192079	1.65750442906017	-1\\
1.74477233525383	1.63673203175308	-1\\
1.74966267516788	1.61608383044526	-1\\
1.7535771017491	1.59556845221873	-1\\
1.75652677304588	1.57519408190131	-1\\
1.75852369717357	1.5549684693112	-1\\
1.75958068713627	1.53489893692884	-1\\
1.75971131575822	1.51499238795994	-1\\
1.75892987082534	1.49525531475434	-1\\
1.75725131053274	1.47569380754603	-1\\
1.75469121932866	1.45631356348047	-1\\
1.75126576424051	1.43711989589634	-1\\
1.74699165176331	1.41811774382983	-1\\
1.74188608538576	1.39931168171035	-1\\
1.73596672382384	1.38070592921807	-1\\
1.729251640027	1.36230436127426	-1\\
1.72175928101636	1.34411051813702	-1\\
1.71350842860981	1.32612761557581	-1\\
1.70451816108362	1.30835855509958	-1\\
1.69480781581517	1.29080593421441	-1\\
1.68439695294701	1.27347205668772	-1\\
1.6733053201073	1.25635894279764	-1\\
1.66155281821753	1.23946833954675	-1\\
1.64915946841372	1.2228017308213	-1\\
1.63614538010324	1.20636034747769	-1\\
1.62253072017518	1.19014517733939	-1\\
1.60833568337824	1.17415697508866	-1\\
1.59358046387646	1.15839627203853	-1\\
1.57828522798929	1.1428633857716	-1\\
1.56247008811939	1.12755842963336	-1\\
1.54615507786788	1.11248132206881	-1\\
1.5293601283342	1.09763179579211	-1\\
1.51210504559431	1.08300940678014	-1\\
1.4944094893488	1.06861354308165	-1\\
1.47629295272941	1.05444343343469	-1\\
1.45777474325063	1.04049815568613	-1\\
1.43887396489042	1.02677664500734	-1\\
1.41960950128241	1.01327770190175	-1\\
1.4	0.999999999999998	-1\\
};


==> figures/results/scenario-det-traj.tex <==
\addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999097315186919	0.240119845720588	-0.998329213122516\\
-0.938412095353681	0.295440126566335	-0.949231614583555\\
-0.878512791615236	0.340806297596779	-0.897664364211227\\
-0.816611331132436	0.388391284107827	-0.846652518350923\\
-0.756264247299061	0.430953857706298	-0.788542795559308\\
-0.693346798677602	0.477179850170322	-0.732806726098525\\
-0.633599009497513	0.525691123326287	-0.676768599237468\\
-0.577290825638977	0.574995702674751	-0.62150517088954\\
-0.522309512888715	0.624423455192063	-0.563569290256212\\
-0.465574742731491	0.673509682453996	-0.505666770494669\\
-0.408892490796794	0.719829021405084	-0.4466054956301\\
-0.352503658971736	0.766191572476398	-0.387410026197205\\
-0.297805366356346	0.812078150921203	-0.32558236930593\\
-0.243030960615153	0.85623754604451	-0.266362897759654\\
-0.193520760069313	0.904286350006819	-0.206959562961663\\
-0.141157391253395	0.953475887168867	-0.147201815584372\\
-0.0907455166952493	1.00139735951368	-0.0872885080405619\\
-0.0425576690079486	1.04778289551989	-0.0244577705657749\\
0.00282492915169044	1.09781824649243	0.0438777373380001\\
0.0565737955837675	1.15187541298268	0.106313216204646\\
0.10797019440556	1.20087217888338	0.172377656132818\\
0.161325119672917	1.25350548595618	0.237191095676087\\
0.21515978458401	1.31753096196156	0.300213086496812\\
0.271392805977068	1.37424111359057	0.362520098681723\\
0.33201801548201	1.43988655879183	0.427342396078996\\
0.391186315944183	1.50307631027328	0.495517768370902\\
0.445452114069583	1.56734539496914	0.566020288498512\\
0.506908482655378	1.63732088245499	0.634263296387283\\
0.549331935555102	1.6982240836136	0.699553937681523\\
0.604175723754949	1.76574419525826	0.765610972521112\\
0.659242072905705	1.82706975910274	0.835674754685076\\
0.713341541594064	1.89135293476561	0.902719944809226\\
0.770566008293583	1.94223570293987	0.964915878680431\\
0.827908195113713	1.99664706311779	1.02845572132607\\
0.890029784434075	2.04669553968328	1.09704364513822\\
0.955033659834317	2.09854691738488	1.16135988571675\\
1.01606760509757	2.14580206338748	1.21349562315363\\
1.07817559373134	2.21111847854855	1.27513029909803\\
1.1385821153485	2.26186625269289	1.32688609329567\\
1.20282493344029	2.32082152819043	1.39144809294066\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999667657862896	0.238173218303069	-0.997920668690405\\
-0.935784903697031	0.294398781427412	-0.949305133532812\\
-0.871210886795331	0.339217052961964	-0.902298536164682\\
-0.808200323443767	0.381929987661314	-0.849842262277774\\
-0.745813121953649	0.427107037955903	-0.798055905865515\\
-0.685129650788503	0.471942116021726	-0.745323886694096\\
-0.625304784298019	0.513570237308726	-0.693036976465682\\
-0.561810557637919	0.5554630076023	-0.643233500134224\\
-0.497163268612965	0.602609195051863	-0.589181958819995\\
-0.432870421577076	0.647717260435037	-0.541959806017581\\
-0.364732968296831	0.69175127298335	-0.492664363513962\\
-0.293457473207169	0.737765842164415	-0.443461715072101\\
-0.221934597662915	0.781366467477909	-0.396141012609215\\
-0.151103072946458	0.829666097750292	-0.352774052167906\\
-0.079247201751869	0.875330162963369	-0.306992134685458\\
-0.0065383115673814	0.920822809406805	-0.261741840358181\\
0.0644181911695005	0.969729747414371	-0.222088542729676\\
0.133873375463614	1.01213439957069	-0.174695113950791\\
0.211492204651671	1.05545602117726	-0.134289503229383\\
0.285919287914461	1.09413121789221	-0.0965963536127306\\
0.360094750580293	1.141824701382	-0.0564671814732959\\
0.437112530752416	1.18201692282175	-0.0158825087122953\\
0.511901831117608	1.22021870252017	0.0238666390745128\\
0.589930337717635	1.26811685005856	0.0683396505306249\\
0.668505584305252	1.31221622217147	0.102603112503561\\
0.739820170185275	1.35102097343292	0.137093133287093\\
0.817936143758984	1.39689732988944	0.171108615644905\\
0.89195169614011	1.43951244671421	0.204191235630114\\
0.968833705356383	1.47991378231493	0.227407522908481\\
1.04335471652829	1.53088700243087	0.254942466392028\\
1.11826650658343	1.57120971867254	0.276889956690151\\
1.19464354405239	1.61076484245047	0.300673516767108\\
1.272374741656	1.64905852456528	0.32068422032466\\
1.35515506597905	1.68737253394039	0.34225510062944\\
1.43732706164774	1.71610694613945	0.361396622647346\\
1.52164483412661	1.74963531223171	0.381795171980213\\
1.59752818231351	1.7863372178692	0.393402774599737\\
1.68048549684154	1.82243685751266	0.411131597581458\\
1.76939850653048	1.84988554472865	0.429142328458342\\
1.85293455268544	1.88858911443502	0.447308380711106\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999924837645672	0.241729177915146	-0.997478542776999\\
-0.937681164454054	0.292192750777386	-0.946703338527673\\
-0.878568289169036	0.343650225908645	-0.905308451817009\\
-0.818919711852958	0.394420933981825	-0.860678227362683\\
-0.754598519921171	0.440324111021316	-0.816337589535641\\
-0.689433670270014	0.489478495783867	-0.771326094999197\\
-0.626931673928238	0.534328670500652	-0.724755812370957\\
-0.566270433800586	0.583945836072204	-0.673426835276538\\
-0.5027953539105	0.633129182445539	-0.617329134314982\\
-0.443648624447506	0.681483771291245	-0.557108680896433\\
-0.381459744230073	0.724035331737841	-0.500230688911273\\
-0.321631027984259	0.76620000505117	-0.445800818212269\\
-0.259610519426787	0.816590856645716	-0.389021038288267\\
-0.196360582528207	0.863726388066227	-0.329800722523275\\
-0.138093303928964	0.911039500425341	-0.26642811127088\\
-0.0803888829457074	0.964797150196262	-0.208107030910868\\
-0.0211098465411437	1.01986537164632	-0.14941524298466\\
0.0424767654185755	1.0735123437897	-0.0850116423601921\\
0.102890399436442	1.12647594020454	-0.0267406652018197\\
0.1638152334735	1.17812365106589	0.0335642712888511\\
0.217369303309985	1.22710835879745	0.0923958316330016\\
0.273212289080171	1.2769121142545	0.151282815622763\\
0.326735137756616	1.32810755374869	0.208531645226444\\
0.37725296408845	1.37561128013418	0.266859890366238\\
0.429410292599422	1.42541532145426	0.328279951489699\\
0.481162847280057	1.47170369969262	0.389705496781714\\
0.52932906959137	1.52164030506356	0.449005272619135\\
0.574000185312082	1.56991382284694	0.505705798064868\\
0.619548005893587	1.60567741835183	0.55876119786146\\
0.662750942195111	1.64296270893025	0.615527738407152\\
0.707841582658699	1.68811455830587	0.672353114429739\\
0.750445765376639	1.73566971057371	0.730152122611179\\
0.796494069861394	1.78355092966546	0.786834106374463\\
0.839344706221885	1.83297375351583	0.850164601489153\\
0.87931395490178	1.89326684830717	0.90916643430478\\
0.915777648722567	1.94770717605551	0.959944434582392\\
0.949782110304803	1.99867803352606	1.02079645971072\\
0.983925357006963	2.05455423479001	1.08344051779624\\
1.01075553830751	2.10281458745752	1.13305205104931\\
1.04379994530776	2.15211816265308	1.1907194622744\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999478013440514	0.239121487946158	-0.999664169531621\\
-0.937919876202622	0.300262643840738	-0.949440908815235\\
-0.872945467509057	0.340046629608734	-0.896844670300923\\
-0.804632616432495	0.391936590717664	-0.839258657082587\\
-0.742691908422451	0.442684134614955	-0.781659198657779\\
-0.673202502243283	0.495630071255598	-0.719673845258915\\
-0.608168576948165	0.54780125920894	-0.651868795849366\\
-0.544810218600067	0.607407133032499	-0.579597294613321\\
-0.487314311397158	0.665107114801059	-0.509448534652274\\
-0.432317215081443	0.720341586380996	-0.439604476220697\\
-0.376675469530773	0.776095232950088	-0.369240626938829\\
-0.327117596602069	0.838461179420792	-0.302687526082584\\
-0.270657245407119	0.893645480317961	-0.2334230398002\\
-0.217031304029397	0.951272579562135	-0.16979722191176\\
-0.16313207559679	1.0019400607661	-0.101346322294367\\
-0.110643155564647	1.0579217936251	-0.032360869655571\\
-0.0571374588816951	1.11765721426541	0.0321714731982948\\
-0.00268375698680666	1.17624748971723	0.0957200692271709\\
0.0600950417554353	1.23908422052683	0.155574377739027\\
0.116628584544364	1.29854070254098	0.221616645435937\\
0.174352152453095	1.35911963201167	0.282043748453936\\
0.226881686004214	1.41883910376421	0.342040959781102\\
0.278859926509455	1.47489728216788	0.409194268661487\\
0.338077194537511	1.53169947861436	0.478150815151479\\
0.389425510186719	1.59133650957836	0.54159794166849\\
0.440920309230101	1.64134669664039	0.614851913131274\\
0.500769228324601	1.69736098010417	0.684263666035433\\
0.557427566640788	1.74929691731827	0.757367514396136\\
0.620095323988923	1.80111935439877	0.825193497402672\\
0.679861845802182	1.8504353721842	0.888987578365886\\
0.749867191447688	1.9049557385142	0.959037787026043\\
0.816187231743557	1.95461102350735	1.02605016818157\\
0.882605878828086	2.01233926787184	1.09987866918675\\
0.945865302569833	2.06557461300503	1.16485708437803\\
1.0054864236239	2.11745255540829	1.24129861209178\\
1.07355599734616	2.17706887679202	1.30473662224727\\
1.14074214222072	2.22275149504989	1.37680807708408\\
1.21409580086994	2.27917271594911	1.44486037917327\\
1.28265929370191	2.33709720180578	1.51601873073528\\
1.35064422845006	2.39357851378861	1.58384642030979\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998394363748421	0.241391636925528	-0.999676549414364\\
-0.936918381121223	0.298669992849192	-0.952094821158014\\
-0.875767908208196	0.343758352253392	-0.902905729901582\\
-0.815197212569857	0.392635576534526	-0.852626760192742\\
-0.753561249753385	0.440544606832965	-0.804526772703398\\
-0.688172570774846	0.490685192407003	-0.75064146760025\\
-0.624898115728265	0.546176192777976	-0.699077403445479\\
-0.561099281407153	0.602664714348731	-0.647079927584265\\
-0.49883757961662	0.65759771439262	-0.596232810753198\\
-0.435796183985938	0.710038888086768	-0.545440631051465\\
-0.373558648862864	0.769846214817057	-0.498040297105428\\
-0.314811782972639	0.828358498517937	-0.449357447921745\\
-0.2524024449055	0.896486465279975	-0.400265727976023\\
-0.192428253892741	0.962132014710789	-0.352285981124797\\
-0.13614184645904	1.0347170348175	-0.302497530760353\\
-0.0789206302516105	1.10277525703474	-0.248021472590597\\
-0.0251768291052274	1.17080059360707	-0.194291800797375\\
0.0293264326133252	1.2338702608214	-0.139257610005553\\
0.0861150100645423	1.30144023970158	-0.0886725710442827\\
0.143442980144328	1.36360002529055	-0.0369989662238396\\
0.201833597136823	1.43654387106327	0.0139565168372836\\
0.264952058314463	1.49954728847255	0.0605763557484886\\
0.327707811149283	1.56599261571286	0.110653745496687\\
0.394652125690023	1.63494296894629	0.160483867893581\\
0.452484459751574	1.70202312042417	0.210802665712741\\
0.5188420244303	1.76826251934115	0.265571934717872\\
0.583542550314195	1.83009966842947	0.317526540822369\\
0.652423235208146	1.89615201453503	0.371432798691608\\
0.722234329351696	1.95296742904529	0.427563973234104\\
0.797316877094472	2.00265708470708	0.483030450142666\\
0.872521777413502	2.06269868321607	0.544082891500222\\
0.942497800152492	2.10832357916145	0.597794893697672\\
1.02164341774071	2.16643438555882	0.659641741117754\\
1.09658968206325	2.22547782002623	0.722617067153515\\
1.16500599235602	2.28256003924498	0.778822768177995\\
1.23073515842758	2.33094914084345	0.832729757842996\\
1.30930344784289	2.38209429114025	0.887390751044605\\
1.38102199640084	2.43537171679772	0.947746989953797\\
1.45358138892782	2.49672284031577	1.01248982293028\\
1.52283257003745	2.54991729243403	1.0745339534392\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999206536821372	0.240614747710416	-0.999073765700739\\
-0.935747572771599	0.302554105470016	-0.949879809824215\\
-0.870085126440494	0.346651400973685	-0.898353459256663\\
-0.801329617155861	0.391252537491979	-0.844179580165398\\
-0.727861053855633	0.437286842337528	-0.793252966531727\\
-0.659903423554284	0.481716265764999	-0.742017905787137\\
-0.588749767361451	0.526441936775682	-0.687609600606862\\
-0.521788163477617	0.569496176155087	-0.635303353428615\\
-0.452161445437019	0.612263906426604	-0.583944864080208\\
-0.384968777677234	0.653505830051902	-0.53273794985631\\
-0.319373798657001	0.699595877740737	-0.480702393197372\\
-0.25002209192796	0.745477200657465	-0.426650616009033\\
-0.183112722215193	0.790983304225942	-0.367161808439276\\
-0.116039073883759	0.832499824607219	-0.305981387013783\\
-0.0491504999613637	0.872769645838886	-0.239981629032361\\
0.0134816638648992	0.917597551479742	-0.178202779981601\\
0.0776509297510142	0.956300051644895	-0.121771618324796\\
0.14816734953278	1.00064341847066	-0.0626745455673806\\
0.209082679261966	1.03734764337466	-0.00566020908517983\\
0.270636163818125	1.08074926264287	0.0485983283630865\\
0.335290536577594	1.11599847599121	0.111213780993127\\
0.398364715998242	1.15735503127916	0.170549149837201\\
0.462491158506485	1.19526592435404	0.228020511597368\\
0.526985046473297	1.23750385738186	0.281181029826116\\
0.595398138508177	1.28667294923754	0.340404343741137\\
0.654031403299382	1.33332692039148	0.400327171479644\\
0.715529531168409	1.38070372121129	0.464413802530454\\
0.774004358053077	1.42673058628537	0.532988378815541\\
0.832772151192636	1.46705069051013	0.599592577059147\\
0.888441175422733	1.51648837018956	0.662001696238218\\
0.946164642931846	1.56144889657937	0.72553379100922\\
1.00727868284173	1.61147515367677	0.792025434252592\\
1.0605874770109	1.66222244787825	0.852979107012315\\
1.11579267058985	1.71036936269883	0.913129270544734\\
1.17362794424683	1.7652853772959	0.985685724399741\\
1.23473228422935	1.81102251786995	1.05801304258326\\
1.29133062734567	1.86213339013939	1.12443621282147\\
1.35060711126922	1.92355931891312	1.19781805762717\\
1.4072385425516	1.9799713390525	1.26482317833978\\
1.4677627386464	2.03973471946858	1.33607070297014\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997883052500354	0.239562788719727	-0.999762184395189\\
-0.940996731810911	0.299202210121269	-0.948236377052586\\
-0.87911351281499	0.346255871198857	-0.898271486084\\
-0.823675025519549	0.389823822937065	-0.838610405547637\\
-0.769904405349007	0.434968934088193	-0.780165200632715\\
-0.712807781097405	0.474518048507076	-0.71472077338568\\
-0.65255664237385	0.520020696850162	-0.652418996932862\\
-0.595516806784177	0.558357933009645	-0.585080714163673\\
-0.538107912019687	0.602900647134081	-0.527400225730435\\
-0.483908647992432	0.644795766482449	-0.470550629464525\\
-0.43519436620072	0.690958385027276	-0.419232662240288\\
-0.382523690858809	0.735316388859158	-0.362577962272532\\
-0.329902162460523	0.776602583521377	-0.306884233448779\\
-0.278082033030916	0.828359581808442	-0.249840917333089\\
-0.225079816712181	0.876241512989808	-0.19531162091268\\
-0.170900832214055	0.925176847067152	-0.144054855766131\\
-0.116742834690869	0.973018330820666	-0.0893300328887857\\
-0.0624394644136377	1.02153583572487	-0.0448568270436764\\
-0.00577332859339685	1.07044479374776	-0.000920093897412682\\
0.0553641530800267	1.12488706094108	0.0436711281739225\\
0.114230016053197	1.17850102451915	0.0856520695225139\\
0.176789081501078	1.22591104014739	0.125805264868109\\
0.235512507891229	1.28004758400266	0.167331607676494\\
0.295535859530024	1.32939277352212	0.209155733249646\\
0.353722194315284	1.38011443215806	0.249022341216393\\
0.414532535755917	1.43675919406431	0.287667774705727\\
0.479258626095354	1.49600354249477	0.329848877583506\\
0.53173124446456	1.55555084735801	0.369697097335034\\
0.592932355954638	1.60842797308848	0.40975237770025\\
0.655115745090827	1.66474625526034	0.444502588779189\\
0.715754777221152	1.72403338974776	0.483427225629467\\
0.781599442546714	1.77381994572981	0.519613707393719\\
0.838067541498961	1.82717185638151	0.554225113916129\\
0.896449291980583	1.88818802403999	0.595879865356262\\
0.950550526056233	1.94171452484885	0.637873644316729\\
1.00895588826109	1.98508109395879	0.666801709341455\\
1.07027089243773	2.03911541539847	0.697469444289449\\
1.13282803001197	2.09728817885692	0.735774512405907\\
1.20244497662939	2.14622201057137	0.768879084125373\\
1.26927320717982	2.19726941539339	0.796044395505939\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00063716616188	0.241454311329808	-0.998645583687718\\
-0.937205208924317	0.301802541380557	-0.952111243642743\\
-0.876642622141368	0.34868600566378	-0.898622993834135\\
-0.819781338820658	0.395331527475424	-0.847474210687307\\
-0.758410314173534	0.444448998456875	-0.797983044158325\\
-0.693252783818156	0.497173217701488	-0.749053419622195\\
-0.629842025464283	0.550715637495785	-0.701412945984744\\
-0.566563601183096	0.60211363522896	-0.649075231225138\\
-0.506677778174417	0.657528260049903	-0.597745300773904\\
-0.438572139081411	0.717734841290323	-0.546013837285958\\
-0.372168895391132	0.777188744693852	-0.492202320471858\\
-0.315253685667198	0.838041290093364	-0.439557757902515\\
-0.251982770072643	0.897644255227291	-0.389011336626355\\
-0.192999006836236	0.960516347810662	-0.340087475761595\\
-0.136795947951068	1.02179893723344	-0.296563342468607\\
-0.0812706194522889	1.08396767647464	-0.248736117013248\\
-0.019614308991939	1.15097630173867	-0.20135460959152\\
0.0417152550813636	1.20744694247774	-0.154055536670709\\
0.10067181800372	1.26969969681178	-0.111070634989086\\
0.157637409496742	1.33124632079093	-0.0681202175718269\\
0.212813424725048	1.39292093026006	-0.020604002537148\\
0.272804998892333	1.45274837527847	0.0261000654517899\\
0.329804275226962	1.51344214336638	0.0676143578808853\\
0.387463218245537	1.57707583713732	0.118925726664259\\
0.446315174987434	1.63949739106265	0.165910214173213\\
0.5064195008976	1.7003305700312	0.215719432735994\\
0.560510198525291	1.75796494449459	0.260280536278802\\
0.623292017097367	1.825073278648	0.309005428639286\\
0.681940798166191	1.89490853929142	0.351218557850494\\
0.735341556594547	1.96304288399763	0.400036837865433\\
0.787907995854191	2.02429818414479	0.45033159091882\\
0.839314956909585	2.09842254323848	0.498438832575956\\
0.889821271244156	2.15752778842198	0.54592261509251\\
0.945814327792981	2.21859733023748	0.599545551758071\\
0.998989254242033	2.29081859034814	0.65084179676585\\
1.0555744088369	2.35574590616082	0.707343019389085\\
1.10345036676242	2.42200679028767	0.75968714801057\\
1.15266204462236	2.48423228126415	0.810776648317614\\
1.20538345445542	2.56802674263579	0.859657922911382\\
1.25750965581708	2.6253702260006	0.914616958698115\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999761700001014	0.239403006681903	-1.00064917212024\\
-0.937083741657319	0.294373445482623	-0.950469718385001\\
-0.866498553188442	0.339414873676002	-0.902809632387336\\
-0.795910058453806	0.382635376069131	-0.855747809311152\\
-0.722870800432642	0.425582219247966	-0.817688634859142\\
-0.650288491168251	0.468951313780107	-0.767575540394902\\
-0.57731033225852	0.514846285250778	-0.723355474033801\\
-0.509280094747592	0.562004399035181	-0.682855542108367\\
-0.443350252481358	0.615311835089838	-0.641896614799916\\
-0.36974734708259	0.668287915692574	-0.601156746642196\\
-0.297977393833331	0.722467178519768	-0.558465022701712\\
-0.222637099954328	0.771493790058387	-0.511730091595466\\
-0.14733763734938	0.822020443010629	-0.474378458458396\\
-0.0695166124726907	0.87151120941725	-0.431700718223935\\
0.00557842257860166	0.918921857558559	-0.388990247379048\\
0.0786352692641716	0.966885612175444	-0.346295891777934\\
0.151804010102404	1.01138556058554	-0.305464995906099\\
0.229184125424188	1.0587036306456	-0.264266006828897\\
0.303815765674651	1.10430062535515	-0.224765862907762\\
0.373161398829609	1.1514467749324	-0.185326287399925\\
0.449074088647261	1.19623366026015	-0.147777091255457\\
0.523856329732424	1.2401467952344	-0.109307611772504\\
0.597050856067149	1.28166219814115	-0.0733329690362184\\
0.666429531420284	1.34028457446826	-0.0357997775499501\\
0.734325524569692	1.39224101652019	0.00773283710159763\\
0.797214043380172	1.44181150257172	0.0432169956484051\\
0.860060750666171	1.48836632867528	0.0800071987863419\\
0.931424530450094	1.53670570482633	0.121163547677733\\
1.00062948743957	1.58978171720524	0.164634962687663\\
1.06316780852666	1.63763103683876	0.210132750385208\\
1.14239457049625	1.68275328595518	0.253975943840862\\
1.21261184245252	1.7298573092557	0.289613858523382\\
1.2852054776753	1.77838257977673	0.328176939380943\\
1.35716420480542	1.82792492289509	0.367898821959726\\
1.43219241032717	1.8799483647952	0.408911875974675\\
1.50751959665862	1.91701301547635	0.451607809764857\\
1.57498585601223	1.95862414773015	0.49433054244464\\
1.65492450528847	2.00299315142748	0.535073312125774\\
1.72552426370735	2.0446060887609	0.588618345274859\\
1.80027746548308	2.09282137366448	0.638922438455971\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996557484340456	0.238127046917851	-1.00033070407717\\
-0.93513036312295	0.294731733763121	-0.949236022945345\\
-0.872248630463624	0.33502965491585	-0.902049049719279\\
-0.811783366682228	0.373738005004437	-0.850490665650075\\
-0.743483424008749	0.420488362023471	-0.802506016003737\\
-0.678178150151024	0.464440157062153	-0.754900619054351\\
-0.613837722533753	0.505346708182796	-0.703550884169227\\
-0.550773095256114	0.544149676926005	-0.654597133463295\\
-0.484783111725279	0.576553565383625	-0.601380901785099\\
-0.419891026595235	0.602767477244866	-0.549539256249417\\
-0.355936053713014	0.628793672874905	-0.491666868401052\\
-0.287871815613709	0.657796338689459	-0.433591164827056\\
-0.223142450241228	0.687876582257511	-0.37692982574188\\
-0.1576564849622	0.716018257216614	-0.320710851529268\\
-0.0902147955503067	0.747648995606423	-0.260003452656784\\
-0.020992257203037	0.782254675672127	-0.202098856176548\\
0.0447952876140054	0.816035904893276	-0.139867454421879\\
0.107240191087314	0.845079539501693	-0.0830441012464023\\
0.166325622747975	0.878813853349971	-0.0204600605168311\\
0.227368626549095	0.913951924739406	0.0382483035671166\\
0.292686560664903	0.948482884708528	0.0986522426200731\\
0.355256906569886	0.978937354953976	0.159478173175479\\
0.417232181140286	1.00983197106356	0.224787873848702\\
0.481064852892179	1.04740121192606	0.291947225524282\\
0.543566132632117	1.08224217749785	0.357307703517591\\
0.608078679972692	1.11415210912127	0.429078478255093\\
0.672066702127995	1.14766939923219	0.49671352484031\\
0.732981496090601	1.18166390481801	0.568159265928992\\
0.783627929520301	1.21376666421331	0.640942806117818\\
0.8344997953883	1.24690171289741	0.716566771170719\\
0.885039902463244	1.28073374473318	0.786940207782146\\
0.930708452832229	1.3115687574571	0.860905840384476\\
0.98360931213329	1.34306895639374	0.939576414751668\\
1.03603582288931	1.37468961101943	1.01230001250279\\
1.08966971776071	1.40527663662884	1.08296245920174\\
1.13626295165955	1.42561490088607	1.15306202232274\\
1.19215253749428	1.45547645371559	1.22816334027747\\
1.24157209939946	1.47269876202887	1.30333572842356\\
1.30164444783406	1.49081693517748	1.38450619067058\\
1.35424781864775	1.51250693156614	1.46719124853321\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998143503907388	0.237834720674987	-0.997862096085271\\
-0.936119373375667	0.29635870836499	-0.948464643518147\\
-0.877015955066647	0.33924871954674	-0.903160394177027\\
-0.812590672948743	0.384192528212344	-0.858675410842631\\
-0.749281978678445	0.43131747400185	-0.814889078940378\\
-0.683932352360197	0.479000083663537	-0.772748103589553\\
-0.623711676075119	0.531963156861454	-0.73212274666469\\
-0.564845833995446	0.581550208705826	-0.694764928561899\\
-0.5055480002133	0.628453895740117	-0.65908097128571\\
-0.444316879162597	0.674607389249144	-0.623936411013735\\
-0.380007057096599	0.724880882819921	-0.58393302298713\\
-0.309997303481852	0.7756871852443	-0.543238813205964\\
-0.239000843607946	0.830241204981572	-0.500675070154326\\
-0.172836106117607	0.882627757546596	-0.460227256581453\\
-0.106308300553263	0.938201516825577	-0.41703412596941\\
-0.0471534947563634	0.989288780128619	-0.371691141212866\\
0.0117366833573346	1.04837825859809	-0.331429212711511\\
0.0727443352361	1.09819029551659	-0.293151152697399\\
0.135386836081989	1.15896980561673	-0.254126685777976\\
0.198628929069509	1.20673347677698	-0.213717569504495\\
0.258673408497719	1.25994052522973	-0.173099333122474\\
0.320150846837991	1.31866106270209	-0.134773249158211\\
0.378929026791078	1.38521212080011	-0.0983565558729863\\
0.437873959975012	1.44270196064706	-0.0614942750998124\\
0.492321536975069	1.50285652136453	-0.025457833716979\\
0.546318410874817	1.55391028322688	0.0166150332734676\\
0.605540743583913	1.60912346203265	0.0588836632214943\\
0.666835145503873	1.66369002246334	0.101656455169822\\
0.72514641941733	1.71731321995269	0.150913802880084\\
0.782775627550259	1.76859293944252	0.196711908174917\\
0.845024159096932	1.83350206120734	0.240048580285645\\
0.905431261187945	1.89610129815776	0.285097770227969\\
0.967434816477778	1.96053005994677	0.329864810774429\\
1.0263995539753	2.02495426435714	0.372367418412664\\
1.08691134623291	2.08659693821654	0.423219304952599\\
1.14247857492891	2.15222889688014	0.470000266194938\\
1.20268458384461	2.22302768969197	0.520221362073296\\
1.2639002057665	2.29081616581861	0.567124247456189\\
1.31723846452443	2.3636705289299	0.616132282466592\\
1.37474288671603	2.42693167401703	0.661817703761842\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00142900461296	0.240147957678304	-0.998406460851612\\
-0.938197324332236	0.295334718464668	-0.952216015599749\\
-0.876839873964868	0.350178567484294	-0.901017568029402\\
-0.817496685826353	0.39618640386396	-0.849058939655302\\
-0.754302742769883	0.44098662705796	-0.794953670378155\\
-0.69192095378022	0.486774376254353	-0.748227583885473\\
-0.631354894185067	0.540080255498246	-0.701509102663529\\
-0.567160208013936	0.589033886692762	-0.65416397239147\\
-0.498960196856029	0.639448901286538	-0.606626205052239\\
-0.433302647164134	0.690927832605153	-0.559422133930822\\
-0.367502040962729	0.740061535168137	-0.510308694318523\\
-0.304932952225055	0.795547537011483	-0.462312130639576\\
-0.246133728336513	0.844070893732651	-0.416333206049848\\
-0.183151079213261	0.89667013869535	-0.372597622473266\\
-0.123073122467333	0.949187994951381	-0.323872478356829\\
-0.0599848181730635	1.00269707003528	-0.283246784079472\\
-0.000309752347445189	1.0556467315861	-0.235367346343113\\
0.063173487596274	1.10473570297316	-0.189521452313285\\
0.123886762248131	1.15126495604683	-0.149011666221997\\
0.186443847513615	1.19844426176845	-0.107739925708104\\
0.24693645963093	1.24410024797039	-0.0705626168191486\\
0.308258490539158	1.28967133235073	-0.0290909828346624\\
0.367846196243475	1.32535456310175	0.00330638897666914\\
0.427108524834924	1.36331730750391	0.0424891208927427\\
0.487278962720125	1.40173273654597	0.078392918436746\\
0.545400045400908	1.43415701456405	0.118292343076596\\
0.609133393740637	1.46883226202543	0.155340761660565\\
0.665965407605042	1.50147064154481	0.192594451722163\\
0.726813411340104	1.53465599570732	0.231493014982381\\
0.78525879049664	1.56803461360385	0.269073261142687\\
0.838786959347744	1.58847390345152	0.303170465642419\\
0.892005642473626	1.61372688249988	0.343783246671645\\
0.950855960118939	1.64824200717464	0.372693398799394\\
1.0072378680843	1.6714115179774	0.404857575435964\\
1.06370903706535	1.69829559562477	0.440066723251571\\
1.12481121783017	1.73151505961917	0.474039891532218\\
1.18624750005605	1.76011557948633	0.50961939888103\\
1.24513870865576	1.79057214961095	0.545563326536426\\
1.30048742944756	1.81247736836193	0.580687749516901\\
1.35829865956036	1.84178797899312	0.611136084006384\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.000431929394	0.242108810241391	-0.996613678930367\\
-0.935395247542184	0.296696837414976	-0.949268898252742\\
-0.873466293320584	0.336764606567942	-0.904652114447874\\
-0.810857531351084	0.385165017454719	-0.862627261291802\\
-0.745019123144069	0.428570708651443	-0.823328312950029\\
-0.679732999223635	0.477891179298135	-0.778109137581995\\
-0.614085299734276	0.525537029290357	-0.73407857204494\\
-0.553436679857362	0.568002879711038	-0.688347702132144\\
-0.48873106549623	0.614967439871658	-0.643905357028129\\
-0.4257494399878	0.661433413824767	-0.600762487765264\\
-0.363236170211182	0.707915303996083	-0.558763809627151\\
-0.303957803765229	0.753165135814846	-0.520776306799409\\
-0.24553924893707	0.79938725917993	-0.481019442302414\\
-0.188214276627694	0.849078387009438	-0.440856542605533\\
-0.128743658521414	0.894051825053391	-0.404589860691225\\
-0.0744397850636842	0.944413409009806	-0.37611361594768\\
-0.0203425627323284	0.989312849002061	-0.342400349984501\\
0.0359658143602226	1.04358101270269	-0.312861974034751\\
0.0925091039836771	1.09763602470283	-0.286264633099817\\
0.144807044968857	1.15212865150002	-0.25918860109279\\
0.195680860483034	1.21246766894415	-0.233152024596562\\
0.240935939112717	1.27762167330057	-0.204539391843426\\
0.291908249317216	1.34282715546215	-0.175139414471213\\
0.340000559067686	1.4063321122499	-0.147170027959631\\
0.39158194427972	1.46969012595874	-0.118719167386497\\
0.442579932439202	1.5367482694804	-0.0870962927934579\\
0.488893576129766	1.6060146048989	-0.0532176495575057\\
0.532908376754002	1.67309253795844	-0.0226400508827586\\
0.577611649866443	1.75170206681924	0.0101117423579534\\
0.622171702248338	1.82756434998143	0.0446559497183861\\
0.666018123806787	1.8964131217669	0.0834059606004055\\
0.715364591791782	1.97093698788423	0.11904090063922\\
0.759105280982104	2.04473207028721	0.15684534030507\\
0.801045366455763	2.11641537296264	0.198211436191412\\
0.852682136375208	2.19166312589285	0.242416508774737\\
0.897160014769339	2.26941307026482	0.277077230807292\\
0.949585212081186	2.35692661164114	0.316272231060444\\
0.991432937900816	2.43551139464911	0.355832102985598\\
1.04250084342095	2.51861318429785	0.400757017845699\\
1.08025195696505	2.60354495538013	0.44687055238035\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999675674549572	0.240809603814368	-0.996921683921689\\
-0.936509765495007	0.295010362876939	-0.946156867203659\\
-0.877103012466081	0.340598187773546	-0.897014585165409\\
-0.818272275394896	0.387880425247887	-0.845897554927339\\
-0.7612194144048	0.435420541447693	-0.794485899749282\\
-0.704979922365958	0.479729633550489	-0.741286744571794\\
-0.639208909238037	0.52062089366172	-0.692090257591796\\
-0.577984003417673	0.563109006909322	-0.642529064414549\\
-0.517015284371299	0.609516847928064	-0.592728708926859\\
-0.453773579922665	0.653794869828183	-0.541515223852534\\
-0.390079089332476	0.697274369166527	-0.485863733536751\\
-0.327504657776601	0.739934896551448	-0.429486405389553\\
-0.262046441398609	0.782759138766421	-0.37033900678668\\
-0.200656581709071	0.823695585443169	-0.314480824297384\\
-0.135284097210144	0.856714784846357	-0.255904593947051\\
-0.0762283681468417	0.903093108106359	-0.202002253319113\\
-0.0157703330350061	0.945477958711656	-0.149355461581598\\
0.0496086043769402	0.983430956724827	-0.0939053984881232\\
0.118090518779486	1.02445102772296	-0.0402722598189369\\
0.193554947819586	1.06240224522367	0.0130537006441972\\
0.267871710043001	1.09142390631313	0.0672498013698857\\
0.340769264519242	1.13167393744778	0.126832226891232\\
0.415027483905811	1.1684706298973	0.185288116350222\\
0.493316719837835	1.20831694210164	0.246903465407932\\
0.569107983300983	1.24994792427442	0.306778315649002\\
0.643339190981587	1.28563769326021	0.362948265532255\\
0.717433211087527	1.32212580465582	0.420520769832319\\
0.789162984553019	1.36187154184974	0.47776243035757\\
0.857169685997231	1.4034313712596	0.529632835913584\\
0.924296060951781	1.43705292018788	0.591922695395719\\
0.99248551362416	1.46425018627655	0.653714754855534\\
1.06219677563893	1.49906144777219	0.716928985872617\\
1.12793576496037	1.532796602114	0.784138692702429\\
1.19188657303142	1.57148097241137	0.851479263160206\\
1.25398166792128	1.61627880764542	0.925146542849287\\
1.31955955764024	1.6621984086671	0.994470907699137\\
1.38426700887822	1.70276569314377	1.07090787017195\\
1.44694614785174	1.73113117810826	1.13828249090098\\
1.51331152355335	1.77379614841949	1.20205150378024\\
1.58202688317567	1.80498441091493	1.26572979578591\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998523188471092	0.24048552892452	-1.00170842600049\\
-0.935694876595461	0.294255158763531	-0.953312919699704\\
-0.873418569530788	0.338750563478147	-0.903297305057812\\
-0.805937368358524	0.384714228935152	-0.856472366409174\\
-0.73644881916597	0.432362602700558	-0.809117172270303\\
-0.666096514273311	0.47435451738839	-0.762009897867566\\
-0.591687476407541	0.515490821271538	-0.714647926220729\\
-0.520202312442606	0.554686755200702	-0.668895876428494\\
-0.445075328958954	0.597204489312534	-0.620528376394389\\
-0.373611501295216	0.636541202900459	-0.573202326591494\\
-0.295549321703794	0.675197984979172	-0.531126962977454\\
-0.219949517412132	0.716566562050213	-0.489533313473778\\
-0.147744684498745	0.762571193658453	-0.449373578371776\\
-0.0747871774099083	0.805580254413355	-0.405371776163637\\
-0.000202109465291554	0.846650434434639	-0.363725599102718\\
0.0753779075001549	0.888742353086232	-0.324305521727015\\
0.148253855657127	0.930235521506898	-0.283263750983281\\
0.223504508926574	0.977710040914858	-0.241468903491411\\
0.298977616156341	1.02924642998083	-0.201342160570331\\
0.371607400002179	1.08011982849191	-0.158799968742345\\
0.44370301713544	1.12859088483185	-0.119848679034722\\
0.515670821589246	1.17716622598193	-0.0756963960955148\\
0.584310341113133	1.22100853665103	-0.0380155945506723\\
0.659067341253921	1.26929434150498	-0.00232670106254471\\
0.732343555720719	1.32066213858617	0.0353356334245465\\
0.80901870036679	1.36620824688496	0.0765995747885008\\
0.884830417415499	1.42409074044718	0.117268979460787\\
0.953978596030018	1.47702275851655	0.157121450691774\\
1.02794018824188	1.5266594734392	0.194957906169915\\
1.0977445584735	1.5784186864705	0.235820516626036\\
1.16676120248622	1.62998773548756	0.282958365704768\\
1.23308664372872	1.68333826260255	0.329986096163865\\
1.30143636944258	1.7270812039364	0.375240226634142\\
1.36936122985612	1.7726067393875	0.423324001247358\\
1.42882773716402	1.8141801079722	0.465804077238354\\
1.49270864182533	1.86094409073697	0.517680618134507\\
1.55421912696374	1.90875222482126	0.564929672971485\\
1.61189952531815	1.95651327017592	0.617552476208053\\
1.68018299996685	2.01627387974435	0.671481385110162\\
1.74317521048629	2.07317420510261	0.725931570315693\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996266401555801	0.241065408109953	-0.997524270030674\\
-0.935616037530966	0.298961037372814	-0.951290848895173\\
-0.874271186655702	0.341871700352364	-0.899247061247083\\
-0.809770474953617	0.390197258806424	-0.845434199766446\\
-0.744783683903365	0.440345301405434	-0.792957324392102\\
-0.67832651014073	0.489964877939231	-0.74178982719984\\
-0.614311038930228	0.537634431299462	-0.686781912050792\\
-0.550704392560502	0.587461630952286	-0.628914223909\\
-0.485076361067475	0.645340318151365	-0.570181501562755\\
-0.422779396086289	0.693670264799247	-0.513776130221047\\
-0.358407445522421	0.745514559139438	-0.45387248940336\\
-0.294554756489185	0.800494452650882	-0.395580236585909\\
-0.228370504371983	0.857626438502614	-0.340759525021052\\
-0.164919570666964	0.918189069285596	-0.284081000782394\\
-0.100428300424231	0.975671411156861	-0.233126161714587\\
-0.0364873631808184	1.03354529816135	-0.174485607486058\\
0.03039503565278	1.09414494202886	-0.120043416591615\\
0.0966370966310939	1.15705947319445	-0.0604133705478779\\
0.164139675264674	1.21258994170563	-0.00387211094833333\\
0.234579919298428	1.27117994893513	0.0555895249896556\\
0.305604083576958	1.33347476322621	0.115301323866013\\
0.379635059950721	1.3991913971082	0.179514850063613\\
0.445239738524514	1.45915603264508	0.244340787753376\\
0.511424747596353	1.53032589957715	0.308376282465888\\
0.587592606715259	1.59903285665379	0.373734646131174\\
0.662927073760067	1.66167057488262	0.442080929446937\\
0.733463540853294	1.72478466110331	0.505233329322579\\
0.808293643815278	1.79699096215508	0.569880227308837\\
0.8822383050201	1.85960945772145	0.63979966364737\\
0.956602348522238	1.92284929365042	0.707140390382085\\
1.03346178189316	1.98734342347434	0.773131982992607\\
1.09750265277435	2.03994716096301	0.839721978493359\\
1.17178781605971	2.09700204093048	0.91469809006404\\
1.24578754766594	2.1606719798423	0.990379204647398\\
1.32598663784628	2.22737527943389	1.06791622348461\\
1.39326662282973	2.27572595369693	1.14591160953309\\
1.46317253085109	2.3362594425709	1.22851334309658\\
1.53616151781272	2.39669887221766	1.30699230440716\\
1.60590422014942	2.44918304097556	1.38804621914146\\
1.67886003856337	2.51380092142403	1.46795566141155\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996553195622749	0.241428731307668	-0.998680181989563\\
-0.936946398371795	0.296336888334277	-0.952899488956145\\
-0.868689540023367	0.344896077759647	-0.908049532780763\\
-0.797570013485324	0.392245353521358	-0.858788927314199\\
-0.727135133834651	0.439187572096872	-0.810245505490446\\
-0.656863674494348	0.491748415547409	-0.762986536853851\\
-0.589304108632216	0.535215398766491	-0.710713696252079\\
-0.521841596907772	0.583515855202647	-0.663010546813638\\
-0.459070593961333	0.632181652937738	-0.617375011773583\\
-0.396084333707836	0.68122609357534	-0.566609871526138\\
-0.331537023497307	0.728529095980444	-0.516462479103587\\
-0.270461608280935	0.776666307276697	-0.468661122470562\\
-0.208959096208436	0.82253710485579	-0.418560260672453\\
-0.148109906408346	0.867854260607204	-0.368559657787423\\
-0.0852661901429587	0.911916664075609	-0.322616294682748\\
-0.0281724629784662	0.956549830375345	-0.273431922590461\\
0.0316297453834707	1.00411955573829	-0.226040408533207\\
0.0940424900614943	1.04969457192387	-0.177012415465904\\
0.153463820027174	1.09871927638879	-0.12832482154147\\
0.208426073295889	1.14300127994308	-0.0758349198329008\\
0.263029737410235	1.18294801174318	-0.027244607005956\\
0.309987666860116	1.22848019726555	0.0183252554270275\\
0.355168539900888	1.27011340902465	0.0641514958055227\\
0.400838745159028	1.31232369003444	0.104748933688482\\
0.446210174248702	1.3561230716174	0.14553077380875\\
0.490297226838374	1.39353204803897	0.184628834162501\\
0.53132077982562	1.43449859590389	0.225259351355798\\
0.579360011591246	1.47423522063302	0.265770644211078\\
0.620114687428883	1.5137881427356	0.310008645574089\\
0.662268500042963	1.56344772551497	0.35352676324262\\
0.704181777392747	1.61483448149668	0.393366649469507\\
0.74416992319634	1.67017122458545	0.4359345662294\\
0.786861093748554	1.72853097027624	0.480056910850364\\
0.825863620126442	1.77262520011	0.519936418871072\\
0.867748587436645	1.81846500584132	0.559978643448845\\
0.904348079717769	1.87077411002873	0.601503898989438\\
0.939957131715918	1.91938102343195	0.647163560902774\\
0.984100613984313	1.968429123356	0.687504026488806\\
1.01875351501244	2.01604337703786	0.72948485477501\\
1.04955551295515	2.071497787221	0.76585638322754\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998879902201073	0.240496085513992	-0.99988366606658\\
-0.939370794986175	0.299688628768168	-0.950860526824933\\
-0.873789045122942	0.345583716334724	-0.904156203431173\\
-0.804188423871314	0.397335530731634	-0.85364545886601\\
-0.738232606420457	0.45007556760859	-0.806257935093803\\
-0.673380637037804	0.504234232855233	-0.75674450493024\\
-0.609847130544732	0.562259906775999	-0.704740058997178\\
-0.544257641839152	0.613043902150979	-0.657951432356445\\
-0.474965162789158	0.664304469295863	-0.611695161932119\\
-0.407099820977274	0.724749841543837	-0.558969937446712\\
-0.33348289548803	0.783060905035537	-0.506787300641006\\
-0.26540003473959	0.841948910151505	-0.457250201837349\\
-0.195976614764264	0.897326878189592	-0.409250105902261\\
-0.123554371748513	0.955647713582156	-0.356437774225914\\
-0.0552666572992857	1.00993096643663	-0.308400481284111\\
0.0144717608967379	1.06703826389719	-0.25437161816529\\
0.0911764688052082	1.11871904774566	-0.206025367099183\\
0.163761483087618	1.16945201153436	-0.153264874298582\\
0.237617842680693	1.21996092266649	-0.103993833305754\\
0.31463664029243	1.2789093299813	-0.0549133951063001\\
0.393438353942507	1.33219400122285	-0.00456118324455546\\
0.470623632413837	1.38843610152572	0.0422677329824553\\
0.5526201097657	1.44449013484385	0.0885204495478698\\
0.634651552228326	1.50616302618079	0.136904016950607\\
0.72025096587917	1.5724370314638	0.189311364249635\\
0.794706215447156	1.63153022791049	0.240944076360831\\
0.880896683430186	1.70352199722535	0.295045005811415\\
0.966734560096649	1.76698222317146	0.338746543162434\\
1.05158054734628	1.83490239619738	0.383807170676711\\
1.14501742093597	1.90974711679438	0.428760396921591\\
1.23643583967319	1.97863582803307	0.464731570803217\\
1.32462125867028	2.04379879798905	0.504847827125861\\
1.41534672207407	2.10608913194866	0.539949721838696\\
1.51144870099735	2.16982541766346	0.577831754697006\\
1.59059562940606	2.2382519077932	0.614215323291034\\
1.67620167064393	2.30195908047853	0.648005908040606\\
1.76144098834775	2.36756621870626	0.684560028601531\\
1.85342007642594	2.43203666681135	0.712997443832887\\
1.93248096066779	2.50270747971638	0.742465233245272\\
2.01662392343828	2.55281677520205	0.766402992723045\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998186840084946	0.241238126532768	-0.99575913010429\\
-0.93910655074124	0.295197335550279	-0.94816137861081\\
-0.879566605680491	0.34774384672798	-0.904031152519019\\
-0.815485814067297	0.39518190071445	-0.855337447663044\\
-0.751283235483321	0.447638161782792	-0.807095082872336\\
-0.68777329853078	0.498580686058877	-0.759130780209098\\
-0.623532697387901	0.54981545761173	-0.712553875593714\\
-0.560444288094363	0.596732133763351	-0.669823215352021\\
-0.500923289589524	0.649962270044387	-0.630354768568722\\
-0.439217692788261	0.70269553082119	-0.597529292235517\\
-0.382377505947668	0.753636233053346	-0.565417465490072\\
-0.326986875308349	0.808659484033586	-0.533639240895368\\
-0.276188885195786	0.863493979132822	-0.50445883928031\\
-0.220440558413139	0.922386013886069	-0.476520822699489\\
-0.167307434473189	0.984501715839633	-0.450362731923827\\
-0.115980537432391	1.04575834750217	-0.42361032661191\\
-0.0605358746356502	1.10209660914717	-0.398929354089092\\
-0.0124327974852918	1.16072501346216	-0.371653134877353\\
0.034373815565122	1.22345447538754	-0.342406795347864\\
0.083441933861303	1.28633735897505	-0.315279287820554\\
0.129345241622559	1.3499962899717	-0.286714139511742\\
0.173700219918909	1.40807926239857	-0.261012966568939\\
0.216862447993608	1.46865706647241	-0.23840836540336\\
0.263608652318412	1.53897001686056	-0.205886321889335\\
0.30119146157233	1.60681819495591	-0.181663804550202\\
0.339887347097249	1.6722033398497	-0.155163638663346\\
0.377296124081438	1.73704096989589	-0.129173329717089\\
0.419244588911832	1.80532865269098	-0.103187554488832\\
0.461599638526467	1.874338641162	-0.080219185013098\\
0.500299350194451	1.95379052822162	-0.0602792524145983\\
0.542228900556564	2.02021763986239	-0.0325275099175743\\
0.579641688465665	2.08746259300911	-0.00937972038193605\\
0.623227073988167	2.15365560616595	0.0195321961606601\\
0.665600501944054	2.2253126287606	0.0434950617180265\\
0.712914359812287	2.29086498906892	0.0728816646467084\\
0.762924661189738	2.3626291983752	0.101602939638156\\
0.809700720262381	2.42841258189739	0.128586396792931\\
0.858518206548166	2.49392383211801	0.155222973011852\\
0.908667903130117	2.56441707039368	0.174748914416757\\
0.953441004133035	2.62692835231056	0.193056381098966\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998501463206577	0.240622048850611	-0.997956032982096\\
-0.937380092684389	0.299739589435348	-0.948773765656467\\
-0.87288428821746	0.347166221913456	-0.894320302504629\\
-0.807684610880128	0.396017859973276	-0.835151346077745\\
-0.744529176595335	0.444283635809204	-0.776977159531321\\
-0.684774500862059	0.497270244904476	-0.722827206419273\\
-0.623058659794482	0.552846761725483	-0.674611875493064\\
-0.557856907490218	0.603684184662123	-0.624846806898406\\
-0.496017379702059	0.652288335401447	-0.573934216827273\\
-0.43300214697173	0.697762032164445	-0.529414021468079\\
-0.371599276837317	0.741167709577692	-0.484825068934523\\
-0.309379588785731	0.78443817232376	-0.435807416039495\\
-0.248278621653015	0.823641573001581	-0.391412712832659\\
-0.190766229789827	0.863015670568478	-0.352671634355826\\
-0.132950857574769	0.900897601534577	-0.315171867906392\\
-0.0785247158253818	0.939622352569191	-0.273730439469658\\
-0.0208412267141289	0.977094025030942	-0.236186927751407\\
0.0332996331060053	1.01712525855086	-0.19707575583392\\
0.0849339521357008	1.06091755685768	-0.162941831995224\\
0.143076282026755	1.11128190240168	-0.129669269501444\\
0.20129723334914	1.153573022764	-0.0894201939493836\\
0.259652317216535	1.19729800428796	-0.0599667397297685\\
0.315237186577836	1.24883014064212	-0.024474621888829\\
0.365262307022047	1.29946267625776	0.0084960433227074\\
0.411739106210097	1.35514135094607	0.0410666842690655\\
0.456330172505233	1.39810397050393	0.0749012268964479\\
0.502916568478967	1.4489316490109	0.108553878157218\\
0.550320654886159	1.49342870763487	0.143259081876911\\
0.597633145833903	1.54265003791567	0.186611771047641\\
0.651254439085877	1.58989861541072	0.225795991854095\\
0.706089601716066	1.63824149921117	0.265464746672398\\
0.755232603225867	1.68050412134056	0.302410296115793\\
0.801892633952299	1.72176174228032	0.338168917135952\\
0.851107023511234	1.7598184382646	0.379277603095691\\
0.910045444506951	1.79817423689589	0.419285501841558\\
0.961868295151989	1.84519947095436	0.456521047292635\\
1.01436343173049	1.88725122739054	0.489987371502914\\
1.06542357727094	1.93391401759271	0.52582168386404\\
1.11707626417437	1.98249589454058	0.560983146840853\\
1.16637519937206	2.02691607247731	0.594805476282318\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99941386444476	0.23981958381857	-0.99940192455211\\
-0.935790783494671	0.295973440151058	-0.946644440945783\\
-0.870953484147256	0.337920676615916	-0.895624035090351\\
-0.806049533947736	0.38222421949771	-0.84251474270725\\
-0.740628400801643	0.422809568428598	-0.785407613821271\\
-0.680530627252956	0.462177667265037	-0.732220734954956\\
-0.61755393063427	0.500809723334486	-0.677468006362588\\
-0.553039189053207	0.537744681941029	-0.619959926684529\\
-0.489261787921256	0.578833756878931	-0.563527496873362\\
-0.423585694721391	0.628139430911374	-0.507387672388164\\
-0.358626023549135	0.671992438111445	-0.451438345867636\\
-0.296604452183055	0.718979492251215	-0.394927180571802\\
-0.233893918287818	0.762479305620649	-0.344553852355452\\
-0.167105297522116	0.806033925762861	-0.294907121623299\\
-0.100313319827201	0.85173982157492	-0.243923305374739\\
-0.0347131128428459	0.899667072910527	-0.188163931381889\\
0.0318992766133705	0.951575077588766	-0.1292858123271\\
0.0939587124992772	1.0023203271045	-0.0722763537621054\\
0.155471461729173	1.05367549544397	-0.0178115528891776\\
0.217321132960819	1.11225191889027	0.0369684793519381\\
0.27554528441688	1.16293097072858	0.0897093697707379\\
0.326660311383942	1.21901725621047	0.140407098341125\\
0.385442278344885	1.27733913367489	0.19077295311036\\
0.442732556338243	1.33109214322283	0.242704778539406\\
0.496396603946829	1.38733670957261	0.29438914405709\\
0.555329633902037	1.44313816929292	0.346349961766558\\
0.620033187587347	1.49933564394949	0.390839968070357\\
0.681681133192265	1.55385734626562	0.444059387189137\\
0.744135120431133	1.60681685856481	0.497028103161948\\
0.806308037579827	1.66159800091263	0.548153405497722\\
0.868407163507737	1.71062740831277	0.599199521246646\\
0.934676220674764	1.76448356459484	0.647910551823576\\
0.994983441668676	1.81627499769647	0.706145087474844\\
1.05601828200952	1.87000952781779	0.763689518130537\\
1.11861872131484	1.92268947511914	0.822631392863396\\
1.18239123002556	1.97118733942239	0.883338236373165\\
1.24547410558845	2.00886829986752	0.942097873926395\\
1.30541690925659	2.06605985835185	1.00160730671751\\
1.37020522015701	2.1142811032267	1.06388348153475\\
1.43553978055996	2.15908326526873	1.1259099546486\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999628468123505	0.239790642200563	-0.99897927759309\\
-0.939925800908706	0.296042592806576	-0.949064983131013\\
-0.875266349827194	0.341981759663927	-0.899805478039031\\
-0.804988157029969	0.388379733543896	-0.848054750657497\\
-0.730863878676326	0.439183077783096	-0.798524228362854\\
-0.657229628784629	0.486499827915499	-0.74908000212884\\
-0.591572705893785	0.534692114499472	-0.692385359734553\\
-0.523491044983277	0.580256089716363	-0.637898006433409\\
-0.457554556262484	0.626900853575511	-0.579719222240134\\
-0.389307561274564	0.675277867740183	-0.520757303740208\\
-0.321688393728467	0.722238445144696	-0.462161158743266\\
-0.261025051333469	0.772806747316398	-0.398790377925144\\
-0.201063345419251	0.825260249199859	-0.33289621954988\\
-0.142939694616152	0.880967357489524	-0.271365782089549\\
-0.0813910921469937	0.936155200593185	-0.207630848641898\\
-0.0210017469487869	0.98501080558381	-0.146600239202634\\
0.0408571880641842	1.03141430640984	-0.0835191396259772\\
0.102559629102903	1.08339897598826	-0.0226885379086642\\
0.163285941463538	1.13423531389365	0.0368329525571538\\
0.219276401783637	1.17918896804226	0.0982186832816128\\
0.276765559566223	1.23679105028662	0.163320752261187\\
0.333328969610198	1.28749214820276	0.231279035800933\\
0.388619171172642	1.34493843504955	0.292770640756229\\
0.444828414861031	1.40285138095071	0.357407266050898\\
0.494106637458335	1.45481133434207	0.417668955022045\\
0.551519976997145	1.50744282891953	0.479277005462752\\
0.609527334442341	1.56374080085298	0.533384600137526\\
0.660641882932611	1.61065360475036	0.591186262409852\\
0.707875668819173	1.6616160999572	0.644315273213129\\
0.759877049222264	1.70183406754071	0.698100463494905\\
0.807391382574032	1.74113329991917	0.747273110092868\\
0.860306972237768	1.78248401822611	0.806325190862904\\
0.913578169490901	1.82597288384577	0.87063592936746\\
0.969532391995316	1.86960373815914	0.930738166463832\\
1.01990463281503	1.91287429474502	1.00193963235164\\
1.07299453257888	1.95180604141512	1.07103755000408\\
1.12383537811516	1.99496799553102	1.13293339534748\\
1.17997811518489	2.032273860388	1.20544540890979\\
1.23499557658421	2.06542254474042	1.27272747378511\\
1.29846587084545	2.10068936214979	1.33756443870261\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999289387007216	0.237332812311051	-0.99865554709324\\
-0.936795955100432	0.295679216182619	-0.947864624687105\\
-0.876927253238595	0.343276485769654	-0.901835879960475\\
-0.807559195861177	0.394613411621275	-0.854747083355907\\
-0.743768546633476	0.446741482146726	-0.809483242443629\\
-0.678382896751087	0.498546391877843	-0.768793193958187\\
-0.610558805239572	0.546513126155076	-0.724701612024884\\
-0.544798088817717	0.594782594672072	-0.682477760140318\\
-0.477717423893348	0.644362771969552	-0.639171197285377\\
-0.414418358748862	0.691799180516605	-0.600266258985882\\
-0.351400665563637	0.73769750361156	-0.560931573073746\\
-0.285030344315029	0.792222367499755	-0.520799493921138\\
-0.215875518663512	0.839978188612703	-0.482957520864315\\
-0.150297843540294	0.886646079218679	-0.447237042402936\\
-0.0834243279194481	0.941460547367289	-0.410865954985957\\
-0.0120904358143467	0.989775199494328	-0.368771018321348\\
0.0604389596442129	1.03455854433696	-0.321992784550233\\
0.128151640113722	1.08341974135171	-0.279405541600614\\
0.196461201678463	1.12184412337843	-0.236337765105618\\
0.261364979629248	1.16835261839804	-0.194519704650955\\
0.321670162964917	1.21348011410584	-0.148443088243086\\
0.386880370280435	1.25469593481258	-0.101284454693346\\
0.450604139635742	1.29798441047623	-0.0553452158533105\\
0.519616769322175	1.33857252486657	-0.00927014479227918\\
0.586521906558447	1.38208814561038	0.0334872371659635\\
0.651479688190949	1.42906114369178	0.0822244820957161\\
0.715133057155426	1.46881180996613	0.134969932829681\\
0.778497133532508	1.50840607572028	0.184921140176153\\
0.844392620888717	1.55205640548613	0.235492388502672\\
0.913743415717288	1.60113650258431	0.288495733080519\\
0.978645205210958	1.63933218766213	0.338369617629305\\
1.04825500823173	1.68263559166572	0.393018859135845\\
1.12063304513119	1.7377561187081	0.436865577122685\\
1.18924802745821	1.78313708669981	0.487671860194042\\
1.25671338534207	1.82607100488179	0.540897220914599\\
1.33248467847619	1.87102929043667	0.581395060032421\\
1.39846247339973	1.91831311160546	0.624230507074932\\
1.46414328393671	1.9681844481162	0.672364141523025\\
1.53497308785455	2.01054778187278	0.70841517391463\\
1.60973388371968	2.06134501267281	0.757824264378024\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998744597993324	0.239697364611478	-1.00082330309869\\
-0.934967296140122	0.29989064312524	-0.950157034366223\\
-0.86972779897256	0.344447275570136	-0.898492931569805\\
-0.80380434347782	0.395393403286442	-0.847069314899717\\
-0.736630584077776	0.442494611847942	-0.789790776091889\\
-0.674003912521172	0.487020472623881	-0.73099047887085\\
-0.611323579525427	0.536326358550417	-0.679711199720687\\
-0.547947112786439	0.579137292523701	-0.625531639441308\\
-0.481311197084737	0.625684368217938	-0.576752741050633\\
-0.409642341342085	0.671437090276521	-0.524345978719481\\
-0.336718700514058	0.719340455289502	-0.468647733249641\\
-0.263515877624212	0.764537815183044	-0.412902093600487\\
-0.193170181448085	0.817074647324963	-0.355392900262836\\
-0.121621247147764	0.85974469495509	-0.296083232311909\\
-0.0529290729005914	0.913964513283499	-0.234183540893584\\
0.018066553158035	0.967257398950404	-0.174826262009692\\
0.0855842031244479	1.01565889554435	-0.109527439163188\\
0.153506741555135	1.06719276334748	-0.0450340921768153\\
0.220285061205617	1.11310777866069	0.0210252373313124\\
0.281497338579451	1.17102949831046	0.0829191434970286\\
0.339841322499021	1.22475310286617	0.142844238515142\\
0.401649742735817	1.28167213514423	0.201115439123611\\
0.463472286329777	1.32816451866386	0.255587450212393\\
0.529027501161274	1.38937239025773	0.310707537689259\\
0.596295164673068	1.44161626270088	0.360966187991806\\
0.665240306388588	1.49373270512595	0.418294113130643\\
0.734892174207189	1.54703805668162	0.471188238947233\\
0.802609297475846	1.59677301506572	0.519727335807\\
0.876217114705428	1.64423008323368	0.577104341061865\\
0.946329772400645	1.69834838831746	0.636998461431551\\
1.01487012611064	1.74117426820574	0.693202951143347\\
1.07895364097138	1.80104867708122	0.747922193424177\\
1.14008865783622	1.84884542085864	0.792570040054611\\
1.19945130966865	1.90334134584269	0.842317791907883\\
1.25928968363361	1.96176365750833	0.888586581774754\\
1.32203621734675	2.01759594992835	0.933677571088026\\
1.38257667373151	2.0641937818398	0.978972812005777\\
1.44072191073415	2.12339258232747	1.03295774611234\\
1.50546098626268	2.18206423228079	1.07036803043518\\
1.55975887555877	2.23136827473192	1.11391344887868\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998885511378266	0.241910664800918	-0.996976547477393\\
-0.940040387614954	0.29766777320707	-0.951626881813066\\
-0.875761564352633	0.347260468102953	-0.907998660757468\\
-0.816470024118318	0.392983354135737	-0.858395523848572\\
-0.754390311738232	0.436969118715538	-0.807615616507622\\
-0.696814774846039	0.489813934789821	-0.756835415722019\\
-0.638662270138816	0.541508877072344	-0.704843504179646\\
-0.574028968528997	0.591552378645295	-0.647513506425095\\
-0.509217796623769	0.641755340240551	-0.592825936813614\\
-0.443576874144499	0.690388034449658	-0.536188529144945\\
-0.383392334500443	0.745883388683918	-0.481844860460854\\
-0.32076791702083	0.799986152509635	-0.427792737651208\\
-0.262775469604114	0.850507944820221	-0.372664024183134\\
-0.205120722121782	0.902966353198475	-0.317669078495082\\
-0.146466695321946	0.95216406785298	-0.262405454807257\\
-0.0944402357188441	1.00064680946135	-0.211676887176349\\
-0.0387710902211556	1.04811022977455	-0.155471755459173\\
0.0155118148154992	1.09073778226011	-0.100539150071169\\
0.0740883287702382	1.13531226263472	-0.0482031999438352\\
0.133198466176663	1.17946127642741	0.00682531674891407\\
0.186390976823255	1.22438350327784	0.0622041620040903\\
0.240426482745683	1.27381480766936	0.118910359755193\\
0.298220804718212	1.31774535893661	0.182176961892837\\
0.350962282352541	1.36020652557454	0.240485424587223\\
0.415578450780406	1.40564377342666	0.305952817557809\\
0.470425707641884	1.44524272280929	0.372190904752373\\
0.529456695012825	1.48131013532241	0.43712942967256\\
0.585962618128176	1.51817796589832	0.499198162661889\\
0.637974139056772	1.56445863246761	0.565512641325222\\
0.694442306998844	1.61081872437219	0.633828917433982\\
0.744965992305821	1.66223244724247	0.702182438107963\\
0.798239336855592	1.70818277921315	0.770943857544714\\
0.847036322537959	1.75413794824888	0.842854623769122\\
0.900452089866363	1.79544184131232	0.915267609387747\\
0.948305547722496	1.83679549021743	0.983009012267143\\
0.998056758900664	1.88047852779191	1.05674893858474\\
1.05288580690814	1.92371468087948	1.13069712490679\\
1.1109080787291	1.96615330191371	1.20299207227131\\
1.171317220047	2.001858577902	1.27624387367332\\
1.23238388325872	2.03815751318162	1.34446825975575\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00001242079505	0.236996152839202	-0.99819153226049\\
-0.934071827168765	0.296812721566474	-0.94900119376642\\
-0.869154732172692	0.344744304962989	-0.900387001894552\\
-0.79642778770078	0.394936458189387	-0.850653752790028\\
-0.724114088376697	0.438060104253512	-0.801718915695451\\
-0.650537362239834	0.485391800508191	-0.747573480286097\\
-0.57773296631891	0.529078210200821	-0.692855667079673\\
-0.504445910849418	0.582120446020019	-0.638795725563779\\
-0.429242111180558	0.633573562556222	-0.581522457967665\\
-0.355596050621327	0.689397248334908	-0.529820957518047\\
-0.277605823264592	0.744025645700843	-0.47633578096978\\
-0.199464303040165	0.801486135250879	-0.41671253912194\\
-0.122780568721429	0.861266032837976	-0.362785688665567\\
-0.0440789177556352	0.915108996921414	-0.311361944494187\\
0.0376143232755785	0.964246304458507	-0.259084321432278\\
0.114555016102637	1.01717209054488	-0.197963055414828\\
0.187652303337601	1.06501729941302	-0.137974963125784\\
0.26584750854522	1.12235537817069	-0.0722826722553435\\
0.342214514737491	1.17232645876298	-0.00694439717821829\\
0.425095419691448	1.23003949135393	0.0603241347804975\\
0.506051039720301	1.28562175609566	0.127239496273135\\
0.588726789046525	1.3455447752446	0.196363111926027\\
0.672750288388868	1.39837087970005	0.266023417678813\\
0.763300391205067	1.4537587327465	0.340530625352004\\
0.845050678727478	1.51670035775515	0.415465343803769\\
0.933384432083729	1.5761458834542	0.491962714885336\\
1.02078988600718	1.63705539115459	0.571323212294579\\
1.10603932995362	1.70225133901559	0.650189837848793\\
1.18831784754637	1.76770875406839	0.733853873662714\\
1.26777717813386	1.82873884287846	0.812237617839167\\
1.34952679680076	1.9049332078562	0.899655597811849\\
1.43023232104486	1.97248192837176	0.982938615477784\\
1.50815864026067	2.03757105632708	1.06420760837613\\
1.59801144846906	2.1096956557521	1.14491569803146\\
1.67678481840977	2.16956626187837	1.224696605501\\
1.75765028520496	2.23070549876961	1.29624968926503\\
1.84149806923614	2.29541484691098	1.37234131875728\\
1.92514715181643	2.37122963631975	1.44830650358269\\
1.9971120621971	2.43906794267888	1.52812329081828\\
2.08444550915334	2.50715141416051	1.60504175661068\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998959593193632	0.240823525972835	-0.999191176356675\\
-0.937010795032799	0.300216708677304	-0.950798757480133\\
-0.87334516007607	0.346598183946491	-0.898595061458361\\
-0.807243845062648	0.395176248501185	-0.846686296870997\\
-0.738726750337258	0.44901308854195	-0.792835340129378\\
-0.674809951292105	0.501516665581982	-0.735094708555018\\
-0.613246013689922	0.565083374984484	-0.683987868051571\\
-0.54891879701058	0.620154772982619	-0.626935790129387\\
-0.494581278850229	0.678818587696362	-0.570675149732432\\
-0.437961561225523	0.736192162727018	-0.510339127697848\\
-0.382006970165087	0.792729988358544	-0.456813446877408\\
-0.324940245612966	0.845608906805838	-0.406925583598001\\
-0.265459355197348	0.901028253007747	-0.358317956109875\\
-0.208780879225109	0.955769508095268	-0.312279004473023\\
-0.148822244643829	1.01457655363819	-0.268603560105727\\
-0.0903744801752249	1.06876803256187	-0.224527404626605\\
-0.0304028315660734	1.1214519565387	-0.178812812022271\\
0.0261867198232864	1.1799634297082	-0.135150437802118\\
0.0842436869465917	1.23110491121767	-0.0898054785672626\\
0.146511414082153	1.281126012722	-0.0454046688802251\\
0.200467321021819	1.32709893484523	-0.00216007815982188\\
0.257103877359511	1.3730911663498	0.0435746712649696\\
0.309144408186614	1.42404195628767	0.0868939116132905\\
0.360342798483346	1.47345591400591	0.134641943185379\\
0.414149720803435	1.5178097101618	0.18064810862728\\
0.472514186448061	1.56764316127003	0.229361709620298\\
0.527780466255169	1.62124292067037	0.283387300713208\\
0.581130005235912	1.66993874378876	0.342200478945902\\
0.634407725475579	1.72488377066727	0.396223324057947\\
0.692139517135441	1.77217418895066	0.454341751580407\\
0.743921075392271	1.82214649284332	0.51454618724282\\
0.79654300926419	1.87985002499337	0.577410328918531\\
0.854115664323511	1.92543174209933	0.644217003467266\\
0.90022435501774	1.96793687696675	0.709619137513361\\
0.966890599445676	2.01567905004838	0.781902994752975\\
1.02199232452066	2.0599629255512	0.849641584649331\\
1.07923862695916	2.10860169005699	0.922623894353172\\
1.13476459690299	2.1487117346492	0.992759550697976\\
1.19308301456914	2.2052443731381	1.06277004046379\\
1.23738648649508	2.25464620386159	1.12787503622771\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997171050210162	0.242309090692241	-0.996856148079034\\
-0.937953212107463	0.291755435391893	-0.950300294838887\\
-0.874338901098554	0.338380256899547	-0.897086027350147\\
-0.809936557705549	0.386072686519136	-0.848017856588324\\
-0.745226017347575	0.428677698644661	-0.794412132155935\\
-0.682260929886819	0.46539293664249	-0.741298955255845\\
-0.614482118094976	0.501047798801286	-0.686561242554906\\
-0.548526305100165	0.542715800119847	-0.631653466289102\\
-0.485189318634579	0.576620933496199	-0.574101718415877\\
-0.422431078751044	0.615974476458091	-0.515009777648744\\
-0.361523563236864	0.654856634204266	-0.456808022333485\\
-0.303253140899515	0.694586018559849	-0.399680829704244\\
-0.246141853522201	0.728963767175671	-0.336187767877396\\
-0.18904891675754	0.767986409842892	-0.277333602911615\\
-0.134219016517722	0.808695614020911	-0.215408219074509\\
-0.0747573033008048	0.843606849702167	-0.156692217518261\\
-0.020439103678019	0.880994131762678	-0.100807855237628\\
0.0308231566903629	0.920606330591664	-0.0416489872792073\\
0.0808987896925517	0.960693259966886	0.0132311483872555\\
0.13503506867386	0.998287652151354	0.0690422961662859\\
0.189121798651164	1.04605663037633	0.126899421908199\\
0.241632307076704	1.09533521782169	0.18321581161012\\
0.289088449535143	1.14818569882429	0.240838878250628\\
0.341635793937148	1.19844786306698	0.298515739981637\\
0.390620499027097	1.2514446960535	0.358623049495604\\
0.44037802866175	1.3057942783143	0.423754115037171\\
0.492366191100857	1.35979320576295	0.487627553340278\\
0.546959208579579	1.41876008517543	0.548116684093643\\
0.604939244749512	1.46904829359612	0.607578124750659\\
0.660573994833797	1.51906110742651	0.670788838088915\\
0.714346576479404	1.56530781521669	0.734290947927073\\
0.773232220495355	1.61769114305016	0.795908073882546\\
0.827056078168975	1.6685483539366	0.865222302470622\\
0.884649168799789	1.71609847453967	0.931142573225979\\
0.94279561381222	1.75541818859283	0.996761328191133\\
1.00365240816101	1.80281039374679	1.0601130003862\\
1.06139464529507	1.84850973278397	1.1218372490159\\
1.11176811346607	1.9064506906578	1.19580671838589\\
1.16752068001643	1.96114731062464	1.26199259438727\\
1.21242801334302	2.01176867289048	1.33151190333676\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99881542207184	0.239720675091591	-0.997009706141376\\
-0.93765438649253	0.293302287911362	-0.950338539456461\\
-0.869224040670987	0.341062677973897	-0.908219846069401\\
-0.802830145121424	0.384962598225273	-0.860089905537413\\
-0.736439119814415	0.428485983725362	-0.810663876648319\\
-0.6720725014157	0.473118919162488	-0.76157666135308\\
-0.60245268510537	0.512837574179635	-0.713395481161917\\
-0.535784511961406	0.553593169948548	-0.669184674280052\\
-0.46943362475402	0.590316720273654	-0.62140876858919\\
-0.405174768763193	0.627116208757717	-0.567639410473795\\
-0.341413477227322	0.658247247352008	-0.511749739559889\\
-0.274952109312681	0.686808168155472	-0.452594442425038\\
-0.212133355944118	0.712822282752146	-0.392052513313729\\
-0.150238256484949	0.747561761275763	-0.33143886344707\\
-0.0880784706303454	0.779728865981586	-0.274808037601344\\
-0.027241009211033	0.812778617646553	-0.217757421531806\\
0.0295094920265874	0.845846977734625	-0.158777798795608\\
0.0844644599779759	0.87003809891487	-0.101148612229172\\
0.136126783426729	0.901627949880876	-0.0450344538206197\\
0.185331432392828	0.934700539268137	0.0137375670675768\\
0.239245711797525	0.970980696186618	0.0698762516650012\\
0.293065230290556	1.00615936608342	0.126745002362658\\
0.3467361272706	1.04080800777651	0.181111997680564\\
0.40050250221656	1.06991908897503	0.243173940796566\\
0.45338491730481	1.10579333147593	0.298056240101713\\
0.505927408420464	1.14584979740738	0.358049174784228\\
0.557187442254682	1.18059088957487	0.419798414594443\\
0.612581072679843	1.21840820756129	0.480505434749133\\
0.668686584045907	1.26003803946999	0.538491828149655\\
0.718193141856078	1.29689957895612	0.598880508895309\\
0.768156830112073	1.33572758034375	0.660334870951474\\
0.823054801709109	1.37014354126151	0.721016806931345\\
0.872970513785764	1.4010853048614	0.778265407102967\\
0.916461767262063	1.42736373941219	0.841438082322793\\
0.9581234247532	1.46346311122217	0.908784035508842\\
1.00940237580738	1.48260922256318	0.977998602327537\\
1.05518353083684	1.50182569737712	1.04318962620448\\
1.10058996882661	1.52886099630075	1.10921458286862\\
1.14632596156738	1.55772619054662	1.17340932362644\\
1.19255061153981	1.5795581201526	1.23465112685251\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997012033215349	0.24330068421086	-0.997794551516377\\
-0.935046798425955	0.298331143526988	-0.948599736134172\\
-0.877277236483502	0.342459339848217	-0.902726415850275\\
-0.814669154167901	0.393082259395234	-0.856981882805012\\
-0.749920772611216	0.437942885646406	-0.807679066289984\\
-0.683661094653007	0.48777849040452	-0.755918285862468\\
-0.615854413113115	0.535417746192292	-0.699236077390068\\
-0.547529425554012	0.585554814945076	-0.646623772223913\\
-0.480691576204443	0.634305277389931	-0.595065014043382\\
-0.419153196352777	0.677119078228366	-0.539491424340906\\
-0.355294414861889	0.721092523051041	-0.486892311783569\\
-0.2908482045041	0.76611903355803	-0.431675315929284\\
-0.223698482560711	0.813334032213213	-0.37485043208904\\
-0.152302963352282	0.858028083916582	-0.32025107240638\\
-0.0841121191825706	0.914284559544938	-0.262546904637881\\
-0.0112241195221479	0.960153916225502	-0.207302417851785\\
0.0611541607231782	1.01720944185419	-0.154038639758797\\
0.130875427844638	1.07857116786437	-0.0947173547830037\\
0.200704812438192	1.13373001560595	-0.0419674127951958\\
0.274121980040014	1.19084234531123	0.00894577875177411\\
0.347242506776232	1.24223765103077	0.0546834713958657\\
0.418169622218477	1.29420207593525	0.0981704153936394\\
0.493912617695954	1.3510320642693	0.142897087055774\\
0.567470216808397	1.41680221662017	0.188926013040699\\
0.642893850621634	1.4797344126437	0.235581895090041\\
0.712250478568749	1.54312912430285	0.277834221027388\\
0.781320156877461	1.60995409592037	0.31834794263671\\
0.851328636946908	1.66759827741845	0.356788027957719\\
0.922317692307335	1.73136632070841	0.394917838158719\\
0.993139273470782	1.79275987572677	0.433501894570389\\
1.06208109058572	1.85260995675399	0.478472772888404\\
1.13085998158348	1.9080268871646	0.526415361146105\\
1.20561838425786	1.96031745717501	0.573650695661233\\
1.27940775815342	2.02909199764573	0.615813676925079\\
1.34812676516791	2.08579132681223	0.662019367126311\\
1.42323235006741	2.15256453372894	0.709438559981014\\
1.50163366840412	2.22009740292004	0.768343110669741\\
1.57865052890917	2.27819189196283	0.825738759724162\\
1.64886201638829	2.3423943225935	0.882816717518549\\
1.71839996723213	2.40376474448927	0.939394887715484\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998176300892813	0.237865833133155	-0.998194406771928\\
-0.937303139918043	0.301206038514602	-0.955159411637351\\
-0.877955500618571	0.341612321654935	-0.901700143340558\\
-0.815697139260197	0.38866548598159	-0.847394338464941\\
-0.754143895367212	0.430870756298495	-0.795036705558929\\
-0.695123827072046	0.47192298746436	-0.740694369683829\\
-0.636612473235756	0.513406346603183	-0.689101644847527\\
-0.575032286854936	0.553967385215815	-0.638111316675945\\
-0.513083470553701	0.595876225786883	-0.587766782640912\\
-0.444961479073543	0.640597481984597	-0.537032591693204\\
-0.375109129653081	0.686710488668791	-0.487021612306725\\
-0.305788006071599	0.738137242989012	-0.436234430769775\\
-0.236235057231604	0.790671883468174	-0.386684809936003\\
-0.166272574417097	0.844525951527236	-0.33937749510591\\
-0.0957488805514085	0.899234206104683	-0.294071544167977\\
-0.0287840323751033	0.947013920874275	-0.251677305336781\\
0.0370096021764849	0.998177322843597	-0.217118878873802\\
0.106559765166078	1.04915798202384	-0.185801895940089\\
0.175524576186528	1.09731864515887	-0.159031018255411\\
0.247090072300033	1.14257724693	-0.130554407973902\\
0.320650086654296	1.18591216187324	-0.0992287650876434\\
0.396506940491463	1.23054750219539	-0.0663487510487194\\
0.473262288155237	1.27090201263435	-0.0358039625641331\\
0.547150548605702	1.32022030747578	-0.00922259580246202\\
0.617612867216872	1.3638636895872	0.0196621500621873\\
0.694060621126363	1.41300564579005	0.0496943384016945\\
0.766817069046539	1.4620538715338	0.0795899787416229\\
0.840694727531361	1.51379585644396	0.107119387534553\\
0.916371968829657	1.55932985424325	0.137390991854598\\
0.986270069766298	1.60614246401446	0.157036274438943\\
1.05994897286179	1.65659647997805	0.177171941443293\\
1.14236102668261	1.70095270256798	0.198267012071467\\
1.22077245933225	1.7449746750989	0.217168008824423\\
1.30174902847641	1.80233641298785	0.236217088454865\\
1.38498294775674	1.84450456804972	0.257150003929835\\
1.46323256195656	1.89905012349442	0.281349483875322\\
1.54165447658842	1.94970008162033	0.299185692966051\\
1.61540358604717	1.9928729763946	0.317860407036865\\
1.69469191291839	2.04210792162139	0.335359285789529\\
1.7690063979206	2.08325071458976	0.348953423649663\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999026809756535	0.240084072736964	-0.997186525363316\\
-0.937873815393769	0.28967113699289	-0.947090346365476\\
-0.876860272021384	0.336162596714522	-0.899783480302242\\
-0.815991866953933	0.374145979761952	-0.845304774590324\\
-0.751994476824377	0.415632959899356	-0.794475312091002\\
-0.686778194362638	0.458797438851635	-0.739701187755375\\
-0.627605385818242	0.503830515606959	-0.68005789915831\\
-0.566547545387096	0.545637617384054	-0.622607224593526\\
-0.503936658596177	0.594855401902417	-0.564993427143466\\
-0.438320011588788	0.642782608333275	-0.504658429485865\\
-0.375478476232125	0.687192464260465	-0.44526305176219\\
-0.308159911482955	0.73004697263157	-0.39000716087015\\
-0.241156607477187	0.777411022254915	-0.336463856328745\\
-0.174061770631356	0.82403155585738	-0.277345976009463\\
-0.10486370531114	0.873540001962725	-0.215885276501215\\
-0.0368351010875903	0.921968606119207	-0.154301419672757\\
0.0352965784408696	0.969923748653492	-0.0985417381874972\\
0.107365650539453	1.01483411074924	-0.0439649237183216\\
0.17852823118301	1.06499157184381	0.0123500405207406\\
0.252988118991231	1.10798188326143	0.0692998063376193\\
0.324674321103164	1.15050947084429	0.121003339138511\\
0.397949577684284	1.19501616192912	0.180555936746498\\
0.473364431316479	1.24268040914959	0.239097947298748\\
0.545629887653631	1.28511754885857	0.29474247897868\\
0.624062823757318	1.33446554971271	0.348368203238439\\
0.696902145321275	1.37974103052407	0.39702875778487\\
0.765864186848373	1.42323863456084	0.448953727889677\\
0.835407573261454	1.47151330209006	0.496716204694803\\
0.911822953534982	1.52218291835479	0.545612252387766\\
0.987355304340101	1.57533580662666	0.597840773942296\\
1.06699119232964	1.62074241684759	0.640775965105837\\
1.1443542979802	1.66500212822931	0.694792355215661\\
1.22386349796091	1.71069188308638	0.740759768098063\\
1.30120078908873	1.75939351204546	0.780265499927767\\
1.38056713543597	1.8047598494121	0.824418111341939\\
1.45858501764373	1.8591800544068	0.867882324642663\\
1.53586213295151	1.90467116231381	0.911349175518199\\
1.61166310691167	1.95393255513782	0.950029641586803\\
1.69261146201018	2.00780060703468	0.993757001465706\\
1.76463446750705	2.05253411494051	1.03503570205977\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997879915141782	0.240723834463188	-0.999168889014659\\
-0.93748846371567	0.29578431763191	-0.949112663857146\\
-0.877506879767706	0.340666471202947	-0.901367203309815\\
-0.81828102223304	0.385778399581687	-0.851568414035801\\
-0.758475161648497	0.41728631044418	-0.790800486192482\\
-0.696758803682568	0.450605705924523	-0.733853644270089\\
-0.63012978521123	0.483857723835722	-0.676504194955924\\
-0.559901449700274	0.51515558376121	-0.620472334296321\\
-0.486488222387591	0.548557895308757	-0.560535094181325\\
-0.414254584382845	0.58645423104225	-0.50402883411144\\
-0.34326554769929	0.620158009652069	-0.444362201889022\\
-0.270252541405304	0.656875971545244	-0.386990669966016\\
-0.196781722409483	0.691933541867233	-0.327018374141601\\
-0.119339712032173	0.728207606773953	-0.270446554979799\\
-0.0392375618379667	0.762284876798912	-0.212516762445096\\
0.0415057536030486	0.804345008496095	-0.157295862094667\\
0.121531736053101	0.844624971425868	-0.0991319209041784\\
0.203639614171569	0.888855805124475	-0.0394044528791185\\
0.289487572404761	0.928857570711002	0.0231126599104726\\
0.376117204545984	0.968847786826805	0.0854360726969179\\
0.465095317817891	1.00740476415502	0.146591123438999\\
0.557493651169457	1.04422051330196	0.203524848471919\\
0.646824089656116	1.0780964891026	0.264323063934983\\
0.742863385230756	1.11676734553909	0.321822907861678\\
0.837293289437147	1.14754467520788	0.378478008567543\\
0.930407683833772	1.18480623858365	0.435963850931195\\
1.02223084245309	1.21310923073638	0.493826434766483\\
1.11237642567779	1.24304141275884	0.552845848946321\\
1.20135571679794	1.27085977331896	0.607994156445073\\
1.28703691402899	1.29764923427642	0.66330445628818\\
1.37928290914193	1.32455573233626	0.723390635976518\\
1.46633572506791	1.34360319370611	0.784467614375736\\
1.55746169070873	1.37249197476557	0.839519989063708\\
1.64768587859859	1.40569684452051	0.896841338311787\\
1.73632235954012	1.43182115355377	0.95415872997896\\
1.83167783360269	1.46284562124802	1.00858384733011\\
1.92885825317725	1.50539079342544	1.06530005971972\\
2.01950827512859	1.53759128973342	1.11422387640636\\
2.10790145732014	1.57350020728463	1.1586601154678\\
2.20074517062483	1.6147083344714	1.21414273416725\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998900049507609	0.23946258346467	-1.00236186302348\\
-0.93806067009773	0.302519151556484	-0.950950613184611\\
-0.875000445130725	0.34699679525257	-0.898855919643974\\
-0.807523332820102	0.399939492504463	-0.851285822771237\\
-0.738732635501012	0.445773708896972	-0.796963483493859\\
-0.669092704552241	0.501131436994574	-0.745389357327111\\
-0.60005637424219	0.548687998038143	-0.69339381968737\\
-0.533763555398126	0.601989143068871	-0.640513674384112\\
-0.466344084745919	0.654606823009821	-0.586634068745826\\
-0.398007404048346	0.710458816879273	-0.538198073873161\\
-0.327189986256386	0.759940545504296	-0.487007320007984\\
-0.257946654787438	0.809827569760894	-0.43996819690865\\
-0.191281519487314	0.861244261710227	-0.390965179810164\\
-0.12319918263032	0.911170938031984	-0.338469896876595\\
-0.0529063399520557	0.960457796370175	-0.284931000275585\\
0.0121370572840651	1.01574173164898	-0.229259852347004\\
0.0765303206470667	1.06787582952735	-0.170580592335158\\
0.143069308250466	1.11454289464276	-0.109509190008538\\
0.213559308238234	1.16392499238551	-0.0477897791321512\\
0.28721610406568	1.20789589857908	0.0114510218586177\\
0.358532529241753	1.25616075697514	0.0722959106392453\\
0.429327405177635	1.30578607630807	0.134477890687541\\
0.497203519831442	1.34870442139244	0.203180353825679\\
0.562254232382814	1.38330899227083	0.272396949975959\\
0.627976942961598	1.42390989812496	0.339621055467874\\
0.692711245350603	1.4621327251151	0.407176703813703\\
0.762052428146664	1.50546194634553	0.471666439366706\\
0.827083674656355	1.54118103022161	0.533528892923807\\
0.890655771335466	1.58813836406917	0.599556143715644\\
0.954075158083042	1.63126448288713	0.663433784543702\\
1.02342161611523	1.6765237438917	0.71983928635955\\
1.08952057837475	1.71923291006883	0.788377876124591\\
1.15523463036122	1.76660637978147	0.848800343627862\\
1.22134094805314	1.80706547855688	0.911423939221318\\
1.29078921686894	1.84387595527152	0.97058517630706\\
1.36389256135558	1.88184790069749	1.0292848380178\\
1.43414786255193	1.91928223170295	1.08661624506537\\
1.505150003754	1.964961398413	1.14547873735732\\
1.58129992660558	2.01361853179068	1.20726886686901\\
1.65858077122085	2.04374268460611	1.26623010975458\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998224655000947	0.239227642880987	-0.999584344680839\\
-0.938183365774556	0.296710244772038	-0.946828230357148\\
-0.879421108616024	0.342070775244995	-0.900653004904123\\
-0.82166056995277	0.388358721989544	-0.848728249590131\\
-0.758672746177095	0.437676404337165	-0.788815227408785\\
-0.696234678416448	0.483323644158982	-0.729668316975941\\
-0.630062237071506	0.526957723359955	-0.667599634269856\\
-0.56084383392734	0.573351786524257	-0.607117278261738\\
-0.494568391194088	0.623461572408495	-0.543282847000905\\
-0.430201062649796	0.67302141323129	-0.487191414986097\\
-0.365669219281314	0.710817066887927	-0.429540589155897\\
-0.301635764688841	0.757472276670488	-0.374631948451446\\
-0.238711485346451	0.794631524275093	-0.317800635707675\\
-0.176862364651176	0.832099208634916	-0.263700362004811\\
-0.113587870139848	0.871146482061936	-0.205391907212626\\
-0.052673869772478	0.906205089617722	-0.144114067397178\\
0.00804271305616219	0.948575148488696	-0.0829298377588602\\
0.0674849271209098	0.982415880306125	-0.0180213627134236\\
0.128903075544697	1.01730880235047	0.0530535798275169\\
0.190907749431681	1.04886893016138	0.121320853201782\\
0.252379156510826	1.08621983747133	0.193804436751609\\
0.315139499419469	1.12452651095244	0.26797162831777\\
0.378953618905509	1.15149262954047	0.340684298480034\\
0.442835878587877	1.18590449879145	0.416311108173326\\
0.505513346867512	1.2138013079254	0.484497381543919\\
0.566919430330379	1.24261920680413	0.555585856389909\\
0.631971287720878	1.27395118423471	0.631424174361061\\
0.693379736982473	1.30330890834518	0.706850974285168\\
0.753057309240758	1.33605743490273	0.779416091847091\\
0.816047411858848	1.36629210562833	0.853668317339531\\
0.884083930531003	1.40540869704547	0.926000431825431\\
0.947072681365749	1.43618280163544	1.00001698100536\\
1.00663420203886	1.47123221470779	1.07640235977588\\
1.0691447990303	1.5009622286756	1.15093479724517\\
1.12606186973462	1.5446864200095	1.22701164262742\\
1.17974472675541	1.58769448825149	1.30355404511283\\
1.2329264835621	1.62665571917759	1.37577149928208\\
1.28210258936641	1.66271999651647	1.44977142231725\\
1.33055578649617	1.7028061616776	1.52665462199228\\
1.37903574812156	1.74629378364962	1.60168294795199\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00068039801429	0.240653644756187	-0.999024335894011\\
-0.937253295640987	0.300747056284595	-0.948466637951207\\
-0.873652877040978	0.338650004030541	-0.895336306301265\\
-0.808113604720478	0.388253193978652	-0.841404607716261\\
-0.743978307833414	0.436430858469606	-0.788134022778441\\
-0.682478371160331	0.490718587451654	-0.737315538042155\\
-0.620992286937752	0.5365139577963	-0.68702622812266\\
-0.559126266454237	0.586339083846549	-0.638445314630722\\
-0.494960379644859	0.633528757751934	-0.589898566209941\\
-0.428543946918859	0.683150244550394	-0.542683692201893\\
-0.362373878711569	0.73042517132893	-0.492837526232333\\
-0.292264814548535	0.778709195805616	-0.443338481202199\\
-0.222913209015542	0.818688459852304	-0.39347693392683\\
-0.151905178353261	0.855789346155398	-0.347375085952224\\
-0.0786397332109598	0.893602641023956	-0.298894449829859\\
-0.0083435986758045	0.933263829790044	-0.255519614643458\\
0.0692654400206779	0.972730838622875	-0.207740520051098\\
0.143898911173719	1.00587304301728	-0.157196654923438\\
0.224904696508977	1.03794175311786	-0.110746295232362\\
0.308109665172005	1.07450635599904	-0.0650790587178632\\
0.391693928912089	1.10759844889851	-0.016851449573118\\
0.475247228923485	1.14339743846377	0.0330466799342419\\
0.558987369576932	1.1779462152993	0.0877520837481897\\
0.641236597108186	1.21279989619249	0.139539230690144\\
0.730327880690867	1.24736327756213	0.196787522417735\\
0.818403581360737	1.27869592800771	0.254486754886065\\
0.911133894349329	1.32304172617135	0.311510344469394\\
1.00196265849277	1.36857489729479	0.363292126884496\\
1.08499303940429	1.41039054155304	0.416193982274278\\
1.17357355895132	1.45437433853469	0.465193744115268\\
1.27108916573045	1.49585615817136	0.511198188920007\\
1.36738815203217	1.5288777946603	0.559249988865571\\
1.46459792584918	1.57099099022238	0.60704842066653\\
1.56212782255143	1.61255482846046	0.657140249559243\\
1.65101905229456	1.64009040659743	0.697355172143784\\
1.73689753157938	1.68738904946681	0.743162119241309\\
1.83612693015357	1.72298066468903	0.788077066694301\\
1.93577383028603	1.7571649821941	0.834936806521095\\
2.03580061539425	1.79740284902888	0.871827160397645\\
2.14640774918638	1.82927946907133	0.91891253168607\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00078365475287	0.23992355535741	-0.999728671012028\\
-0.935891642953166	0.300091825089731	-0.951474389462341\\
-0.87418466838095	0.346093476197099	-0.909218351198902\\
-0.812655596659914	0.38997905399921	-0.866003938379414\\
-0.752169420156563	0.43787424959484	-0.822649289058851\\
-0.693160374216775	0.485257210769055	-0.783997105360234\\
-0.633899961413753	0.536927934143049	-0.750349007416267\\
-0.578063148420872	0.585347426857786	-0.713390213594638\\
-0.522336889168724	0.633788617358528	-0.680267083935142\\
-0.466170272683795	0.679281679845899	-0.648519521131764\\
-0.413201259798065	0.729604239953143	-0.61380063664545\\
-0.356193498793296	0.777507316190032	-0.577618642803768\\
-0.300237980555567	0.824550367130647	-0.539948180551264\\
-0.239572284860228	0.872342499049926	-0.501372323047942\\
-0.180259819052109	0.922921441578816	-0.462921887665123\\
-0.121082899804986	0.974075155469182	-0.427164662472606\\
-0.0596028969316553	1.02779599155048	-0.389515978863963\\
0.00501546932763867	1.07894707697658	-0.348259722788119\\
0.0710579821881429	1.13287548301642	-0.309723734836253\\
0.14031608034427	1.18204009515857	-0.272939079172506\\
0.201524037587837	1.22856440719882	-0.238853614006538\\
0.263305609475994	1.2749900556921	-0.205138519084251\\
0.32685918959988	1.32175041691463	-0.173873034309376\\
0.391412762787077	1.3758752709622	-0.14299065739635\\
0.452820392377637	1.42970299149503	-0.115271006907894\\
0.517680455999868	1.47537224732817	-0.0883101602986723\\
0.579419045623243	1.53030767951344	-0.0581559539972585\\
0.637925300760748	1.5806756508248	-0.0350750467162361\\
0.695185422632207	1.63571118302487	-0.00440397548219863\\
0.756929900314464	1.69009717857704	0.0185571639265925\\
0.815811620634022	1.75058499785149	0.042499890303336\\
0.870765183520883	1.80180156512811	0.064911783031098\\
0.928885152338001	1.84612847431331	0.0876981845852584\\
0.989320626855028	1.90289284182915	0.104575673815243\\
1.04275871276515	1.96252053390895	0.120934328141935\\
1.09530686760527	2.02619255868345	0.1387665029957\\
1.15094350015327	2.09891026242926	0.154727215184451\\
1.20222732319365	2.16430494030975	0.169206799873526\\
1.2573556028871	2.22674555926012	0.181193062032712\\
1.31218258441105	2.28963419120086	0.191422453652016\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997765059396343	0.239368119619885	-0.998632467358541\\
-0.93937373323242	0.30214329108609	-0.949185409875145\\
-0.875430882826985	0.348818635030752	-0.899319098786669\\
-0.814920588751239	0.390444458877849	-0.849219374066013\\
-0.756449272533883	0.434456193704606	-0.804731821703027\\
-0.697587230861426	0.479936607372494	-0.758398834170475\\
-0.639413273211574	0.532570180522667	-0.716201607484398\\
-0.583250669876915	0.580930796622951	-0.66750582265269\\
-0.527361234888502	0.625535916742555	-0.619366080362518\\
-0.473860540054439	0.675138429741735	-0.573455403431676\\
-0.416842602137691	0.718787849718638	-0.526531922360328\\
-0.355517228729186	0.761941008670046	-0.481906741047513\\
-0.29924429795684	0.797860286506303	-0.43411365788437\\
-0.241579316760711	0.842665495279437	-0.38576965554492\\
-0.186214436407172	0.884510695935943	-0.33955466820198\\
-0.131472460259029	0.922322507515103	-0.291391040471825\\
-0.0818283018778097	0.965781306244273	-0.243710623772155\\
-0.0289450444715565	1.01362678155263	-0.196341134494746\\
0.0192766868295891	1.06065271318524	-0.147124525310489\\
0.0663651930763715	1.10930768509397	-0.095297947451749\\
0.117825522326872	1.15754189666042	-0.0483557043478084\\
0.164682153080368	1.20379487712617	-0.00279573383468452\\
0.211010479540805	1.25258364544966	0.0411455465734933\\
0.255594040030545	1.30692149575259	0.0922078762991131\\
0.298254564870538	1.35645848800623	0.142000608966418\\
0.342873876235389	1.40253907038574	0.189173183692991\\
0.392926276047407	1.4486794048328	0.23175092839643\\
0.43680424289492	1.48816583448801	0.276156170773253\\
0.4807378215762	1.53137364047456	0.322775513737631\\
0.526620198531542	1.56920228882126	0.359127831373691\\
0.56591489672637	1.61693229148691	0.404238742203233\\
0.610099917813616	1.65270722008485	0.447338321696072\\
0.652502599965383	1.69384746474384	0.485782584780267\\
0.700410178129929	1.73198556856864	0.52402903078929\\
0.752113576201318	1.76889797773974	0.565405797293733\\
0.801923949775538	1.80660358681109	0.605765402145737\\
0.857822291965766	1.84933557779032	0.644559486875519\\
0.914588074077971	1.88384810618892	0.689810740450099\\
0.961631798383387	1.92606158107412	0.731858711330456\\
1.0148826543844	1.96115444333319	0.774784027441618\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00124092589185	0.239816003778784	-0.998979463466204\\
-0.937288483883964	0.298652216485728	-0.947305080414681\\
-0.874324015956683	0.346679988346124	-0.895911654551714\\
-0.813086423541777	0.396488056541292	-0.843166313898894\\
-0.751010436713365	0.446269804704144	-0.78817970307042\\
-0.682882612520197	0.493528138625298	-0.736862023324279\\
-0.613861780293297	0.545395910931668	-0.682527468420955\\
-0.538838020915168	0.590867343909261	-0.625300948241179\\
-0.466039239828263	0.641714009902162	-0.569903590745812\\
-0.398667635275314	0.69222350235383	-0.520227774555629\\
-0.330008627457289	0.747162137589701	-0.46170774691253\\
-0.260499094905648	0.801375354698887	-0.40616405740866\\
-0.186767739138402	0.856294633077699	-0.351163497386381\\
-0.111019062347564	0.908056769338158	-0.294500064696019\\
-0.0350835522365496	0.958857705356086	-0.240772170645303\\
0.0426463628396927	1.0186034213848	-0.190925113936523\\
0.11791103936777	1.0705704139845	-0.141053473742598\\
0.197839296599261	1.12843363279935	-0.0872794812274623\\
0.277347790307844	1.1823768445215	-0.0310909748515738\\
0.360988620334964	1.23250037248435	0.026051780568783\\
0.438124102287111	1.27967137325163	0.0790201668357556\\
0.515206366190743	1.33008348979629	0.129780283140996\\
0.599816880653003	1.38299679982594	0.182631115781806\\
0.678888828794389	1.43166401753439	0.234165040762675\\
0.758029893448463	1.48160154547055	0.286636606059209\\
0.841015536434754	1.52993908396869	0.336523085378486\\
0.924889234355651	1.581273031991	0.381659253479001\\
1.00387249973436	1.62711092001131	0.425831594133192\\
1.08168968192146	1.67569786099973	0.463410534659372\\
1.16164203108494	1.72351386188058	0.504984800696315\\
1.23737000582405	1.77232198652142	0.549479689877577\\
1.31104377052331	1.82690193330057	0.595304293111153\\
1.38668724076	1.87766090010812	0.632646767553519\\
1.46437653667485	1.92354642765666	0.674047007503459\\
1.54456738776447	1.97765707938978	0.710337580898264\\
1.62013027426845	2.02878200653533	0.745168892467828\\
1.70279727725444	2.08362349291647	0.787683450570283\\
1.78568175922823	2.13599486884661	0.819525740697244\\
1.87154876593784	2.19139625223957	0.863728576209412\\
1.94806169574255	2.24685221306749	0.907639684684533\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99935194721902	0.238681935338578	-0.998614880487704\\
-0.940335836971935	0.294976492649077	-0.948870499024057\\
-0.874908791475569	0.341477802018139	-0.896921152791689\\
-0.812388641867099	0.385690279888144	-0.844281874115211\\
-0.750864214281315	0.429173650735838	-0.792088891824479\\
-0.690905511463685	0.464874821347287	-0.740351533534099\\
-0.631977740516516	0.503337534656834	-0.685425691263554\\
-0.571132209431751	0.54134772890941	-0.631745062895502\\
-0.507316451248349	0.579404089114587	-0.579542816811058\\
-0.441180989267618	0.615904911165074	-0.528489391519457\\
-0.372345206888199	0.650356337398777	-0.47468554690201\\
-0.3042245244206	0.688509812480207	-0.425825793298077\\
-0.234662626611892	0.72125536451384	-0.375200019770466\\
-0.163090084788497	0.760131401500791	-0.326837971516642\\
-0.0893268737884853	0.791805202790887	-0.279677400815967\\
-0.0183310397317188	0.838870042194565	-0.230546207273301\\
0.0587946373017586	0.879888778294201	-0.187346580087519\\
0.129542188948448	0.928790274326802	-0.146944594367335\\
0.19870398092916	0.97008979090525	-0.106744648497142\\
0.268992986614762	1.00845715728851	-0.0587876227145755\\
0.342444831359641	1.05597310529209	-0.016633186444905\\
0.416066471449191	1.1013404563555	0.0303418665508237\\
0.493292186449519	1.14913228388169	0.0724549004087658\\
0.565144821047364	1.19875654035141	0.120335642148666\\
0.631988359088721	1.24445046761545	0.164866528774112\\
0.699383810166387	1.29010785268828	0.207833740504836\\
0.766648989026749	1.34489441145531	0.248559227784297\\
0.833580294365854	1.39385174978063	0.297406458174374\\
0.901497318434043	1.43850835907576	0.346483250157958\\
0.966442046604626	1.48763067637605	0.392314535904749\\
1.03047451970741	1.53159672115588	0.440687899918605\\
1.09051333003387	1.57761600039227	0.485585283586414\\
1.15272401877982	1.61953124886624	0.534540816773247\\
1.21364671499112	1.66189468245294	0.57786534400908\\
1.27806458218462	1.71141740171944	0.618109534977801\\
1.33858492863642	1.75846661187408	0.665612352640433\\
1.40684406280712	1.80841245433489	0.704197487856624\\
1.47287973581568	1.85293521433314	0.749909007172522\\
1.5436681275598	1.89714042979675	0.793034464721989\\
1.61550488564297	1.94724852083146	0.834530127630623\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999634859621356	0.239271779481475	-0.998679462684257\\
-0.936111764381054	0.296283614453489	-0.94831683958489\\
-0.879129763640786	0.344920328813215	-0.89736794283437\\
-0.820567957889284	0.392716186502721	-0.844863550836345\\
-0.765485602045061	0.443495726580834	-0.789972709196182\\
-0.71005856716443	0.497655503148952	-0.732126627113771\\
-0.659365634265378	0.550808457412839	-0.676819882311723\\
-0.604592497605471	0.606490147647145	-0.621946983750836\\
-0.55054846969073	0.651072972043645	-0.564630384875968\\
-0.499489541386082	0.699347844936272	-0.507702707992726\\
-0.446330041569933	0.7502738321523	-0.450930613005345\\
-0.396044907406805	0.798113391378133	-0.391029921300544\\
-0.338611297900659	0.849822383643951	-0.331618714582251\\
-0.280690737471354	0.894578984122785	-0.270568912008518\\
-0.224711941751689	0.93849644601338	-0.209683058849851\\
-0.16892685369019	0.986275482886221	-0.155018792153008\\
-0.111134990825546	1.02559974484507	-0.100499468719658\\
-0.0549752908328018	1.06320527674927	-0.0456769296444546\\
-0.000977872683983087	1.09666252849073	0.010302887012338\\
0.0557587964780432	1.13781354447212	0.0607750484519258\\
0.116110577061856	1.17545485565356	0.115959218816399\\
0.175691679666404	1.20992923955523	0.161901311504316\\
0.232748765770166	1.24716034135514	0.210486992358668\\
0.292881897898659	1.28045142232902	0.257209720815239\\
0.351400916583728	1.31226386929515	0.305560539142629\\
0.407759025047308	1.34674089736457	0.353242150936268\\
0.464362193982513	1.38289946352213	0.40354352753329\\
0.519806515232579	1.41766533333554	0.450756754805817\\
0.579791581474152	1.45298806998336	0.49982899465621\\
0.630330461225914	1.48939798469553	0.548791834620117\\
0.680207559994775	1.52433116639941	0.590702092131388\\
0.732210593375266	1.56916542552337	0.64101786961329\\
0.782830371440488	1.60933724902005	0.688040626190246\\
0.835222882756387	1.64714827145702	0.742395842277165\\
0.879167065106617	1.6908307056549	0.787836221186975\\
0.922554779812626	1.73442902138144	0.835343280017121\\
0.968229202375749	1.7800803062225	0.875578095160023\\
1.00468409432214	1.82122244587443	0.920233266083355\\
1.04954752099087	1.86385882139071	0.972889979690468\\
1.09424933934566	1.90572203463849	1.01571907640299\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998820335376772	0.238921318243581	-0.996969581059155\\
-0.937071634582295	0.295140179291052	-0.943756993473794\\
-0.876139596659584	0.344939806167525	-0.897342204977664\\
-0.813721266783148	0.397691538934039	-0.841597462365402\\
-0.748021699902443	0.445484609128519	-0.78301767507068\\
-0.685043459105533	0.499721975901537	-0.73103355466423\\
-0.618842846105844	0.547120151214652	-0.677477946235264\\
-0.546844142562826	0.587095564076127	-0.623561101067313\\
-0.46823195206458	0.632124148862021	-0.571199447699018\\
-0.395515238202973	0.675072970046032	-0.520880772337115\\
-0.319938529664889	0.713615139425768	-0.465927183386198\\
-0.243211956264313	0.752923796959993	-0.410387217377009\\
-0.168155245938329	0.790597964672429	-0.354645879879868\\
-0.0958117218807896	0.829815104746962	-0.301180641105088\\
-0.0259715780474841	0.860550878588039	-0.246873953464595\\
0.0421023788172709	0.904274596508869	-0.195717790601222\\
0.113715180511701	0.951859870071415	-0.141406863864737\\
0.184706948439921	0.997536369595875	-0.091462727889696\\
0.249250946848064	1.04057469957017	-0.0424766261122953\\
0.320079487574856	1.08890931768402	0.0106434234306132\\
0.392174896817315	1.13407108515269	0.0610073539818095\\
0.457136971874876	1.17454222116694	0.112058158005418\\
0.519428042632615	1.22245260767292	0.160549911540699\\
0.584663574066972	1.2627042345698	0.209544686831594\\
0.649822494004643	1.32118306801154	0.26012615385116\\
0.719907162719835	1.36934072698426	0.307409175359373\\
0.78338103065916	1.41597416906786	0.356188806277736\\
0.847678004201852	1.46567996380167	0.406173497391645\\
0.913221152014442	1.5151702694116	0.460843008360163\\
0.98030984083085	1.55695937707148	0.517205072955565\\
1.03952857790341	1.60332881896411	0.571317714147402\\
1.09798755174183	1.65011344344005	0.625106222583626\\
1.1643635454599	1.69280340409992	0.676078149923056\\
1.22877548910632	1.7465278474927	0.734725491744017\\
1.29305008212906	1.79291020122233	0.784666086452308\\
1.36131578464863	1.85129472235578	0.837823693033084\\
1.42229886754359	1.90412508397255	0.884608592598434\\
1.49063846924171	1.9581272450955	0.931869184869564\\
1.56626535556546	2.02545736600662	0.976794527451747\\
1.63564991973717	2.07397037829095	1.02263920234139\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998141641676941	0.240967974914197	-1.00104573129492\\
-0.940289965417701	0.296436333508483	-0.951756290257576\\
-0.880642106735884	0.346193713113848	-0.90194032523838\\
-0.823903869886611	0.394281991098614	-0.848688414968544\\
-0.774515055117073	0.44663042020815	-0.795615391257305\\
-0.718953555876818	0.493396837258269	-0.743592861836015\\
-0.663014760487011	0.540758853407822	-0.691942101793505\\
-0.604643703120425	0.584821925667062	-0.643936819934352\\
-0.551142793187199	0.635150151318448	-0.599578378844916\\
-0.493137791939963	0.678849867648144	-0.552117599593888\\
-0.438176982506915	0.724377433661882	-0.502596057358096\\
-0.381608546230655	0.766878362948332	-0.449712819452601\\
-0.324235174831834	0.806449695532166	-0.399555125349189\\
-0.264110604083804	0.850979232727021	-0.350140378946814\\
-0.206512661124915	0.894379517090073	-0.301081461622054\\
-0.154237726861326	0.941430839990925	-0.250857608285135\\
-0.10086694970637	0.98442856337781	-0.201758719189176\\
-0.0459965825642973	1.03030334795318	-0.152779607595599\\
0.0108273687164005	1.07162883151285	-0.108031767186483\\
0.0630459839546758	1.12172448432462	-0.0640373791277421\\
0.114140364546358	1.16516459074779	-0.0185712643445556\\
0.167483057058572	1.21027796183965	0.0260149100624995\\
0.22499017885151	1.26023140779112	0.0689347587561598\\
0.275815418455338	1.30780796524357	0.112388677324613\\
0.329024379692852	1.35324196944629	0.15361027360572\\
0.38405613968104	1.39732267347827	0.192652958101126\\
0.440666272778179	1.44568166461066	0.23004812488495\\
0.497406879657085	1.49283470924521	0.275313496475246\\
0.559461237584241	1.5377608107421	0.31895704973692\\
0.623380174570776	1.58877975853588	0.360598797189408\\
0.693562409807554	1.62522930427611	0.403593824844869\\
0.765342611122525	1.66695834452229	0.44944560983481\\
0.83752062084654	1.71001844620491	0.494724077995049\\
0.908406001396094	1.75106936413118	0.55064618493569\\
0.983922390329083	1.78547007538123	0.597413206791784\\
1.05826693551764	1.82043870407701	0.655931597015267\\
1.13113499572271	1.85605619904299	0.708403706593457\\
1.20619129348005	1.88540233292976	0.755280510916421\\
1.28143016981168	1.91792636176267	0.811799247013876\\
1.3578558127962	1.94481149689388	0.868215907014479\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999379532098069	0.241223723327276	-0.999920084408998\\
-0.93492165331174	0.295914305409757	-0.946124244297636\\
-0.874994082955451	0.343031763381411	-0.894850305142999\\
-0.809094593462341	0.385981203187363	-0.841311767072062\\
-0.750513715131491	0.435396407421481	-0.789834135005093\\
-0.687586902390309	0.480360499957345	-0.736112328938023\\
-0.632691069686544	0.526903928045293	-0.681665340098762\\
-0.577944258981679	0.572691468807821	-0.626757505663241\\
-0.525543804283991	0.618660045578255	-0.57429801599278\\
-0.473354545274657	0.664572066760024	-0.518335892726232\\
-0.416061773757111	0.71889625048144	-0.461207246992515\\
-0.357857832172204	0.765455440821941	-0.3978378972767\\
-0.302274939986316	0.816627044511738	-0.335877313033306\\
-0.247947521476374	0.862266087482545	-0.275042145613876\\
-0.199879405995406	0.904374457595352	-0.216176381583011\\
-0.156466604454471	0.945687096831013	-0.154985257768373\\
-0.112194634728078	0.992549864846286	-0.0905928258134019\\
-0.0691812259949483	1.03655867008954	-0.0319964039603638\\
-0.0231554325911002	1.07949726980244	0.0243611132704072\\
0.025900862016675	1.12645333379324	0.0791319056483098\\
0.0718501885869285	1.16993008852809	0.136942515132676\\
0.119671273213875	1.21654756500959	0.19367263401488\\
0.168020561329555	1.25850470482246	0.244341762240554\\
0.21802461144304	1.30164387328126	0.304327430250959\\
0.270951950541524	1.34508155835582	0.357294114281204\\
0.321030143896179	1.39422266287677	0.409521576158534\\
0.377994998122363	1.43741189245949	0.461461115991604\\
0.435859567248624	1.48389534083306	0.514845197059223\\
0.496265467782873	1.53040445464621	0.565186714389318\\
0.556299039976345	1.58255010062908	0.615363436602804\\
0.617047681951464	1.63552058297951	0.669227994220004\\
0.680907093515907	1.6872794052462	0.719695355352909\\
0.742044735390273	1.7413481484156	0.76984166661847\\
0.802018594842547	1.79214191244091	0.820403165860948\\
0.859282127973218	1.84274059100774	0.872457664819439\\
0.916853818852517	1.89879759749512	0.931304340332778\\
0.975616134558948	1.9593164400295	0.987942311220517\\
1.02881600198417	2.02219584921213	1.04481651384734\\
1.0832693049385	2.08176642178776	1.09728417561781\\
1.13277286916824	2.14841003268375	1.15596800117175\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999692310620872	0.239927674033235	-0.999472432615463\\
-0.933209819728707	0.294748472255955	-0.952261281905421\\
-0.868577711023995	0.335765656725296	-0.904340802739909\\
-0.799092069724105	0.377827820415651	-0.853678993657259\\
-0.727332144761213	0.422970624041353	-0.807275525685005\\
-0.655851728054118	0.473916580110526	-0.75888187800323\\
-0.587001768519097	0.520084917967592	-0.707430624155749\\
-0.515955211025173	0.567453846966708	-0.656195506366815\\
-0.446198405426685	0.612821995961846	-0.605449946997307\\
-0.373250218732531	0.65216923049297	-0.554816287316858\\
-0.299296176120974	0.690687677149231	-0.501713936178241\\
-0.223971979258598	0.729535119464636	-0.449265513717634\\
-0.152145543292195	0.762859695512808	-0.393640208907787\\
-0.077939023765532	0.792386590549032	-0.334102158390686\\
-0.00772147692959863	0.820768415406884	-0.276871959717681\\
0.0610432880036605	0.845364995915679	-0.214686061882883\\
0.129184138865217	0.869133626882791	-0.159136365829675\\
0.197104110175878	0.898505083067777	-0.105594134850437\\
0.263868304657298	0.92054046392094	-0.0480516806394047\\
0.333409676023692	0.947021412351271	0.00319140706745683\\
0.403062971142568	0.970883716135543	0.0584373869445038\\
0.475682004816493	0.995920020940746	0.11412895053286\\
0.5449443372319	1.01752848431982	0.163525375301499\\
0.610392438290691	1.03998945592692	0.216423960829373\\
0.674330360522012	1.06938989168373	0.271322847711803\\
0.738445814596909	1.09437680542196	0.328401356808452\\
0.801823353084034	1.11926185706369	0.381847195154675\\
0.864314845733103	1.14190470530954	0.438691398473727\\
0.920222809590428	1.16666620393811	0.485574912785679\\
0.977558104172646	1.19310145446199	0.534438156242062\\
1.03463157503337	1.21726284661055	0.580998946992507\\
1.08685230105948	1.23856160545643	0.627852252630681\\
1.13793081805297	1.2593147644309	0.677243817230983\\
1.19545577295665	1.27798699002787	0.728361159733363\\
1.24754004030227	1.30250091317863	0.776440145446456\\
1.30191549833444	1.31824391475217	0.821097606228413\\
1.3575995649498	1.34538921661929	0.86869134821583\\
1.40889647097055	1.37273800670513	0.914263774778509\\
1.46259078616865	1.39435947213133	0.958178684058967\\
1.5196290196583	1.41998842495514	0.99970630630871\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.0008872540537	0.241432926064298	-0.996633556315726\\
-0.937172206737194	0.303169074359908	-0.953146360197932\\
-0.877023053451693	0.345234437205845	-0.905475789191137\\
-0.811349230914318	0.393087850027326	-0.857675931327085\\
-0.748557536889076	0.43950763832727	-0.807468564276365\\
-0.690821605453801	0.49064589322845	-0.757118489027448\\
-0.631296132199868	0.538810205812094	-0.707828558577903\\
-0.571461507142488	0.585759839128613	-0.661269483166922\\
-0.513408007728163	0.6381450439303	-0.610789885088859\\
-0.455146235541629	0.688970344751322	-0.55923029660364\\
-0.401220864936343	0.745194904194207	-0.512607935279978\\
-0.342709330464797	0.798349645315461	-0.463116163216725\\
-0.282164833815141	0.856037033053808	-0.41532914635638\\
-0.222468242143816	0.917796548686238	-0.361975760192633\\
-0.165045956534996	0.981677973042248	-0.309740304771138\\
-0.108364342811272	1.04652973304131	-0.257534753134524\\
-0.0587552517817292	1.11217382389008	-0.206808854252477\\
-0.00200931185334325	1.17737973156386	-0.155243031753258\\
0.0562196644555416	1.24351072637553	-0.100664547768488\\
0.114940699105903	1.30766965566372	-0.0488840862162478\\
0.170919506281538	1.37229158082352	0.00453343930163976\\
0.226041481777202	1.44372672196622	0.0567280100758777\\
0.282446284908058	1.50867484967037	0.110299882473515\\
0.340083934919905	1.57077561906573	0.161165948861961\\
0.390407734954244	1.64136285524902	0.206372763361386\\
0.445499308068681	1.71892544365508	0.255642234222136\\
0.498051206182195	1.79675195542776	0.306691133636599\\
0.551553624648943	1.87939959894694	0.353772234579832\\
0.601596043468437	1.95851317361973	0.403985923034679\\
0.65806362583231	2.04401454564946	0.452116753343756\\
0.709241154377718	2.12176029890201	0.506249261000002\\
0.755720320081895	2.20270713280254	0.554394415598567\\
0.800217191516422	2.29846251561385	0.602512599047508\\
0.852456529453143	2.37994727284175	0.654591488133874\\
0.894773629436084	2.45194429646527	0.712713921456089\\
0.940881650942463	2.5302859323334	0.758885602116381\\
0.985561789341494	2.60697507286057	0.807825988608978\\
1.02382142933863	2.67772575072283	0.853294196716483\\
1.06953942346816	2.75370739644224	0.901880082748034\\
1.12365698166703	2.83573277421499	0.944352229336189\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00082743567633	0.238885170251025	-0.996206865027175\\
-0.940817417922833	0.296881056563082	-0.948557069637876\\
-0.881878366995346	0.35101660361673	-0.897637455255167\\
-0.819402456815038	0.400725296794156	-0.842970874700834\\
-0.758599621810355	0.455218953359551	-0.782301494425766\\
-0.698250709671254	0.516697996269605	-0.724683641260743\\
-0.642195280607129	0.574935395397737	-0.660382756763835\\
-0.591977079946194	0.635209516502012	-0.596605906885547\\
-0.540601864243441	0.701893624195876	-0.534844301705328\\
-0.48334891784124	0.764034702508068	-0.471390740652786\\
-0.429295032459792	0.827783704820473	-0.407844601893901\\
-0.373027477484754	0.899178055716306	-0.347857776586655\\
-0.319733916661838	0.966387419444043	-0.285557069314635\\
-0.268251566022367	1.02707986125062	-0.22193314363696\\
-0.221575564879888	1.09072701171127	-0.160646300653345\\
-0.167831926242652	1.14869201584876	-0.0979971288513163\\
-0.114306874366952	1.21188288584621	-0.039256381790911\\
-0.0568484378683423	1.27135149170009	0.0208765077156277\\
-0.00269477784702398	1.33240485248897	0.0767110264607232\\
0.0553665454390656	1.39401571314772	0.130330605519855\\
0.102977587419805	1.44898789224728	0.183197551203754\\
0.15567900311223	1.50842486891107	0.235722722361896\\
0.207823061891058	1.56571513228968	0.28555200706942\\
0.255135614146583	1.61638481097362	0.337960088325288\\
0.304790259240445	1.67414838607076	0.384614022381312\\
0.355903086354957	1.73159358461473	0.439592646541742\\
0.406634016269651	1.7868743930437	0.491809721004599\\
0.460914263153398	1.8343807011135	0.543374422784016\\
0.511542861930725	1.88494950697514	0.592598079622089\\
0.565263290721416	1.93961102731021	0.646332373128015\\
0.616981555691952	1.99077201622695	0.702819101503462\\
0.671197567301063	2.04015319134609	0.760803284275124\\
0.726075240116637	2.10650310794462	0.81718418991772\\
0.783255221024317	2.16623585687345	0.865259934274922\\
0.853000676037957	2.22763775186827	0.917531008264735\\
0.913478824212786	2.29682918743265	0.966696296980674\\
0.969452970558019	2.36517560733474	1.02015598397779\\
1.02946830395265	2.4281140161147	1.0748752797848\\
1.09250649588298	2.49312186411354	1.13649164958425\\
1.14801020465013	2.55986789988781	1.19054503258881\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00008317066648	0.242834635470484	-0.999899041095014\\
-0.939346175301803	0.296314821407122	-0.949410557679027\\
-0.880099002568571	0.343752438190296	-0.906356273050507\\
-0.824651746555369	0.391426348091208	-0.859385172836208\\
-0.771442787411484	0.437491768170075	-0.813425413378958\\
-0.714945218902297	0.485506554465226	-0.766641089437531\\
-0.662834128060215	0.534399092098705	-0.716416013327529\\
-0.608251504078102	0.584689137110478	-0.662707721076069\\
-0.554193738412495	0.631881020127409	-0.610628535553922\\
-0.500856522659415	0.673592449757168	-0.557450907962817\\
-0.446866294993415	0.723393243569409	-0.508738522550848\\
-0.392892391536904	0.770496439283146	-0.464306520964812\\
-0.333205082199676	0.82227573006045	-0.41442530380006\\
-0.276525099730795	0.873340341902548	-0.362061970649051\\
-0.223084849807473	0.92940436471091	-0.311476610522187\\
-0.168194829036812	0.98411040994248	-0.256843284268853\\
-0.107695320415129	1.04428466753511	-0.203963361014592\\
-0.0511222109411478	1.1030549491784	-0.157362670295097\\
0.00767296756030962	1.15454670598118	-0.108365094141501\\
0.0652733523734312	1.20667399690555	-0.0580264467290626\\
0.124304356030193	1.25576257928068	-0.00255882061443522\\
0.184480909991661	1.30970698496415	0.0576169470209865\\
0.248308933665813	1.35810446897833	0.119255205753347\\
0.312381494076611	1.41291239064518	0.184709998448736\\
0.375793362004162	1.45854951669542	0.249077833742865\\
0.436653862834686	1.50533424380876	0.309392810111666\\
0.502277859071436	1.55091135955666	0.373128960529219\\
0.571816446990701	1.60072996369009	0.437708227074967\\
0.640634339259514	1.64180824132921	0.503741223253932\\
0.702863475564713	1.6938980380019	0.569547105290018\\
0.767703523237002	1.74477144201522	0.640765705504502\\
0.838987846409415	1.80057861810469	0.716908063729262\\
0.905544002759294	1.8570284413532	0.787790908144922\\
0.975474719821674	1.91674420466195	0.86644919650893\\
1.04026145249735	1.96817372844567	0.940443625728088\\
1.10619586999997	2.02246670642592	1.00891639137243\\
1.16765686988811	2.06939376269636	1.07931471959946\\
1.23573994474283	2.12443111378121	1.14497919445465\\
1.30158775659136	2.17076864519567	1.20471193671836\\
1.3671983888644	2.21714675790961	1.25959274581551\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00020775695172	0.241752468326017	-0.998207411825569\\
-0.935412660457032	0.293829513775434	-0.945800936610767\\
-0.871239674859816	0.336606502333263	-0.896456181201684\\
-0.808541806413232	0.383791459409964	-0.843740034979626\\
-0.747295722993108	0.428188110837707	-0.787160495564368\\
-0.685957354453649	0.471724817867047	-0.728515526449395\\
-0.624326120910088	0.517746242483975	-0.671694126636045\\
-0.565079026375145	0.5647115272411	-0.616493908649543\\
-0.506665091639353	0.612639196436584	-0.562975793784745\\
-0.450662943200388	0.666281371968875	-0.514734149996427\\
-0.390564184894974	0.713579958084468	-0.4687636267017\\
-0.332438751806191	0.765269474638649	-0.424816335969826\\
-0.271536519170302	0.817951094590046	-0.383183921346484\\
-0.209292031525921	0.870531366154017	-0.339336111957847\\
-0.146875008068577	0.920883730011517	-0.292182145126404\\
-0.0830619297188933	0.967117923257754	-0.24622403560658\\
-0.0190025917659913	1.01543061657803	-0.197558077179422\\
0.0463146252773338	1.0665823738543	-0.147657825204193\\
0.107590326974069	1.11861402453776	-0.0985198091543596\\
0.172196688471171	1.17227969641039	-0.05130621956541\\
0.237663158652785	1.22669549039476	-0.00404275707666333\\
0.307380372152273	1.28342599295708	0.0408935012984167\\
0.3796894396644	1.33444743074769	0.0868261666490223\\
0.454845401889092	1.38895559911942	0.132489653079162\\
0.531622067764118	1.44535519983395	0.176263967132718\\
0.601800283013693	1.49885816783364	0.222326432057736\\
0.676908940749516	1.55113522791756	0.268860502759302\\
0.748302461751008	1.60708930892292	0.312574123220425\\
0.817069811649118	1.65967719847086	0.356537006104763\\
0.886239338921974	1.71254464257122	0.407946342020007\\
0.957336911433076	1.75698937713088	0.451327092603668\\
1.030913206791	1.79956243382572	0.495754502256299\\
1.1073219333597	1.8619595214226	0.549421259363623\\
1.18463833455541	1.90987749375411	0.603452648070007\\
1.25684062884056	1.96240220296043	0.65338077251216\\
1.32739545930923	2.02083954535988	0.703923561802601\\
1.39664955208251	2.07153467299757	0.755171261002132\\
1.4642169515537	2.13032785613182	0.807560154139646\\
1.54029054503522	2.18966417491797	0.862873472463479\\
1.60160131632678	2.23871556754639	0.910406606830474\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997497770797953	0.241338622250135	-0.997689821932872\\
-0.935305408722999	0.297768099946843	-0.949867904844403\\
-0.875335708765558	0.342110242819317	-0.901852183933097\\
-0.815849241962318	0.393494416689344	-0.8581953643271\\
-0.757742463920341	0.434221336330512	-0.814672587605776\\
-0.699074320449531	0.477099486565259	-0.772991064002535\\
-0.640336141124177	0.512716515695571	-0.727457110946281\\
-0.575840145144716	0.548120828302769	-0.681013638705464\\
-0.518686074606721	0.587661264146064	-0.632144825901329\\
-0.460136356239959	0.622039593487913	-0.585035216907204\\
-0.405973766081343	0.659569930648631	-0.535321942193913\\
-0.351197114697678	0.69908797156257	-0.485978198919754\\
-0.296672365262517	0.734122246153381	-0.438880075596537\\
-0.242053822006569	0.765820407948098	-0.388312838826704\\
-0.186553322901428	0.797359101361913	-0.337177588026869\\
-0.132205049122026	0.834877891222277	-0.287265621766334\\
-0.0820790894718472	0.872534512104874	-0.236114342486902\\
-0.0360199003929473	0.902788813015577	-0.184077630742093\\
0.014504698540903	0.942014452743439	-0.126699027959907\\
0.0580565922504901	0.97575901111624	-0.0709197961710588\\
0.108704760710776	1.01065614913078	-0.0158575813236208\\
0.162441128017141	1.04281582328382	0.0350139541656995\\
0.211868799919124	1.07835584954129	0.0895762618026884\\
0.267614654424767	1.11508846064413	0.145417667938227\\
0.321295401555564	1.14590299024124	0.196990341840391\\
0.376017110984062	1.17830678585824	0.251811820578513\\
0.424864898874264	1.21009749242554	0.306463046234224\\
0.474134593098504	1.24102549811481	0.36185673587438\\
0.526208333874866	1.27205964880837	0.416768847238454\\
0.575730902605529	1.3043520829736	0.468890479567695\\
0.63048359626773	1.34259998022593	0.52301232229123\\
0.681910995817487	1.37421245082713	0.579085006821283\\
0.733135676836192	1.40693314636095	0.636641263658516\\
0.776524622534419	1.44108002332212	0.686512503131546\\
0.8293758470028	1.47087445357308	0.75200471300118\\
0.878038599561469	1.49615492704504	0.809110371381686\\
0.929546584371171	1.5283081672303	0.870945893273693\\
0.979460470974572	1.56142999572212	0.933079533889153\\
1.0321669016887	1.58884239567125	0.998263790334524\\
1.08094257537962	1.62718464447431	1.05514064333366\\
};
\label{pgf:realized-trajectories}

==> figures/results/scenario-rand-traj.tex <==
\addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999097315186919	0.240119845720588	-0.998329213122516\\
-0.938412095353681	0.295440126566335	-0.949231614583555\\
-0.878512791615236	0.340806297596779	-0.897664364211227\\
-0.816611331132436	0.388391284107827	-0.846652518350923\\
-0.756264247299061	0.430953857706298	-0.788542795559308\\
-0.693346798677602	0.477179850170322	-0.732806726098525\\
-0.633599009497513	0.525691123326287	-0.676768599237468\\
-0.577290825638977	0.574995702674751	-0.62150517088954\\
-0.522309512888715	0.624423455192063	-0.563569290256212\\
-0.465574742731491	0.673509682453996	-0.505666770494669\\
-0.408892490796794	0.719829021405084	-0.4466054956301\\
-0.352503658971736	0.766191572476398	-0.387410026197205\\
-0.297805366356346	0.812078150921203	-0.32558236930593\\
-0.243030960615153	0.85623754604451	-0.266362897759654\\
-0.193520760069313	0.904286350006819	-0.206959562961663\\
-0.141157391253395	0.953475887168867	-0.147201815584372\\
-0.0907455166952493	1.00139735951368	-0.0872885080405619\\
-0.0425576690079486	1.04778289551989	-0.0244577705657749\\
0.00282492915169044	1.09781824649243	0.0438777373380001\\
0.0565737955837675	1.15187541298268	0.106313216204646\\
0.10797019440556	1.20087217888338	0.172377656132818\\
0.161325119672917	1.25350548595618	0.237191095676087\\
0.21515978458401	1.31753096196156	0.300213086496812\\
0.271392805977068	1.37424111359057	0.362520098681723\\
0.33201801548201	1.43988655879183	0.427342396078996\\
0.391186315944183	1.50307631027328	0.495517768370902\\
0.445452114069583	1.56734539496914	0.566020288498512\\
0.506908482655378	1.63732088245499	0.634263296387283\\
0.549331935555102	1.6982240836136	0.699553937681523\\
0.604175723754949	1.76574419525826	0.765610972521112\\
0.659242072905705	1.82706975910274	0.835674754685076\\
0.713341541594064	1.89135293476561	0.902719944809226\\
0.770566008293583	1.94223570293987	0.964915878680431\\
0.827908195113713	1.99664706311779	1.02845572132607\\
0.890029784434075	2.04669553968328	1.09704364513822\\
0.955033659834317	2.09854691738488	1.16135988571675\\
1.01606760509757	2.14580206338748	1.21349562315363\\
1.07817559373134	2.21111847854855	1.27513029909803\\
1.1385821153485	2.26186625269289	1.32688609329567\\
1.20282493344029	2.32082152819043	1.39144809294066\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999667657862896	0.238173218303069	-0.997920668690405\\
-0.935784903697031	0.294398781427412	-0.949305133532812\\
-0.871210886795331	0.339217052961964	-0.902298536164682\\
-0.808200323443767	0.381929987661314	-0.849842262277774\\
-0.745813121953649	0.427107037955903	-0.798055905865515\\
-0.685129650788503	0.471942116021726	-0.745323886694096\\
-0.625304784298019	0.513570237308726	-0.693036976465682\\
-0.561810557637919	0.5554630076023	-0.643233500134224\\
-0.497163268612965	0.602609195051863	-0.589181958819995\\
-0.432870421577076	0.647717260435037	-0.541959806017581\\
-0.364732968296831	0.69175127298335	-0.492664363513962\\
-0.293457473207169	0.737765842164415	-0.443461715072101\\
-0.221934597662915	0.781366467477909	-0.396141012609215\\
-0.151103072946458	0.829666097750292	-0.352774052167906\\
-0.079247201751869	0.875330162963369	-0.306992134685458\\
-0.0065383115673814	0.920822809406805	-0.261741840358181\\
0.0644181911695005	0.969729747414371	-0.222088542729676\\
0.133873375463614	1.01213439957069	-0.174695113950791\\
0.211492204651671	1.05545602117726	-0.134289503229383\\
0.285919287914461	1.09413121789221	-0.0965963536127306\\
0.360094750580293	1.141824701382	-0.0564671814732959\\
0.437112530752416	1.18201692282175	-0.0158825087122953\\
0.511901831117608	1.22021870252017	0.0238666390745128\\
0.589930337717635	1.26811685005856	0.0683396505306249\\
0.668505584305252	1.31221622217147	0.102603112503561\\
0.739820170185275	1.35102097343292	0.137093133287093\\
0.817936143758984	1.39689732988944	0.171108615644905\\
0.89195169614011	1.43951244671421	0.204191235630114\\
0.968833705356383	1.47991378231493	0.227407522908481\\
1.04335471652829	1.53088700243087	0.254942466392028\\
1.11826650658343	1.57120971867254	0.276889956690151\\
1.19464354405239	1.61076484245047	0.300673516767108\\
1.272374741656	1.64905852456528	0.32068422032466\\
1.35515506597905	1.68737253394039	0.34225510062944\\
1.43732706164774	1.71610694613945	0.361396622647346\\
1.52164483412661	1.74963531223171	0.381795171980213\\
1.59752818231351	1.7863372178692	0.393402774599737\\
1.68048549684154	1.82243685751266	0.411131597581458\\
1.76939850653048	1.84988554472865	0.429142328458342\\
1.85293455268544	1.88858911443502	0.447308380711106\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999924837645672	0.241729177915146	-0.997478542776999\\
-0.937681164454054	0.292192750777386	-0.946703338527673\\
-0.878568289169036	0.343650225908645	-0.905308451817009\\
-0.818919711852958	0.394420933981825	-0.860678227362683\\
-0.754598519921171	0.440324111021316	-0.816337589535641\\
-0.689433670270014	0.489478495783867	-0.771326094999197\\
-0.626931673928238	0.534328670500652	-0.724755812370957\\
-0.566270433800586	0.583945836072204	-0.673426835276538\\
-0.5027953539105	0.633129182445539	-0.617329134314982\\
-0.443648624447506	0.681483771291245	-0.557108680896433\\
-0.381459744230073	0.724035331737841	-0.500230688911273\\
-0.321631027984259	0.76620000505117	-0.445800818212269\\
-0.259610519426787	0.816590856645716	-0.389021038288267\\
-0.196360582528207	0.863726388066227	-0.329800722523275\\
-0.138093303928964	0.911039500425341	-0.26642811127088\\
-0.0803888829457074	0.964797150196262	-0.208107030910868\\
-0.0211098465411437	1.01986537164632	-0.14941524298466\\
0.0424767654185755	1.0735123437897	-0.0850116423601921\\
0.102890399436442	1.12647594020454	-0.0267406652018197\\
0.1638152334735	1.17812365106589	0.0335642712888511\\
0.217369303309985	1.22710835879745	0.0923958316330016\\
0.273212289080171	1.2769121142545	0.151282815622763\\
0.326735137756616	1.32810755374869	0.208531645226444\\
0.37725296408845	1.37561128013418	0.266859890366238\\
0.429410292599422	1.42541532145426	0.328279951489699\\
0.481162847280057	1.47170369969262	0.389705496781714\\
0.52932906959137	1.52164030506356	0.449005272619135\\
0.574000185312082	1.56991382284694	0.505705798064868\\
0.619548005893587	1.60567741835183	0.55876119786146\\
0.662750942195111	1.64296270893025	0.615527738407152\\
0.707841582658699	1.68811455830587	0.672353114429739\\
0.750445765376639	1.73566971057371	0.730152122611179\\
0.796494069861394	1.78355092966546	0.786834106374463\\
0.839344706221885	1.83297375351583	0.850164601489153\\
0.87931395490178	1.89326684830717	0.90916643430478\\
0.915777648722567	1.94770717605551	0.959944434582392\\
0.949782110304803	1.99867803352606	1.02079645971072\\
0.983925357006963	2.05455423479001	1.08344051779624\\
1.01075553830751	2.10281458745752	1.13305205104931\\
1.04379994530776	2.15211816265308	1.1907194622744\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999478013440514	0.239121487946158	-0.999664169531621\\
-0.937919876202622	0.300262643840738	-0.949440908815235\\
-0.872945467509057	0.340046629608734	-0.896844670300923\\
-0.804632616432495	0.391936590717664	-0.839258657082587\\
-0.742691908422451	0.442684134614955	-0.781659198657779\\
-0.673202502243283	0.495630071255598	-0.719673845258915\\
-0.608168576948165	0.54780125920894	-0.651868795849366\\
-0.544810218600067	0.607407133032499	-0.579597294613321\\
-0.487314311397158	0.665107114801059	-0.509448534652274\\
-0.432317215081443	0.720341586380996	-0.439604476220697\\
-0.376675469530773	0.776095232950088	-0.369240626938829\\
-0.327117596602069	0.838461179420792	-0.302687526082584\\
-0.270657245407119	0.893645480317961	-0.2334230398002\\
-0.217031304029397	0.951272579562135	-0.16979722191176\\
-0.16313207559679	1.0019400607661	-0.101346322294367\\
-0.110643155564647	1.0579217936251	-0.032360869655571\\
-0.0571374588816951	1.11765721426541	0.0321714731982948\\
-0.00268375698680666	1.17624748971723	0.0957200692271709\\
0.0600950417554353	1.23908422052683	0.155574377739027\\
0.116628584544364	1.29854070254098	0.221616645435937\\
0.174352152453095	1.35911963201167	0.282043748453936\\
0.226881686004214	1.41883910376421	0.342040959781102\\
0.278859926509455	1.47489728216788	0.409194268661487\\
0.338077194537511	1.53169947861436	0.478150815151479\\
0.389425510186719	1.59133650957836	0.54159794166849\\
0.440920309230101	1.64134669664039	0.614851913131274\\
0.500769228324601	1.69736098010417	0.684263666035433\\
0.557427566640788	1.74929691731827	0.757367514396136\\
0.620095323988923	1.80111935439877	0.825193497402672\\
0.679861845802182	1.8504353721842	0.888987578365886\\
0.749867191447688	1.9049557385142	0.959037787026043\\
0.816187231743557	1.95461102350735	1.02605016818157\\
0.882605878828086	2.01233926787184	1.09987866918675\\
0.945865302569833	2.06557461300503	1.16485708437803\\
1.0054864236239	2.11745255540829	1.24129861209178\\
1.07355599734616	2.17706887679202	1.30473662224727\\
1.14074214222072	2.22275149504989	1.37680807708408\\
1.21409580086994	2.27917271594911	1.44486037917327\\
1.28265929370191	2.33709720180578	1.51601873073528\\
1.35064422845006	2.39357851378861	1.58384642030979\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998394363748421	0.241391636925528	-0.999676549414364\\
-0.936918381121223	0.298669992849192	-0.952094821158014\\
-0.875767908208196	0.343758352253392	-0.902905729901582\\
-0.815197212569857	0.392635576534526	-0.852626760192742\\
-0.753561249753385	0.440544606832965	-0.804526772703398\\
-0.688172570774846	0.490685192407003	-0.75064146760025\\
-0.624898115728265	0.546176192777976	-0.699077403445479\\
-0.561099281407153	0.602664714348731	-0.647079927584265\\
-0.49883757961662	0.65759771439262	-0.596232810753198\\
-0.435796183985938	0.710038888086768	-0.545440631051465\\
-0.373558648862864	0.769846214817057	-0.498040297105428\\
-0.314811782972639	0.828358498517937	-0.449357447921745\\
-0.2524024449055	0.896486465279975	-0.400265727976023\\
-0.192428253892741	0.962132014710789	-0.352285981124797\\
-0.13614184645904	1.0347170348175	-0.302497530760353\\
-0.0789206302516105	1.10277525703474	-0.248021472590597\\
-0.0251768291052274	1.17080059360707	-0.194291800797375\\
0.0293264326133252	1.2338702608214	-0.139257610005553\\
0.0861150100645423	1.30144023970158	-0.0886725710442827\\
0.143442980144328	1.36360002529055	-0.0369989662238396\\
0.201833597136823	1.43654387106327	0.0139565168372836\\
0.264952058314463	1.49954728847255	0.0605763557484886\\
0.327707811149283	1.56599261571286	0.110653745496687\\
0.394652125690023	1.63494296894629	0.160483867893581\\
0.452484459751574	1.70202312042417	0.210802665712741\\
0.5188420244303	1.76826251934115	0.265571934717872\\
0.583542550314195	1.83009966842947	0.317526540822369\\
0.652423235208146	1.89615201453503	0.371432798691608\\
0.722234329351696	1.95296742904529	0.427563973234104\\
0.797316877094472	2.00265708470708	0.483030450142666\\
0.872521777413502	2.06269868321607	0.544082891500222\\
0.942497800152492	2.10832357916145	0.597794893697672\\
1.02164341774071	2.16643438555882	0.659641741117754\\
1.09658968206325	2.22547782002623	0.722617067153515\\
1.16500599235602	2.28256003924498	0.778822768177995\\
1.23073515842758	2.33094914084345	0.832729757842996\\
1.30930344784289	2.38209429114025	0.887390751044605\\
1.38102199640084	2.43537171679772	0.947746989953797\\
1.45358138892782	2.49672284031577	1.01248982293028\\
1.52283257003745	2.54991729243403	1.0745339534392\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999206536821372	0.240614747710416	-0.999073765700739\\
-0.935747572771599	0.302554105470016	-0.949879809824215\\
-0.870085126440494	0.346651400973685	-0.898353459256663\\
-0.801329617155861	0.391252537491979	-0.844179580165398\\
-0.727861053855633	0.437286842337528	-0.793252966531727\\
-0.659903423554284	0.481716265764999	-0.742017905787137\\
-0.588749767361451	0.526441936775682	-0.687609600606862\\
-0.521788163477617	0.569496176155087	-0.635303353428615\\
-0.452161445437019	0.612263906426604	-0.583944864080208\\
-0.384968777677234	0.653505830051902	-0.53273794985631\\
-0.319373798657001	0.699595877740737	-0.480702393197372\\
-0.25002209192796	0.745477200657465	-0.426650616009033\\
-0.183112722215193	0.790983304225942	-0.367161808439276\\
-0.116039073883759	0.832499824607219	-0.305981387013783\\
-0.0491504999613637	0.872769645838886	-0.239981629032361\\
0.0134816638648992	0.917597551479742	-0.178202779981601\\
0.0776509297510142	0.956300051644895	-0.121771618324796\\
0.14816734953278	1.00064341847066	-0.0626745455673806\\
0.209082679261966	1.03734764337466	-0.00566020908517983\\
0.270636163818125	1.08074926264287	0.0485983283630865\\
0.335290536577594	1.11599847599121	0.111213780993127\\
0.398364715998242	1.15735503127916	0.170549149837201\\
0.462491158506485	1.19526592435404	0.228020511597368\\
0.526985046473297	1.23750385738186	0.281181029826116\\
0.595398138508177	1.28667294923754	0.340404343741137\\
0.654031403299382	1.33332692039148	0.400327171479644\\
0.715529531168409	1.38070372121129	0.464413802530454\\
0.774004358053077	1.42673058628537	0.532988378815541\\
0.832772151192636	1.46705069051013	0.599592577059147\\
0.888441175422733	1.51648837018956	0.662001696238218\\
0.946164642931846	1.56144889657937	0.72553379100922\\
1.00727868284173	1.61147515367677	0.792025434252592\\
1.0605874770109	1.66222244787825	0.852979107012315\\
1.11579267058985	1.71036936269883	0.913129270544734\\
1.17362794424683	1.7652853772959	0.985685724399741\\
1.23473228422935	1.81102251786995	1.05801304258326\\
1.29133062734567	1.86213339013939	1.12443621282147\\
1.35060711126922	1.92355931891312	1.19781805762717\\
1.4072385425516	1.9799713390525	1.26482317833978\\
1.4677627386464	2.03973471946858	1.33607070297014\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997883052500354	0.239562788719727	-0.999762184395189\\
-0.940996731810911	0.299202210121269	-0.948236377052586\\
-0.87911351281499	0.346255871198857	-0.898271486084\\
-0.823675025519549	0.389823822937065	-0.838610405547637\\
-0.769904405349007	0.434968934088193	-0.780165200632715\\
-0.712807781097405	0.474518048507076	-0.71472077338568\\
-0.65255664237385	0.520020696850162	-0.652418996932862\\
-0.595516806784177	0.558357933009645	-0.585080714163673\\
-0.538107912019687	0.602900647134081	-0.527400225730435\\
-0.483908647992432	0.644795766482449	-0.470550629464525\\
-0.43519436620072	0.690958385027276	-0.419232662240288\\
-0.382523690858809	0.735316388859158	-0.362577962272532\\
-0.329902162460523	0.776602583521377	-0.306884233448779\\
-0.278082033030916	0.828359581808442	-0.249840917333089\\
-0.225079816712181	0.876241512989808	-0.19531162091268\\
-0.170900832214055	0.925176847067152	-0.144054855766131\\
-0.116742834690869	0.973018330820666	-0.0893300328887857\\
-0.0624394644136377	1.02153583572487	-0.0448568270436764\\
-0.00577332859339685	1.07044479374776	-0.000920093897412682\\
0.0553641530800267	1.12488706094108	0.0436711281739225\\
0.114230016053197	1.17850102451915	0.0856520695225139\\
0.176789081501078	1.22591104014739	0.125805264868109\\
0.235512507891229	1.28004758400266	0.167331607676494\\
0.295535859530024	1.32939277352212	0.209155733249646\\
0.353722194315284	1.38011443215806	0.249022341216393\\
0.414532535755917	1.43675919406431	0.287667774705727\\
0.479258626095354	1.49600354249477	0.329848877583506\\
0.53173124446456	1.55555084735801	0.369697097335034\\
0.592932355954638	1.60842797308848	0.40975237770025\\
0.655115745090827	1.66474625526034	0.444502588779189\\
0.715754777221152	1.72403338974776	0.483427225629467\\
0.781599442546714	1.77381994572981	0.519613707393719\\
0.838067541498961	1.82717185638151	0.554225113916129\\
0.896449291980583	1.88818802403999	0.595879865356262\\
0.950550526056233	1.94171452484885	0.637873644316729\\
1.00895588826109	1.98508109395879	0.666801709341455\\
1.07027089243773	2.03911541539847	0.697469444289449\\
1.13282803001197	2.09728817885692	0.735774512405907\\
1.20244497662939	2.14622201057137	0.768879084125373\\
1.26927320717982	2.19726941539339	0.796044395505939\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00063716616188	0.241454311329808	-0.998645583687718\\
-0.937205208924317	0.301802541380557	-0.952111243642743\\
-0.876642622141368	0.34868600566378	-0.898622993834135\\
-0.819781338820658	0.395331527475424	-0.847474210687307\\
-0.758410314173534	0.444448998456875	-0.797983044158325\\
-0.693252783818156	0.497173217701488	-0.749053419622195\\
-0.629842025464283	0.550715637495785	-0.701412945984744\\
-0.566563601183096	0.60211363522896	-0.649075231225138\\
-0.506677778174417	0.657528260049903	-0.597745300773904\\
-0.438572139081411	0.717734841290323	-0.546013837285958\\
-0.372168895391132	0.777188744693852	-0.492202320471858\\
-0.315253685667198	0.838041290093364	-0.439557757902515\\
-0.251982770072643	0.897644255227291	-0.389011336626355\\
-0.192999006836236	0.960516347810662	-0.340087475761595\\
-0.136795947951068	1.02179893723344	-0.296563342468607\\
-0.0812706194522889	1.08396767647464	-0.248736117013248\\
-0.019614308991939	1.15097630173867	-0.20135460959152\\
0.0417152550813636	1.20744694247774	-0.154055536670709\\
0.10067181800372	1.26969969681178	-0.111070634989086\\
0.157637409496742	1.33124632079093	-0.0681202175718269\\
0.212813424725048	1.39292093026006	-0.020604002537148\\
0.272804998892333	1.45274837527847	0.0261000654517899\\
0.329804275226962	1.51344214336638	0.0676143578808853\\
0.387463218245537	1.57707583713732	0.118925726664259\\
0.446315174987434	1.63949739106265	0.165910214173213\\
0.5064195008976	1.7003305700312	0.215719432735994\\
0.560510198525291	1.75796494449459	0.260280536278802\\
0.623292017097367	1.825073278648	0.309005428639286\\
0.681940798166191	1.89490853929142	0.351218557850494\\
0.735341556594547	1.96304288399763	0.400036837865433\\
0.787907995854191	2.02429818414479	0.45033159091882\\
0.839314956909585	2.09842254323848	0.498438832575956\\
0.889821271244156	2.15752778842198	0.54592261509251\\
0.945814327792981	2.21859733023748	0.599545551758071\\
0.998989254242033	2.29081859034814	0.65084179676585\\
1.0555744088369	2.35574590616082	0.707343019389085\\
1.10345036676242	2.42200679028767	0.75968714801057\\
1.15266204462236	2.48423228126415	0.810776648317614\\
1.20538345445542	2.56802674263579	0.859657922911382\\
1.25750965581708	2.6253702260006	0.914616958698115\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999761700001014	0.239403006681903	-1.00064917212024\\
-0.937083741657319	0.294373445482623	-0.950469718385001\\
-0.866498553188442	0.339414873676002	-0.902809632387336\\
-0.795910058453806	0.382635376069131	-0.855747809311152\\
-0.722870800432642	0.425582219247966	-0.817688634859142\\
-0.650288491168251	0.468951313780107	-0.767575540394902\\
-0.57731033225852	0.514846285250778	-0.723355474033801\\
-0.509280094747592	0.562004399035181	-0.682855542108367\\
-0.443350252481358	0.615311835089838	-0.641896614799916\\
-0.36974734708259	0.668287915692574	-0.601156746642196\\
-0.297977393833331	0.722467178519768	-0.558465022701712\\
-0.222637099954328	0.771493790058387	-0.511730091595466\\
-0.14733763734938	0.822020443010629	-0.474378458458396\\
-0.0695166124726907	0.87151120941725	-0.431700718223935\\
0.00557842257860166	0.918921857558559	-0.388990247379048\\
0.0786352692641716	0.966885612175444	-0.346295891777934\\
0.151804010102404	1.01138556058554	-0.305464995906099\\
0.229184125424188	1.0587036306456	-0.264266006828897\\
0.303815765674651	1.10430062535515	-0.224765862907762\\
0.373161398829609	1.1514467749324	-0.185326287399925\\
0.449074088647261	1.19623366026015	-0.147777091255457\\
0.523856329732424	1.2401467952344	-0.109307611772504\\
0.597050856067149	1.28166219814115	-0.0733329690362184\\
0.666429531420284	1.34028457446826	-0.0357997775499501\\
0.734325524569692	1.39224101652019	0.00773283710159763\\
0.797214043380172	1.44181150257172	0.0432169956484051\\
0.860060750666171	1.48836632867528	0.0800071987863419\\
0.931424530450094	1.53670570482633	0.121163547677733\\
1.00062948743957	1.58978171720524	0.164634962687663\\
1.06316780852666	1.63763103683876	0.210132750385208\\
1.14239457049625	1.68275328595518	0.253975943840862\\
1.21261184245252	1.7298573092557	0.289613858523382\\
1.2852054776753	1.77838257977673	0.328176939380943\\
1.35716420480542	1.82792492289509	0.367898821959726\\
1.43219241032717	1.8799483647952	0.408911875974675\\
1.50751959665862	1.91701301547635	0.451607809764857\\
1.57498585601223	1.95862414773015	0.49433054244464\\
1.65492450528847	2.00299315142748	0.535073312125774\\
1.72552426370735	2.0446060887609	0.588618345274859\\
1.80027746548308	2.09282137366448	0.638922438455971\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996557484340456	0.238127046917851	-1.00033070407717\\
-0.93513036312295	0.294731733763121	-0.949236022945345\\
-0.872248630463624	0.33502965491585	-0.902049049719279\\
-0.811783366682228	0.373738005004437	-0.850490665650075\\
-0.743483424008749	0.420488362023471	-0.802506016003737\\
-0.678178150151024	0.464440157062153	-0.754900619054351\\
-0.613837722533753	0.505346708182796	-0.703550884169227\\
-0.550773095256114	0.544149676926005	-0.654597133463295\\
-0.484783111725279	0.576553565383625	-0.601380901785099\\
-0.419891026595235	0.602767477244866	-0.549539256249417\\
-0.355936053713014	0.628793672874905	-0.491666868401052\\
-0.287871815613709	0.657796338689459	-0.433591164827056\\
-0.223142450241228	0.687876582257511	-0.37692982574188\\
-0.1576564849622	0.716018257216614	-0.320710851529268\\
-0.0902147955503067	0.747648995606423	-0.260003452656784\\
-0.020992257203037	0.782254675672127	-0.202098856176548\\
0.0447952876140054	0.816035904893276	-0.139867454421879\\
0.107240191087314	0.845079539501693	-0.0830441012464023\\
0.166325622747975	0.878813853349971	-0.0204600605168311\\
0.227368626549095	0.913951924739406	0.0382483035671166\\
0.292686560664903	0.948482884708528	0.0986522426200731\\
0.355256906569886	0.978937354953976	0.159478173175479\\
0.417232181140286	1.00983197106356	0.224787873848702\\
0.481064852892179	1.04740121192606	0.291947225524282\\
0.543566132632117	1.08224217749785	0.357307703517591\\
0.608078679972692	1.11415210912127	0.429078478255093\\
0.672066702127995	1.14766939923219	0.49671352484031\\
0.732981496090601	1.18166390481801	0.568159265928992\\
0.783627929520301	1.21376666421331	0.640942806117818\\
0.8344997953883	1.24690171289741	0.716566771170719\\
0.885039902463244	1.28073374473318	0.786940207782146\\
0.930708452832229	1.3115687574571	0.860905840384476\\
0.98360931213329	1.34306895639374	0.939576414751668\\
1.03603582288931	1.37468961101943	1.01230001250279\\
1.08966971776071	1.40527663662884	1.08296245920174\\
1.13626295165955	1.42561490088607	1.15306202232274\\
1.19215253749428	1.45547645371559	1.22816334027747\\
1.24157209939946	1.47269876202887	1.30333572842356\\
1.30164444783406	1.49081693517748	1.38450619067058\\
1.35424781864775	1.51250693156614	1.46719124853321\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998143503907388	0.237834720674987	-0.997862096085271\\
-0.936119373375667	0.29635870836499	-0.948464643518147\\
-0.877015955066647	0.33924871954674	-0.903160394177027\\
-0.812590672948743	0.384192528212344	-0.858675410842631\\
-0.749281978678445	0.43131747400185	-0.814889078940378\\
-0.683932352360197	0.479000083663537	-0.772748103589553\\
-0.623711676075119	0.531963156861454	-0.73212274666469\\
-0.564845833995446	0.581550208705826	-0.694764928561899\\
-0.5055480002133	0.628453895740117	-0.65908097128571\\
-0.444316879162597	0.674607389249144	-0.623936411013735\\
-0.380007057096599	0.724880882819921	-0.58393302298713\\
-0.309997303481852	0.7756871852443	-0.543238813205964\\
-0.239000843607946	0.830241204981572	-0.500675070154326\\
-0.172836106117607	0.882627757546596	-0.460227256581453\\
-0.106308300553263	0.938201516825577	-0.41703412596941\\
-0.0471534947563634	0.989288780128619	-0.371691141212866\\
0.0117366833573346	1.04837825859809	-0.331429212711511\\
0.0727443352361	1.09819029551659	-0.293151152697399\\
0.135386836081989	1.15896980561673	-0.254126685777976\\
0.198628929069509	1.20673347677698	-0.213717569504495\\
0.258673408497719	1.25994052522973	-0.173099333122474\\
0.320150846837991	1.31866106270209	-0.134773249158211\\
0.378929026791078	1.38521212080011	-0.0983565558729863\\
0.437873959975012	1.44270196064706	-0.0614942750998124\\
0.492321536975069	1.50285652136453	-0.025457833716979\\
0.546318410874817	1.55391028322688	0.0166150332734676\\
0.605540743583913	1.60912346203265	0.0588836632214943\\
0.666835145503873	1.66369002246334	0.101656455169822\\
0.72514641941733	1.71731321995269	0.150913802880084\\
0.782775627550259	1.76859293944252	0.196711908174917\\
0.845024159096932	1.83350206120734	0.240048580285645\\
0.905431261187945	1.89610129815776	0.285097770227969\\
0.967434816477778	1.96053005994677	0.329864810774429\\
1.0263995539753	2.02495426435714	0.372367418412664\\
1.08691134623291	2.08659693821654	0.423219304952599\\
1.14247857492891	2.15222889688014	0.470000266194938\\
1.20268458384461	2.22302768969197	0.520221362073296\\
1.2639002057665	2.29081616581861	0.567124247456189\\
1.31723846452443	2.3636705289299	0.616132282466592\\
1.37474288671603	2.42693167401703	0.661817703761842\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00142900461296	0.240147957678304	-0.998406460851612\\
-0.938197324332236	0.295334718464668	-0.952216015599749\\
-0.876839873964868	0.350178567484294	-0.901017568029402\\
-0.817496685826353	0.39618640386396	-0.849058939655302\\
-0.754302742769883	0.44098662705796	-0.794953670378155\\
-0.69192095378022	0.486774376254353	-0.748227583885473\\
-0.631354894185067	0.540080255498246	-0.701509102663529\\
-0.567160208013936	0.589033886692762	-0.65416397239147\\
-0.498960196856029	0.639448901286538	-0.606626205052239\\
-0.433302647164134	0.690927832605153	-0.559422133930822\\
-0.367502040962729	0.740061535168137	-0.510308694318523\\
-0.304932952225055	0.795547537011483	-0.462312130639576\\
-0.246133728336513	0.844070893732651	-0.416333206049848\\
-0.183151079213261	0.89667013869535	-0.372597622473266\\
-0.123073122467333	0.949187994951381	-0.323872478356829\\
-0.0599848181730635	1.00269707003528	-0.283246784079472\\
-0.000309752347445189	1.0556467315861	-0.235367346343113\\
0.063173487596274	1.10473570297316	-0.189521452313285\\
0.123886762248131	1.15126495604683	-0.149011666221997\\
0.186443847513615	1.19844426176845	-0.107739925708104\\
0.24693645963093	1.24410024797039	-0.0705626168191486\\
0.308258490539158	1.28967133235073	-0.0290909828346624\\
0.367846196243475	1.32535456310175	0.00330638897666914\\
0.427108524834924	1.36331730750391	0.0424891208927427\\
0.487278962720125	1.40173273654597	0.078392918436746\\
0.545400045400908	1.43415701456405	0.118292343076596\\
0.609133393740637	1.46883226202543	0.155340761660565\\
0.665965407605042	1.50147064154481	0.192594451722163\\
0.726813411340104	1.53465599570732	0.231493014982381\\
0.78525879049664	1.56803461360385	0.269073261142687\\
0.838786959347744	1.58847390345152	0.303170465642419\\
0.892005642473626	1.61372688249988	0.343783246671645\\
0.950855960118939	1.64824200717464	0.372693398799394\\
1.0072378680843	1.6714115179774	0.404857575435964\\
1.06370903706535	1.69829559562477	0.440066723251571\\
1.12481121783017	1.73151505961917	0.474039891532218\\
1.18624750005605	1.76011557948633	0.50961939888103\\
1.24513870865576	1.79057214961095	0.545563326536426\\
1.30048742944756	1.81247736836193	0.580687749516901\\
1.35829865956036	1.84178797899312	0.611136084006384\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.000431929394	0.242108810241391	-0.996613678930367\\
-0.935395247542184	0.296696837414976	-0.949268898252742\\
-0.873466293320584	0.336764606567942	-0.904652114447874\\
-0.810857531351084	0.385165017454719	-0.862627261291802\\
-0.745019123144069	0.428570708651443	-0.823328312950029\\
-0.679732999223635	0.477891179298135	-0.778109137581995\\
-0.614085299734276	0.525537029290357	-0.73407857204494\\
-0.553436679857362	0.568002879711038	-0.688347702132144\\
-0.48873106549623	0.614967439871658	-0.643905357028129\\
-0.4257494399878	0.661433413824767	-0.600762487765264\\
-0.363236170211182	0.707915303996083	-0.558763809627151\\
-0.303957803765229	0.753165135814846	-0.520776306799409\\
-0.24553924893707	0.79938725917993	-0.481019442302414\\
-0.188214276627694	0.849078387009438	-0.440856542605533\\
-0.128743658521414	0.894051825053391	-0.404589860691225\\
-0.0744397850636842	0.944413409009806	-0.37611361594768\\
-0.0203425627323284	0.989312849002061	-0.342400349984501\\
0.0359658143602226	1.04358101270269	-0.312861974034751\\
0.0925091039836771	1.09763602470283	-0.286264633099817\\
0.144807044968857	1.15212865150002	-0.25918860109279\\
0.195680860483034	1.21246766894415	-0.233152024596562\\
0.240935939112717	1.27762167330057	-0.204539391843426\\
0.291908249317216	1.34282715546215	-0.175139414471213\\
0.340000559067686	1.4063321122499	-0.147170027959631\\
0.39158194427972	1.46969012595874	-0.118719167386497\\
0.442579932439202	1.5367482694804	-0.0870962927934579\\
0.488893576129766	1.6060146048989	-0.0532176495575057\\
0.532908376754002	1.67309253795844	-0.0226400508827586\\
0.577611649866443	1.75170206681924	0.0101117423579534\\
0.622171702248338	1.82756434998143	0.0446559497183861\\
0.666018123806787	1.8964131217669	0.0834059606004055\\
0.715364591791782	1.97093698788423	0.11904090063922\\
0.759105280982104	2.04473207028721	0.15684534030507\\
0.801045366455763	2.11641537296264	0.198211436191412\\
0.852682136375208	2.19166312589285	0.242416508774737\\
0.897160014769339	2.26941307026482	0.277077230807292\\
0.949585212081186	2.35692661164114	0.316272231060444\\
0.991432937900816	2.43551139464911	0.355832102985598\\
1.04250084342095	2.51861318429785	0.400757017845699\\
1.08025195696505	2.60354495538013	0.44687055238035\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999675674549572	0.240809603814368	-0.996921683921689\\
-0.936509765495007	0.295010362876939	-0.946156867203659\\
-0.877103012466081	0.340598187773546	-0.897014585165409\\
-0.818272275394896	0.387880425247887	-0.845897554927339\\
-0.7612194144048	0.435420541447693	-0.794485899749282\\
-0.704979922365958	0.479729633550489	-0.741286744571794\\
-0.639208909238037	0.52062089366172	-0.692090257591796\\
-0.577984003417673	0.563109006909322	-0.642529064414549\\
-0.517015284371299	0.609516847928064	-0.592728708926859\\
-0.453773579922665	0.653794869828183	-0.541515223852534\\
-0.390079089332476	0.697274369166527	-0.485863733536751\\
-0.327504657776601	0.739934896551448	-0.429486405389553\\
-0.262046441398609	0.782759138766421	-0.37033900678668\\
-0.200656581709071	0.823695585443169	-0.314480824297384\\
-0.135284097210144	0.856714784846357	-0.255904593947051\\
-0.0762283681468417	0.903093108106359	-0.202002253319113\\
-0.0157703330350061	0.945477958711656	-0.149355461581598\\
0.0496086043769402	0.983430956724827	-0.0939053984881232\\
0.118090518779486	1.02445102772296	-0.0402722598189369\\
0.193554947819586	1.06240224522367	0.0130537006441972\\
0.267871710043001	1.09142390631313	0.0672498013698857\\
0.340769264519242	1.13167393744778	0.126832226891232\\
0.415027483905811	1.1684706298973	0.185288116350222\\
0.493316719837835	1.20831694210164	0.246903465407932\\
0.569107983300983	1.24994792427442	0.306778315649002\\
0.643339190981587	1.28563769326021	0.362948265532255\\
0.717433211087527	1.32212580465582	0.420520769832319\\
0.789162984553019	1.36187154184974	0.47776243035757\\
0.857169685997231	1.4034313712596	0.529632835913584\\
0.924296060951781	1.43705292018788	0.591922695395719\\
0.99248551362416	1.46425018627655	0.653714754855534\\
1.06219677563893	1.49906144777219	0.716928985872617\\
1.12793576496037	1.532796602114	0.784138692702429\\
1.19188657303142	1.57148097241137	0.851479263160206\\
1.25398166792128	1.61627880764542	0.925146542849287\\
1.31955955764024	1.6621984086671	0.994470907699137\\
1.38426700887822	1.70276569314377	1.07090787017195\\
1.44694614785174	1.73113117810826	1.13828249090098\\
1.51331152355335	1.77379614841949	1.20205150378024\\
1.58202688317567	1.80498441091493	1.26572979578591\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998523188471092	0.24048552892452	-1.00170842600049\\
-0.935694876595461	0.294255158763531	-0.953312919699704\\
-0.873418569530788	0.338750563478147	-0.903297305057812\\
-0.805937368358524	0.384714228935152	-0.856472366409174\\
-0.73644881916597	0.432362602700558	-0.809117172270303\\
-0.666096514273311	0.47435451738839	-0.762009897867566\\
-0.591687476407541	0.515490821271538	-0.714647926220729\\
-0.520202312442606	0.554686755200702	-0.668895876428494\\
-0.445075328958954	0.597204489312534	-0.620528376394389\\
-0.373611501295216	0.636541202900459	-0.573202326591494\\
-0.295549321703794	0.675197984979172	-0.531126962977454\\
-0.219949517412132	0.716566562050213	-0.489533313473778\\
-0.147744684498745	0.762571193658453	-0.449373578371776\\
-0.0747871774099083	0.805580254413355	-0.405371776163637\\
-0.000202109465291554	0.846650434434639	-0.363725599102718\\
0.0753779075001549	0.888742353086232	-0.324305521727015\\
0.148253855657127	0.930235521506898	-0.283263750983281\\
0.223504508926574	0.977710040914858	-0.241468903491411\\
0.298977616156341	1.02924642998083	-0.201342160570331\\
0.371607400002179	1.08011982849191	-0.158799968742345\\
0.44370301713544	1.12859088483185	-0.119848679034722\\
0.515670821589246	1.17716622598193	-0.0756963960955148\\
0.584310341113133	1.22100853665103	-0.0380155945506723\\
0.659067341253921	1.26929434150498	-0.00232670106254471\\
0.732343555720719	1.32066213858617	0.0353356334245465\\
0.80901870036679	1.36620824688496	0.0765995747885008\\
0.884830417415499	1.42409074044718	0.117268979460787\\
0.953978596030018	1.47702275851655	0.157121450691774\\
1.02794018824188	1.5266594734392	0.194957906169915\\
1.0977445584735	1.5784186864705	0.235820516626036\\
1.16676120248622	1.62998773548756	0.282958365704768\\
1.23308664372872	1.68333826260255	0.329986096163865\\
1.30143636944258	1.7270812039364	0.375240226634142\\
1.36936122985612	1.7726067393875	0.423324001247358\\
1.42882773716402	1.8141801079722	0.465804077238354\\
1.49270864182533	1.86094409073697	0.517680618134507\\
1.55421912696374	1.90875222482126	0.564929672971485\\
1.61189952531815	1.95651327017592	0.617552476208053\\
1.68018299996685	2.01627387974435	0.671481385110162\\
1.74317521048629	2.07317420510261	0.725931570315693\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996266401555801	0.241065408109953	-0.997524270030674\\
-0.935616037530966	0.298961037372814	-0.951290848895173\\
-0.874271186655702	0.341871700352364	-0.899247061247083\\
-0.809770474953617	0.390197258806424	-0.845434199766446\\
-0.744783683903365	0.440345301405434	-0.792957324392102\\
-0.67832651014073	0.489964877939231	-0.74178982719984\\
-0.614311038930228	0.537634431299462	-0.686781912050792\\
-0.550704392560502	0.587461630952286	-0.628914223909\\
-0.485076361067475	0.645340318151365	-0.570181501562755\\
-0.422779396086289	0.693670264799247	-0.513776130221047\\
-0.358407445522421	0.745514559139438	-0.45387248940336\\
-0.294554756489185	0.800494452650882	-0.395580236585909\\
-0.228370504371983	0.857626438502614	-0.340759525021052\\
-0.164919570666964	0.918189069285596	-0.284081000782394\\
-0.100428300424231	0.975671411156861	-0.233126161714587\\
-0.0364873631808184	1.03354529816135	-0.174485607486058\\
0.03039503565278	1.09414494202886	-0.120043416591615\\
0.0966370966310939	1.15705947319445	-0.0604133705478779\\
0.164139675264674	1.21258994170563	-0.00387211094833333\\
0.234579919298428	1.27117994893513	0.0555895249896556\\
0.305604083576958	1.33347476322621	0.115301323866013\\
0.379635059950721	1.3991913971082	0.179514850063613\\
0.445239738524514	1.45915603264508	0.244340787753376\\
0.511424747596353	1.53032589957715	0.308376282465888\\
0.587592606715259	1.59903285665379	0.373734646131174\\
0.662927073760067	1.66167057488262	0.442080929446937\\
0.733463540853294	1.72478466110331	0.505233329322579\\
0.808293643815278	1.79699096215508	0.569880227308837\\
0.8822383050201	1.85960945772145	0.63979966364737\\
0.956602348522238	1.92284929365042	0.707140390382085\\
1.03346178189316	1.98734342347434	0.773131982992607\\
1.09750265277435	2.03994716096301	0.839721978493359\\
1.17178781605971	2.09700204093048	0.91469809006404\\
1.24578754766594	2.1606719798423	0.990379204647398\\
1.32598663784628	2.22737527943389	1.06791622348461\\
1.39326662282973	2.27572595369693	1.14591160953309\\
1.46317253085109	2.3362594425709	1.22851334309658\\
1.53616151781272	2.39669887221766	1.30699230440716\\
1.60590422014942	2.44918304097556	1.38804621914146\\
1.67886003856337	2.51380092142403	1.46795566141155\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996553195622749	0.241428731307668	-0.998680181989563\\
-0.936946398371795	0.296336888334277	-0.952899488956145\\
-0.868689540023367	0.344896077759647	-0.908049532780763\\
-0.797570013485324	0.392245353521358	-0.858788927314199\\
-0.727135133834651	0.439187572096872	-0.810245505490446\\
-0.656863674494348	0.491748415547409	-0.762986536853851\\
-0.589304108632216	0.535215398766491	-0.710713696252079\\
-0.521841596907772	0.583515855202647	-0.663010546813638\\
-0.459070593961333	0.632181652937738	-0.617375011773583\\
-0.396084333707836	0.68122609357534	-0.566609871526138\\
-0.331537023497307	0.728529095980444	-0.516462479103587\\
-0.270461608280935	0.776666307276697	-0.468661122470562\\
-0.208959096208436	0.82253710485579	-0.418560260672453\\
-0.148109906408346	0.867854260607204	-0.368559657787423\\
-0.0852661901429587	0.911916664075609	-0.322616294682748\\
-0.0281724629784662	0.956549830375345	-0.273431922590461\\
0.0316297453834707	1.00411955573829	-0.226040408533207\\
0.0940424900614943	1.04969457192387	-0.177012415465904\\
0.153463820027174	1.09871927638879	-0.12832482154147\\
0.208426073295889	1.14300127994308	-0.0758349198329008\\
0.263029737410235	1.18294801174318	-0.027244607005956\\
0.309987666860116	1.22848019726555	0.0183252554270275\\
0.355168539900888	1.27011340902465	0.0641514958055227\\
0.400838745159028	1.31232369003444	0.104748933688482\\
0.446210174248702	1.3561230716174	0.14553077380875\\
0.490297226838374	1.39353204803897	0.184628834162501\\
0.53132077982562	1.43449859590389	0.225259351355798\\
0.579360011591246	1.47423522063302	0.265770644211078\\
0.620114687428883	1.5137881427356	0.310008645574089\\
0.662268500042963	1.56344772551497	0.35352676324262\\
0.704181777392747	1.61483448149668	0.393366649469507\\
0.74416992319634	1.67017122458545	0.4359345662294\\
0.786861093748554	1.72853097027624	0.480056910850364\\
0.825863620126442	1.77262520011	0.519936418871072\\
0.867748587436645	1.81846500584132	0.559978643448845\\
0.904348079717769	1.87077411002873	0.601503898989438\\
0.939957131715918	1.91938102343195	0.647163560902774\\
0.984100613984313	1.968429123356	0.687504026488806\\
1.01875351501244	2.01604337703786	0.72948485477501\\
1.04955551295515	2.071497787221	0.76585638322754\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998879902201073	0.240496085513992	-0.99988366606658\\
-0.939370794986175	0.299688628768168	-0.950860526824933\\
-0.873789045122942	0.345583716334724	-0.904156203431173\\
-0.804188423871314	0.397335530731634	-0.85364545886601\\
-0.738232606420457	0.45007556760859	-0.806257935093803\\
-0.673380637037804	0.504234232855233	-0.75674450493024\\
-0.609847130544732	0.562259906775999	-0.704740058997178\\
-0.544257641839152	0.613043902150979	-0.657951432356445\\
-0.474965162789158	0.664304469295863	-0.611695161932119\\
-0.407099820977274	0.724749841543837	-0.558969937446712\\
-0.33348289548803	0.783060905035537	-0.506787300641006\\
-0.26540003473959	0.841948910151505	-0.457250201837349\\
-0.195976614764264	0.897326878189592	-0.409250105902261\\
-0.123554371748513	0.955647713582156	-0.356437774225914\\
-0.0552666572992857	1.00993096643663	-0.308400481284111\\
0.0144717608967379	1.06703826389719	-0.25437161816529\\
0.0911764688052082	1.11871904774566	-0.206025367099183\\
0.163761483087618	1.16945201153436	-0.153264874298582\\
0.237617842680693	1.21996092266649	-0.103993833305754\\
0.31463664029243	1.2789093299813	-0.0549133951063001\\
0.393438353942507	1.33219400122285	-0.00456118324455546\\
0.470623632413837	1.38843610152572	0.0422677329824553\\
0.5526201097657	1.44449013484385	0.0885204495478698\\
0.634651552228326	1.50616302618079	0.136904016950607\\
0.72025096587917	1.5724370314638	0.189311364249635\\
0.794706215447156	1.63153022791049	0.240944076360831\\
0.880896683430186	1.70352199722535	0.295045005811415\\
0.966734560096649	1.76698222317146	0.338746543162434\\
1.05158054734628	1.83490239619738	0.383807170676711\\
1.14501742093597	1.90974711679438	0.428760396921591\\
1.23643583967319	1.97863582803307	0.464731570803217\\
1.32462125867028	2.04379879798905	0.504847827125861\\
1.41534672207407	2.10608913194866	0.539949721838696\\
1.51144870099735	2.16982541766346	0.577831754697006\\
1.59059562940606	2.2382519077932	0.614215323291034\\
1.67620167064393	2.30195908047853	0.648005908040606\\
1.76144098834775	2.36756621870626	0.684560028601531\\
1.85342007642594	2.43203666681135	0.712997443832887\\
1.93248096066779	2.50270747971638	0.742465233245272\\
2.01662392343828	2.55281677520205	0.766402992723045\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998186840084946	0.241238126532768	-0.99575913010429\\
-0.93910655074124	0.295197335550279	-0.94816137861081\\
-0.879566605680491	0.34774384672798	-0.904031152519019\\
-0.815485814067297	0.39518190071445	-0.855337447663044\\
-0.751283235483321	0.447638161782792	-0.807095082872336\\
-0.68777329853078	0.498580686058877	-0.759130780209098\\
-0.623532697387901	0.54981545761173	-0.712553875593714\\
-0.560444288094363	0.596732133763351	-0.669823215352021\\
-0.500923289589524	0.649962270044387	-0.630354768568722\\
-0.439217692788261	0.70269553082119	-0.597529292235517\\
-0.382377505947668	0.753636233053346	-0.565417465490072\\
-0.326986875308349	0.808659484033586	-0.533639240895368\\
-0.276188885195786	0.863493979132822	-0.50445883928031\\
-0.220440558413139	0.922386013886069	-0.476520822699489\\
-0.167307434473189	0.984501715839633	-0.450362731923827\\
-0.115980537432391	1.04575834750217	-0.42361032661191\\
-0.0605358746356502	1.10209660914717	-0.398929354089092\\
-0.0124327974852918	1.16072501346216	-0.371653134877353\\
0.034373815565122	1.22345447538754	-0.342406795347864\\
0.083441933861303	1.28633735897505	-0.315279287820554\\
0.129345241622559	1.3499962899717	-0.286714139511742\\
0.173700219918909	1.40807926239857	-0.261012966568939\\
0.216862447993608	1.46865706647241	-0.23840836540336\\
0.263608652318412	1.53897001686056	-0.205886321889335\\
0.30119146157233	1.60681819495591	-0.181663804550202\\
0.339887347097249	1.6722033398497	-0.155163638663346\\
0.377296124081438	1.73704096989589	-0.129173329717089\\
0.419244588911832	1.80532865269098	-0.103187554488832\\
0.461599638526467	1.874338641162	-0.080219185013098\\
0.500299350194451	1.95379052822162	-0.0602792524145983\\
0.542228900556564	2.02021763986239	-0.0325275099175743\\
0.579641688465665	2.08746259300911	-0.00937972038193605\\
0.623227073988167	2.15365560616595	0.0195321961606601\\
0.665600501944054	2.2253126287606	0.0434950617180265\\
0.712914359812287	2.29086498906892	0.0728816646467084\\
0.762924661189738	2.3626291983752	0.101602939638156\\
0.809700720262381	2.42841258189739	0.128586396792931\\
0.858518206548166	2.49392383211801	0.155222973011852\\
0.908667903130117	2.56441707039368	0.174748914416757\\
0.953441004133035	2.62692835231056	0.193056381098966\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998501463206577	0.240622048850611	-0.997956032982096\\
-0.937380092684389	0.299739589435348	-0.948773765656467\\
-0.87288428821746	0.347166221913456	-0.894320302504629\\
-0.807684610880128	0.396017859973276	-0.835151346077745\\
-0.744529176595335	0.444283635809204	-0.776977159531321\\
-0.684774500862059	0.497270244904476	-0.722827206419273\\
-0.623058659794482	0.552846761725483	-0.674611875493064\\
-0.557856907490218	0.603684184662123	-0.624846806898406\\
-0.496017379702059	0.652288335401447	-0.573934216827273\\
-0.43300214697173	0.697762032164445	-0.529414021468079\\
-0.371599276837317	0.741167709577692	-0.484825068934523\\
-0.309379588785731	0.78443817232376	-0.435807416039495\\
-0.248278621653015	0.823641573001581	-0.391412712832659\\
-0.190766229789827	0.863015670568478	-0.352671634355826\\
-0.132950857574769	0.900897601534577	-0.315171867906392\\
-0.0785247158253818	0.939622352569191	-0.273730439469658\\
-0.0208412267141289	0.977094025030942	-0.236186927751407\\
0.0332996331060053	1.01712525855086	-0.19707575583392\\
0.0849339521357008	1.06091755685768	-0.162941831995224\\
0.143076282026755	1.11128190240168	-0.129669269501444\\
0.20129723334914	1.153573022764	-0.0894201939493836\\
0.259652317216535	1.19729800428796	-0.0599667397297685\\
0.315237186577836	1.24883014064212	-0.024474621888829\\
0.365262307022047	1.29946267625776	0.0084960433227074\\
0.411739106210097	1.35514135094607	0.0410666842690655\\
0.456330172505233	1.39810397050393	0.0749012268964479\\
0.502916568478967	1.4489316490109	0.108553878157218\\
0.550320654886159	1.49342870763487	0.143259081876911\\
0.597633145833903	1.54265003791567	0.186611771047641\\
0.651254439085877	1.58989861541072	0.225795991854095\\
0.706089601716066	1.63824149921117	0.265464746672398\\
0.755232603225867	1.68050412134056	0.302410296115793\\
0.801892633952299	1.72176174228032	0.338168917135952\\
0.851107023511234	1.7598184382646	0.379277603095691\\
0.910045444506951	1.79817423689589	0.419285501841558\\
0.961868295151989	1.84519947095436	0.456521047292635\\
1.01436343173049	1.88725122739054	0.489987371502914\\
1.06542357727094	1.93391401759271	0.52582168386404\\
1.11707626417437	1.98249589454058	0.560983146840853\\
1.16637519937206	2.02691607247731	0.594805476282318\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99941386444476	0.23981958381857	-0.99940192455211\\
-0.935790783494671	0.295973440151058	-0.946644440945783\\
-0.870953484147256	0.337920676615916	-0.895624035090351\\
-0.806049533947736	0.38222421949771	-0.84251474270725\\
-0.740628400801643	0.422809568428598	-0.785407613821271\\
-0.680530627252956	0.462177667265037	-0.732220734954956\\
-0.61755393063427	0.500809723334486	-0.677468006362588\\
-0.553039189053207	0.537744681941029	-0.619959926684529\\
-0.489261787921256	0.578833756878931	-0.563527496873362\\
-0.423585694721391	0.628139430911374	-0.507387672388164\\
-0.358626023549135	0.671992438111445	-0.451438345867636\\
-0.296604452183055	0.718979492251215	-0.394927180571802\\
-0.233893918287818	0.762479305620649	-0.344553852355452\\
-0.167105297522116	0.806033925762861	-0.294907121623299\\
-0.100313319827201	0.85173982157492	-0.243923305374739\\
-0.0347131128428459	0.899667072910527	-0.188163931381889\\
0.0318992766133705	0.951575077588766	-0.1292858123271\\
0.0939587124992772	1.0023203271045	-0.0722763537621054\\
0.155471461729173	1.05367549544397	-0.0178115528891776\\
0.217321132960819	1.11225191889027	0.0369684793519381\\
0.27554528441688	1.16293097072858	0.0897093697707379\\
0.326660311383942	1.21901725621047	0.140407098341125\\
0.385442278344885	1.27733913367489	0.19077295311036\\
0.442732556338243	1.33109214322283	0.242704778539406\\
0.496396603946829	1.38733670957261	0.29438914405709\\
0.555329633902037	1.44313816929292	0.346349961766558\\
0.620033187587347	1.49933564394949	0.390839968070357\\
0.681681133192265	1.55385734626562	0.444059387189137\\
0.744135120431133	1.60681685856481	0.497028103161948\\
0.806308037579827	1.66159800091263	0.548153405497722\\
0.868407163507737	1.71062740831277	0.599199521246646\\
0.934676220674764	1.76448356459484	0.647910551823576\\
0.994983441668676	1.81627499769647	0.706145087474844\\
1.05601828200952	1.87000952781779	0.763689518130537\\
1.11861872131484	1.92268947511914	0.822631392863396\\
1.18239123002556	1.97118733942239	0.883338236373165\\
1.24547410558845	2.00886829986752	0.942097873926395\\
1.30541690925659	2.06605985835185	1.00160730671751\\
1.37020522015701	2.1142811032267	1.06388348153475\\
1.43553978055996	2.15908326526873	1.1259099546486\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999628468123505	0.239790642200563	-0.99897927759309\\
-0.939925800908706	0.296042592806576	-0.949064983131013\\
-0.875266349827194	0.341981759663927	-0.899805478039031\\
-0.804988157029969	0.388379733543896	-0.848054750657497\\
-0.730863878676326	0.439183077783096	-0.798524228362854\\
-0.657229628784629	0.486499827915499	-0.74908000212884\\
-0.591572705893785	0.534692114499472	-0.692385359734553\\
-0.523491044983277	0.580256089716363	-0.637898006433409\\
-0.457554556262484	0.626900853575511	-0.579719222240134\\
-0.389307561274564	0.675277867740183	-0.520757303740208\\
-0.321688393728467	0.722238445144696	-0.462161158743266\\
-0.261025051333469	0.772806747316398	-0.398790377925144\\
-0.201063345419251	0.825260249199859	-0.33289621954988\\
-0.142939694616152	0.880967357489524	-0.271365782089549\\
-0.0813910921469937	0.936155200593185	-0.207630848641898\\
-0.0210017469487869	0.98501080558381	-0.146600239202634\\
0.0408571880641842	1.03141430640984	-0.0835191396259772\\
0.102559629102903	1.08339897598826	-0.0226885379086642\\
0.163285941463538	1.13423531389365	0.0368329525571538\\
0.219276401783637	1.17918896804226	0.0982186832816128\\
0.276765559566223	1.23679105028662	0.163320752261187\\
0.333328969610198	1.28749214820276	0.231279035800933\\
0.388619171172642	1.34493843504955	0.292770640756229\\
0.444828414861031	1.40285138095071	0.357407266050898\\
0.494106637458335	1.45481133434207	0.417668955022045\\
0.551519976997145	1.50744282891953	0.479277005462752\\
0.609527334442341	1.56374080085298	0.533384600137526\\
0.660641882932611	1.61065360475036	0.591186262409852\\
0.707875668819173	1.6616160999572	0.644315273213129\\
0.759877049222264	1.70183406754071	0.698100463494905\\
0.807391382574032	1.74113329991917	0.747273110092868\\
0.860306972237768	1.78248401822611	0.806325190862904\\
0.913578169490901	1.82597288384577	0.87063592936746\\
0.969532391995316	1.86960373815914	0.930738166463832\\
1.01990463281503	1.91287429474502	1.00193963235164\\
1.07299453257888	1.95180604141512	1.07103755000408\\
1.12383537811516	1.99496799553102	1.13293339534748\\
1.17997811518489	2.032273860388	1.20544540890979\\
1.23499557658421	2.06542254474042	1.27272747378511\\
1.29846587084545	2.10068936214979	1.33756443870261\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999289387007216	0.237332812311051	-0.99865554709324\\
-0.936795955100432	0.295679216182619	-0.947864624687105\\
-0.876927253238595	0.343276485769654	-0.901835879960475\\
-0.807559195861177	0.394613411621275	-0.854747083355907\\
-0.743768546633476	0.446741482146726	-0.809483242443629\\
-0.678382896751087	0.498546391877843	-0.768793193958187\\
-0.610558805239572	0.546513126155076	-0.724701612024884\\
-0.544798088817717	0.594782594672072	-0.682477760140318\\
-0.477717423893348	0.644362771969552	-0.639171197285377\\
-0.414418358748862	0.691799180516605	-0.600266258985882\\
-0.351400665563637	0.73769750361156	-0.560931573073746\\
-0.285030344315029	0.792222367499755	-0.520799493921138\\
-0.215875518663512	0.839978188612703	-0.482957520864315\\
-0.150297843540294	0.886646079218679	-0.447237042402936\\
-0.0834243279194481	0.941460547367289	-0.410865954985957\\
-0.0120904358143467	0.989775199494328	-0.368771018321348\\
0.0604389596442129	1.03455854433696	-0.321992784550233\\
0.128151640113722	1.08341974135171	-0.279405541600614\\
0.196461201678463	1.12184412337843	-0.236337765105618\\
0.261364979629248	1.16835261839804	-0.194519704650955\\
0.321670162964917	1.21348011410584	-0.148443088243086\\
0.386880370280435	1.25469593481258	-0.101284454693346\\
0.450604139635742	1.29798441047623	-0.0553452158533105\\
0.519616769322175	1.33857252486657	-0.00927014479227918\\
0.586521906558447	1.38208814561038	0.0334872371659635\\
0.651479688190949	1.42906114369178	0.0822244820957161\\
0.715133057155426	1.46881180996613	0.134969932829681\\
0.778497133532508	1.50840607572028	0.184921140176153\\
0.844392620888717	1.55205640548613	0.235492388502672\\
0.913743415717288	1.60113650258431	0.288495733080519\\
0.978645205210958	1.63933218766213	0.338369617629305\\
1.04825500823173	1.68263559166572	0.393018859135845\\
1.12063304513119	1.7377561187081	0.436865577122685\\
1.18924802745821	1.78313708669981	0.487671860194042\\
1.25671338534207	1.82607100488179	0.540897220914599\\
1.33248467847619	1.87102929043667	0.581395060032421\\
1.39846247339973	1.91831311160546	0.624230507074932\\
1.46414328393671	1.9681844481162	0.672364141523025\\
1.53497308785455	2.01054778187278	0.70841517391463\\
1.60973388371968	2.06134501267281	0.757824264378024\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998744597993324	0.239697364611478	-1.00082330309869\\
-0.934967296140122	0.29989064312524	-0.950157034366223\\
-0.86972779897256	0.344447275570136	-0.898492931569805\\
-0.80380434347782	0.395393403286442	-0.847069314899717\\
-0.736630584077776	0.442494611847942	-0.789790776091889\\
-0.674003912521172	0.487020472623881	-0.73099047887085\\
-0.611323579525427	0.536326358550417	-0.679711199720687\\
-0.547947112786439	0.579137292523701	-0.625531639441308\\
-0.481311197084737	0.625684368217938	-0.576752741050633\\
-0.409642341342085	0.671437090276521	-0.524345978719481\\
-0.336718700514058	0.719340455289502	-0.468647733249641\\
-0.263515877624212	0.764537815183044	-0.412902093600487\\
-0.193170181448085	0.817074647324963	-0.355392900262836\\
-0.121621247147764	0.85974469495509	-0.296083232311909\\
-0.0529290729005914	0.913964513283499	-0.234183540893584\\
0.018066553158035	0.967257398950404	-0.174826262009692\\
0.0855842031244479	1.01565889554435	-0.109527439163188\\
0.153506741555135	1.06719276334748	-0.0450340921768153\\
0.220285061205617	1.11310777866069	0.0210252373313124\\
0.281497338579451	1.17102949831046	0.0829191434970286\\
0.339841322499021	1.22475310286617	0.142844238515142\\
0.401649742735817	1.28167213514423	0.201115439123611\\
0.463472286329777	1.32816451866386	0.255587450212393\\
0.529027501161274	1.38937239025773	0.310707537689259\\
0.596295164673068	1.44161626270088	0.360966187991806\\
0.665240306388588	1.49373270512595	0.418294113130643\\
0.734892174207189	1.54703805668162	0.471188238947233\\
0.802609297475846	1.59677301506572	0.519727335807\\
0.876217114705428	1.64423008323368	0.577104341061865\\
0.946329772400645	1.69834838831746	0.636998461431551\\
1.01487012611064	1.74117426820574	0.693202951143347\\
1.07895364097138	1.80104867708122	0.747922193424177\\
1.14008865783622	1.84884542085864	0.792570040054611\\
1.19945130966865	1.90334134584269	0.842317791907883\\
1.25928968363361	1.96176365750833	0.888586581774754\\
1.32203621734675	2.01759594992835	0.933677571088026\\
1.38257667373151	2.0641937818398	0.978972812005777\\
1.44072191073415	2.12339258232747	1.03295774611234\\
1.50546098626268	2.18206423228079	1.07036803043518\\
1.55975887555877	2.23136827473192	1.11391344887868\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998885511378266	0.241910664800918	-0.996976547477393\\
-0.940040387614954	0.29766777320707	-0.951626881813066\\
-0.875761564352633	0.347260468102953	-0.907998660757468\\
-0.816470024118318	0.392983354135737	-0.858395523848572\\
-0.754390311738232	0.436969118715538	-0.807615616507622\\
-0.696814774846039	0.489813934789821	-0.756835415722019\\
-0.638662270138816	0.541508877072344	-0.704843504179646\\
-0.574028968528997	0.591552378645295	-0.647513506425095\\
-0.509217796623769	0.641755340240551	-0.592825936813614\\
-0.443576874144499	0.690388034449658	-0.536188529144945\\
-0.383392334500443	0.745883388683918	-0.481844860460854\\
-0.32076791702083	0.799986152509635	-0.427792737651208\\
-0.262775469604114	0.850507944820221	-0.372664024183134\\
-0.205120722121782	0.902966353198475	-0.317669078495082\\
-0.146466695321946	0.95216406785298	-0.262405454807257\\
-0.0944402357188441	1.00064680946135	-0.211676887176349\\
-0.0387710902211556	1.04811022977455	-0.155471755459173\\
0.0155118148154992	1.09073778226011	-0.100539150071169\\
0.0740883287702382	1.13531226263472	-0.0482031999438352\\
0.133198466176663	1.17946127642741	0.00682531674891407\\
0.186390976823255	1.22438350327784	0.0622041620040903\\
0.240426482745683	1.27381480766936	0.118910359755193\\
0.298220804718212	1.31774535893661	0.182176961892837\\
0.350962282352541	1.36020652557454	0.240485424587223\\
0.415578450780406	1.40564377342666	0.305952817557809\\
0.470425707641884	1.44524272280929	0.372190904752373\\
0.529456695012825	1.48131013532241	0.43712942967256\\
0.585962618128176	1.51817796589832	0.499198162661889\\
0.637974139056772	1.56445863246761	0.565512641325222\\
0.694442306998844	1.61081872437219	0.633828917433982\\
0.744965992305821	1.66223244724247	0.702182438107963\\
0.798239336855592	1.70818277921315	0.770943857544714\\
0.847036322537959	1.75413794824888	0.842854623769122\\
0.900452089866363	1.79544184131232	0.915267609387747\\
0.948305547722496	1.83679549021743	0.983009012267143\\
0.998056758900664	1.88047852779191	1.05674893858474\\
1.05288580690814	1.92371468087948	1.13069712490679\\
1.1109080787291	1.96615330191371	1.20299207227131\\
1.171317220047	2.001858577902	1.27624387367332\\
1.23238388325872	2.03815751318162	1.34446825975575\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00001242079505	0.236996152839202	-0.99819153226049\\
-0.934071827168765	0.296812721566474	-0.94900119376642\\
-0.869154732172692	0.344744304962989	-0.900387001894552\\
-0.79642778770078	0.394936458189387	-0.850653752790028\\
-0.724114088376697	0.438060104253512	-0.801718915695451\\
-0.650537362239834	0.485391800508191	-0.747573480286097\\
-0.57773296631891	0.529078210200821	-0.692855667079673\\
-0.504445910849418	0.582120446020019	-0.638795725563779\\
-0.429242111180558	0.633573562556222	-0.581522457967665\\
-0.355596050621327	0.689397248334908	-0.529820957518047\\
-0.277605823264592	0.744025645700843	-0.47633578096978\\
-0.199464303040165	0.801486135250879	-0.41671253912194\\
-0.122780568721429	0.861266032837976	-0.362785688665567\\
-0.0440789177556352	0.915108996921414	-0.311361944494187\\
0.0376143232755785	0.964246304458507	-0.259084321432278\\
0.114555016102637	1.01717209054488	-0.197963055414828\\
0.187652303337601	1.06501729941302	-0.137974963125784\\
0.26584750854522	1.12235537817069	-0.0722826722553435\\
0.342214514737491	1.17232645876298	-0.00694439717821829\\
0.425095419691448	1.23003949135393	0.0603241347804975\\
0.506051039720301	1.28562175609566	0.127239496273135\\
0.588726789046525	1.3455447752446	0.196363111926027\\
0.672750288388868	1.39837087970005	0.266023417678813\\
0.763300391205067	1.4537587327465	0.340530625352004\\
0.845050678727478	1.51670035775515	0.415465343803769\\
0.933384432083729	1.5761458834542	0.491962714885336\\
1.02078988600718	1.63705539115459	0.571323212294579\\
1.10603932995362	1.70225133901559	0.650189837848793\\
1.18831784754637	1.76770875406839	0.733853873662714\\
1.26777717813386	1.82873884287846	0.812237617839167\\
1.34952679680076	1.9049332078562	0.899655597811849\\
1.43023232104486	1.97248192837176	0.982938615477784\\
1.50815864026067	2.03757105632708	1.06420760837613\\
1.59801144846906	2.1096956557521	1.14491569803146\\
1.67678481840977	2.16956626187837	1.224696605501\\
1.75765028520496	2.23070549876961	1.29624968926503\\
1.84149806923614	2.29541484691098	1.37234131875728\\
1.92514715181643	2.37122963631975	1.44830650358269\\
1.9971120621971	2.43906794267888	1.52812329081828\\
2.08444550915334	2.50715141416051	1.60504175661068\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998959593193632	0.240823525972835	-0.999191176356675\\
-0.937010795032799	0.300216708677304	-0.950798757480133\\
-0.87334516007607	0.346598183946491	-0.898595061458361\\
-0.807243845062648	0.395176248501185	-0.846686296870997\\
-0.738726750337258	0.44901308854195	-0.792835340129378\\
-0.674809951292105	0.501516665581982	-0.735094708555018\\
-0.613246013689922	0.565083374984484	-0.683987868051571\\
-0.54891879701058	0.620154772982619	-0.626935790129387\\
-0.494581278850229	0.678818587696362	-0.570675149732432\\
-0.437961561225523	0.736192162727018	-0.510339127697848\\
-0.382006970165087	0.792729988358544	-0.456813446877408\\
-0.324940245612966	0.845608906805838	-0.406925583598001\\
-0.265459355197348	0.901028253007747	-0.358317956109875\\
-0.208780879225109	0.955769508095268	-0.312279004473023\\
-0.148822244643829	1.01457655363819	-0.268603560105727\\
-0.0903744801752249	1.06876803256187	-0.224527404626605\\
-0.0304028315660734	1.1214519565387	-0.178812812022271\\
0.0261867198232864	1.1799634297082	-0.135150437802118\\
0.0842436869465917	1.23110491121767	-0.0898054785672626\\
0.146511414082153	1.281126012722	-0.0454046688802251\\
0.200467321021819	1.32709893484523	-0.00216007815982188\\
0.257103877359511	1.3730911663498	0.0435746712649696\\
0.309144408186614	1.42404195628767	0.0868939116132905\\
0.360342798483346	1.47345591400591	0.134641943185379\\
0.414149720803435	1.5178097101618	0.18064810862728\\
0.472514186448061	1.56764316127003	0.229361709620298\\
0.527780466255169	1.62124292067037	0.283387300713208\\
0.581130005235912	1.66993874378876	0.342200478945902\\
0.634407725475579	1.72488377066727	0.396223324057947\\
0.692139517135441	1.77217418895066	0.454341751580407\\
0.743921075392271	1.82214649284332	0.51454618724282\\
0.79654300926419	1.87985002499337	0.577410328918531\\
0.854115664323511	1.92543174209933	0.644217003467266\\
0.90022435501774	1.96793687696675	0.709619137513361\\
0.966890599445676	2.01567905004838	0.781902994752975\\
1.02199232452066	2.0599629255512	0.849641584649331\\
1.07923862695916	2.10860169005699	0.922623894353172\\
1.13476459690299	2.1487117346492	0.992759550697976\\
1.19308301456914	2.2052443731381	1.06277004046379\\
1.23738648649508	2.25464620386159	1.12787503622771\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997171050210162	0.242309090692241	-0.996856148079034\\
-0.937953212107463	0.291755435391893	-0.950300294838887\\
-0.874338901098554	0.338380256899547	-0.897086027350147\\
-0.809936557705549	0.386072686519136	-0.848017856588324\\
-0.745226017347575	0.428677698644661	-0.794412132155935\\
-0.682260929886819	0.46539293664249	-0.741298955255845\\
-0.614482118094976	0.501047798801286	-0.686561242554906\\
-0.548526305100165	0.542715800119847	-0.631653466289102\\
-0.485189318634579	0.576620933496199	-0.574101718415877\\
-0.422431078751044	0.615974476458091	-0.515009777648744\\
-0.361523563236864	0.654856634204266	-0.456808022333485\\
-0.303253140899515	0.694586018559849	-0.399680829704244\\
-0.246141853522201	0.728963767175671	-0.336187767877396\\
-0.18904891675754	0.767986409842892	-0.277333602911615\\
-0.134219016517722	0.808695614020911	-0.215408219074509\\
-0.0747573033008048	0.843606849702167	-0.156692217518261\\
-0.020439103678019	0.880994131762678	-0.100807855237628\\
0.0308231566903629	0.920606330591664	-0.0416489872792073\\
0.0808987896925517	0.960693259966886	0.0132311483872555\\
0.13503506867386	0.998287652151354	0.0690422961662859\\
0.189121798651164	1.04605663037633	0.126899421908199\\
0.241632307076704	1.09533521782169	0.18321581161012\\
0.289088449535143	1.14818569882429	0.240838878250628\\
0.341635793937148	1.19844786306698	0.298515739981637\\
0.390620499027097	1.2514446960535	0.358623049495604\\
0.44037802866175	1.3057942783143	0.423754115037171\\
0.492366191100857	1.35979320576295	0.487627553340278\\
0.546959208579579	1.41876008517543	0.548116684093643\\
0.604939244749512	1.46904829359612	0.607578124750659\\
0.660573994833797	1.51906110742651	0.670788838088915\\
0.714346576479404	1.56530781521669	0.734290947927073\\
0.773232220495355	1.61769114305016	0.795908073882546\\
0.827056078168975	1.6685483539366	0.865222302470622\\
0.884649168799789	1.71609847453967	0.931142573225979\\
0.94279561381222	1.75541818859283	0.996761328191133\\
1.00365240816101	1.80281039374679	1.0601130003862\\
1.06139464529507	1.84850973278397	1.1218372490159\\
1.11176811346607	1.9064506906578	1.19580671838589\\
1.16752068001643	1.96114731062464	1.26199259438727\\
1.21242801334302	2.01176867289048	1.33151190333676\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99881542207184	0.239720675091591	-0.997009706141376\\
-0.93765438649253	0.293302287911362	-0.950338539456461\\
-0.869224040670987	0.341062677973897	-0.908219846069401\\
-0.802830145121424	0.384962598225273	-0.860089905537413\\
-0.736439119814415	0.428485983725362	-0.810663876648319\\
-0.6720725014157	0.473118919162488	-0.76157666135308\\
-0.60245268510537	0.512837574179635	-0.713395481161917\\
-0.535784511961406	0.553593169948548	-0.669184674280052\\
-0.46943362475402	0.590316720273654	-0.62140876858919\\
-0.405174768763193	0.627116208757717	-0.567639410473795\\
-0.341413477227322	0.658247247352008	-0.511749739559889\\
-0.274952109312681	0.686808168155472	-0.452594442425038\\
-0.212133355944118	0.712822282752146	-0.392052513313729\\
-0.150238256484949	0.747561761275763	-0.33143886344707\\
-0.0880784706303454	0.779728865981586	-0.274808037601344\\
-0.027241009211033	0.812778617646553	-0.217757421531806\\
0.0295094920265874	0.845846977734625	-0.158777798795608\\
0.0844644599779759	0.87003809891487	-0.101148612229172\\
0.136126783426729	0.901627949880876	-0.0450344538206197\\
0.185331432392828	0.934700539268137	0.0137375670675768\\
0.239245711797525	0.970980696186618	0.0698762516650012\\
0.293065230290556	1.00615936608342	0.126745002362658\\
0.3467361272706	1.04080800777651	0.181111997680564\\
0.40050250221656	1.06991908897503	0.243173940796566\\
0.45338491730481	1.10579333147593	0.298056240101713\\
0.505927408420464	1.14584979740738	0.358049174784228\\
0.557187442254682	1.18059088957487	0.419798414594443\\
0.612581072679843	1.21840820756129	0.480505434749133\\
0.668686584045907	1.26003803946999	0.538491828149655\\
0.718193141856078	1.29689957895612	0.598880508895309\\
0.768156830112073	1.33572758034375	0.660334870951474\\
0.823054801709109	1.37014354126151	0.721016806931345\\
0.872970513785764	1.4010853048614	0.778265407102967\\
0.916461767262063	1.42736373941219	0.841438082322793\\
0.9581234247532	1.46346311122217	0.908784035508842\\
1.00940237580738	1.48260922256318	0.977998602327537\\
1.05518353083684	1.50182569737712	1.04318962620448\\
1.10058996882661	1.52886099630075	1.10921458286862\\
1.14632596156738	1.55772619054662	1.17340932362644\\
1.19255061153981	1.5795581201526	1.23465112685251\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997012033215349	0.24330068421086	-0.997794551516377\\
-0.935046798425955	0.298331143526988	-0.948599736134172\\
-0.877277236483502	0.342459339848217	-0.902726415850275\\
-0.814669154167901	0.393082259395234	-0.856981882805012\\
-0.749920772611216	0.437942885646406	-0.807679066289984\\
-0.683661094653007	0.48777849040452	-0.755918285862468\\
-0.615854413113115	0.535417746192292	-0.699236077390068\\
-0.547529425554012	0.585554814945076	-0.646623772223913\\
-0.480691576204443	0.634305277389931	-0.595065014043382\\
-0.419153196352777	0.677119078228366	-0.539491424340906\\
-0.355294414861889	0.721092523051041	-0.486892311783569\\
-0.2908482045041	0.76611903355803	-0.431675315929284\\
-0.223698482560711	0.813334032213213	-0.37485043208904\\
-0.152302963352282	0.858028083916582	-0.32025107240638\\
-0.0841121191825706	0.914284559544938	-0.262546904637881\\
-0.0112241195221479	0.960153916225502	-0.207302417851785\\
0.0611541607231782	1.01720944185419	-0.154038639758797\\
0.130875427844638	1.07857116786437	-0.0947173547830037\\
0.200704812438192	1.13373001560595	-0.0419674127951958\\
0.274121980040014	1.19084234531123	0.00894577875177411\\
0.347242506776232	1.24223765103077	0.0546834713958657\\
0.418169622218477	1.29420207593525	0.0981704153936394\\
0.493912617695954	1.3510320642693	0.142897087055774\\
0.567470216808397	1.41680221662017	0.188926013040699\\
0.642893850621634	1.4797344126437	0.235581895090041\\
0.712250478568749	1.54312912430285	0.277834221027388\\
0.781320156877461	1.60995409592037	0.31834794263671\\
0.851328636946908	1.66759827741845	0.356788027957719\\
0.922317692307335	1.73136632070841	0.394917838158719\\
0.993139273470782	1.79275987572677	0.433501894570389\\
1.06208109058572	1.85260995675399	0.478472772888404\\
1.13085998158348	1.9080268871646	0.526415361146105\\
1.20561838425786	1.96031745717501	0.573650695661233\\
1.27940775815342	2.02909199764573	0.615813676925079\\
1.34812676516791	2.08579132681223	0.662019367126311\\
1.42323235006741	2.15256453372894	0.709438559981014\\
1.50163366840412	2.22009740292004	0.768343110669741\\
1.57865052890917	2.27819189196283	0.825738759724162\\
1.64886201638829	2.3423943225935	0.882816717518549\\
1.71839996723213	2.40376474448927	0.939394887715484\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998176300892813	0.237865833133155	-0.998194406771928\\
-0.937303139918043	0.301206038514602	-0.955159411637351\\
-0.877955500618571	0.341612321654935	-0.901700143340558\\
-0.815697139260197	0.38866548598159	-0.847394338464941\\
-0.754143895367212	0.430870756298495	-0.795036705558929\\
-0.695123827072046	0.47192298746436	-0.740694369683829\\
-0.636612473235756	0.513406346603183	-0.689101644847527\\
-0.575032286854936	0.553967385215815	-0.638111316675945\\
-0.513083470553701	0.595876225786883	-0.587766782640912\\
-0.444961479073543	0.640597481984597	-0.537032591693204\\
-0.375109129653081	0.686710488668791	-0.487021612306725\\
-0.305788006071599	0.738137242989012	-0.436234430769775\\
-0.236235057231604	0.790671883468174	-0.386684809936003\\
-0.166272574417097	0.844525951527236	-0.33937749510591\\
-0.0957488805514085	0.899234206104683	-0.294071544167977\\
-0.0287840323751033	0.947013920874275	-0.251677305336781\\
0.0370096021764849	0.998177322843597	-0.217118878873802\\
0.106559765166078	1.04915798202384	-0.185801895940089\\
0.175524576186528	1.09731864515887	-0.159031018255411\\
0.247090072300033	1.14257724693	-0.130554407973902\\
0.320650086654296	1.18591216187324	-0.0992287650876434\\
0.396506940491463	1.23054750219539	-0.0663487510487194\\
0.473262288155237	1.27090201263435	-0.0358039625641331\\
0.547150548605702	1.32022030747578	-0.00922259580246202\\
0.617612867216872	1.3638636895872	0.0196621500621873\\
0.694060621126363	1.41300564579005	0.0496943384016945\\
0.766817069046539	1.4620538715338	0.0795899787416229\\
0.840694727531361	1.51379585644396	0.107119387534553\\
0.916371968829657	1.55932985424325	0.137390991854598\\
0.986270069766298	1.60614246401446	0.157036274438943\\
1.05994897286179	1.65659647997805	0.177171941443293\\
1.14236102668261	1.70095270256798	0.198267012071467\\
1.22077245933225	1.7449746750989	0.217168008824423\\
1.30174902847641	1.80233641298785	0.236217088454865\\
1.38498294775674	1.84450456804972	0.257150003929835\\
1.46323256195656	1.89905012349442	0.281349483875322\\
1.54165447658842	1.94970008162033	0.299185692966051\\
1.61540358604717	1.9928729763946	0.317860407036865\\
1.69469191291839	2.04210792162139	0.335359285789529\\
1.7690063979206	2.08325071458976	0.348953423649663\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999026809756535	0.240084072736964	-0.997186525363316\\
-0.937873815393769	0.28967113699289	-0.947090346365476\\
-0.876860272021384	0.336162596714522	-0.899783480302242\\
-0.815991866953933	0.374145979761952	-0.845304774590324\\
-0.751994476824377	0.415632959899356	-0.794475312091002\\
-0.686778194362638	0.458797438851635	-0.739701187755375\\
-0.627605385818242	0.503830515606959	-0.68005789915831\\
-0.566547545387096	0.545637617384054	-0.622607224593526\\
-0.503936658596177	0.594855401902417	-0.564993427143466\\
-0.438320011588788	0.642782608333275	-0.504658429485865\\
-0.375478476232125	0.687192464260465	-0.44526305176219\\
-0.308159911482955	0.73004697263157	-0.39000716087015\\
-0.241156607477187	0.777411022254915	-0.336463856328745\\
-0.174061770631356	0.82403155585738	-0.277345976009463\\
-0.10486370531114	0.873540001962725	-0.215885276501215\\
-0.0368351010875903	0.921968606119207	-0.154301419672757\\
0.0352965784408696	0.969923748653492	-0.0985417381874972\\
0.107365650539453	1.01483411074924	-0.0439649237183216\\
0.17852823118301	1.06499157184381	0.0123500405207406\\
0.252988118991231	1.10798188326143	0.0692998063376193\\
0.324674321103164	1.15050947084429	0.121003339138511\\
0.397949577684284	1.19501616192912	0.180555936746498\\
0.473364431316479	1.24268040914959	0.239097947298748\\
0.545629887653631	1.28511754885857	0.29474247897868\\
0.624062823757318	1.33446554971271	0.348368203238439\\
0.696902145321275	1.37974103052407	0.39702875778487\\
0.765864186848373	1.42323863456084	0.448953727889677\\
0.835407573261454	1.47151330209006	0.496716204694803\\
0.911822953534982	1.52218291835479	0.545612252387766\\
0.987355304340101	1.57533580662666	0.597840773942296\\
1.06699119232964	1.62074241684759	0.640775965105837\\
1.1443542979802	1.66500212822931	0.694792355215661\\
1.22386349796091	1.71069188308638	0.740759768098063\\
1.30120078908873	1.75939351204546	0.780265499927767\\
1.38056713543597	1.8047598494121	0.824418111341939\\
1.45858501764373	1.8591800544068	0.867882324642663\\
1.53586213295151	1.90467116231381	0.911349175518199\\
1.61166310691167	1.95393255513782	0.950029641586803\\
1.69261146201018	2.00780060703468	0.993757001465706\\
1.76463446750705	2.05253411494051	1.03503570205977\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997879915141782	0.240723834463188	-0.999168889014659\\
-0.93748846371567	0.29578431763191	-0.949112663857146\\
-0.877506879767706	0.340666471202947	-0.901367203309815\\
-0.81828102223304	0.385778399581687	-0.851568414035801\\
-0.758475161648497	0.41728631044418	-0.790800486192482\\
-0.696758803682568	0.450605705924523	-0.733853644270089\\
-0.63012978521123	0.483857723835722	-0.676504194955924\\
-0.559901449700274	0.51515558376121	-0.620472334296321\\
-0.486488222387591	0.548557895308757	-0.560535094181325\\
-0.414254584382845	0.58645423104225	-0.50402883411144\\
-0.34326554769929	0.620158009652069	-0.444362201889022\\
-0.270252541405304	0.656875971545244	-0.386990669966016\\
-0.196781722409483	0.691933541867233	-0.327018374141601\\
-0.119339712032173	0.728207606773953	-0.270446554979799\\
-0.0392375618379667	0.762284876798912	-0.212516762445096\\
0.0415057536030486	0.804345008496095	-0.157295862094667\\
0.121531736053101	0.844624971425868	-0.0991319209041784\\
0.203639614171569	0.888855805124475	-0.0394044528791185\\
0.289487572404761	0.928857570711002	0.0231126599104726\\
0.376117204545984	0.968847786826805	0.0854360726969179\\
0.465095317817891	1.00740476415502	0.146591123438999\\
0.557493651169457	1.04422051330196	0.203524848471919\\
0.646824089656116	1.0780964891026	0.264323063934983\\
0.742863385230756	1.11676734553909	0.321822907861678\\
0.837293289437147	1.14754467520788	0.378478008567543\\
0.930407683833772	1.18480623858365	0.435963850931195\\
1.02223084245309	1.21310923073638	0.493826434766483\\
1.11237642567779	1.24304141275884	0.552845848946321\\
1.20135571679794	1.27085977331896	0.607994156445073\\
1.28703691402899	1.29764923427642	0.66330445628818\\
1.37928290914193	1.32455573233626	0.723390635976518\\
1.46633572506791	1.34360319370611	0.784467614375736\\
1.55746169070873	1.37249197476557	0.839519989063708\\
1.64768587859859	1.40569684452051	0.896841338311787\\
1.73632235954012	1.43182115355377	0.95415872997896\\
1.83167783360269	1.46284562124802	1.00858384733011\\
1.92885825317725	1.50539079342544	1.06530005971972\\
2.01950827512859	1.53759128973342	1.11422387640636\\
2.10790145732014	1.57350020728463	1.1586601154678\\
2.20074517062483	1.6147083344714	1.21414273416725\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998900049507609	0.23946258346467	-1.00236186302348\\
-0.93806067009773	0.302519151556484	-0.950950613184611\\
-0.875000445130725	0.34699679525257	-0.898855919643974\\
-0.807523332820102	0.399939492504463	-0.851285822771237\\
-0.738732635501012	0.445773708896972	-0.796963483493859\\
-0.669092704552241	0.501131436994574	-0.745389357327111\\
-0.60005637424219	0.548687998038143	-0.69339381968737\\
-0.533763555398126	0.601989143068871	-0.640513674384112\\
-0.466344084745919	0.654606823009821	-0.586634068745826\\
-0.398007404048346	0.710458816879273	-0.538198073873161\\
-0.327189986256386	0.759940545504296	-0.487007320007984\\
-0.257946654787438	0.809827569760894	-0.43996819690865\\
-0.191281519487314	0.861244261710227	-0.390965179810164\\
-0.12319918263032	0.911170938031984	-0.338469896876595\\
-0.0529063399520557	0.960457796370175	-0.284931000275585\\
0.0121370572840651	1.01574173164898	-0.229259852347004\\
0.0765303206470667	1.06787582952735	-0.170580592335158\\
0.143069308250466	1.11454289464276	-0.109509190008538\\
0.213559308238234	1.16392499238551	-0.0477897791321512\\
0.28721610406568	1.20789589857908	0.0114510218586177\\
0.358532529241753	1.25616075697514	0.0722959106392453\\
0.429327405177635	1.30578607630807	0.134477890687541\\
0.497203519831442	1.34870442139244	0.203180353825679\\
0.562254232382814	1.38330899227083	0.272396949975959\\
0.627976942961598	1.42390989812496	0.339621055467874\\
0.692711245350603	1.4621327251151	0.407176703813703\\
0.762052428146664	1.50546194634553	0.471666439366706\\
0.827083674656355	1.54118103022161	0.533528892923807\\
0.890655771335466	1.58813836406917	0.599556143715644\\
0.954075158083042	1.63126448288713	0.663433784543702\\
1.02342161611523	1.6765237438917	0.71983928635955\\
1.08952057837475	1.71923291006883	0.788377876124591\\
1.15523463036122	1.76660637978147	0.848800343627862\\
1.22134094805314	1.80706547855688	0.911423939221318\\
1.29078921686894	1.84387595527152	0.97058517630706\\
1.36389256135558	1.88184790069749	1.0292848380178\\
1.43414786255193	1.91928223170295	1.08661624506537\\
1.505150003754	1.964961398413	1.14547873735732\\
1.58129992660558	2.01361853179068	1.20726886686901\\
1.65858077122085	2.04374268460611	1.26623010975458\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998224655000947	0.239227642880987	-0.999584344680839\\
-0.938183365774556	0.296710244772038	-0.946828230357148\\
-0.879421108616024	0.342070775244995	-0.900653004904123\\
-0.82166056995277	0.388358721989544	-0.848728249590131\\
-0.758672746177095	0.437676404337165	-0.788815227408785\\
-0.696234678416448	0.483323644158982	-0.729668316975941\\
-0.630062237071506	0.526957723359955	-0.667599634269856\\
-0.56084383392734	0.573351786524257	-0.607117278261738\\
-0.494568391194088	0.623461572408495	-0.543282847000905\\
-0.430201062649796	0.67302141323129	-0.487191414986097\\
-0.365669219281314	0.710817066887927	-0.429540589155897\\
-0.301635764688841	0.757472276670488	-0.374631948451446\\
-0.238711485346451	0.794631524275093	-0.317800635707675\\
-0.176862364651176	0.832099208634916	-0.263700362004811\\
-0.113587870139848	0.871146482061936	-0.205391907212626\\
-0.052673869772478	0.906205089617722	-0.144114067397178\\
0.00804271305616219	0.948575148488696	-0.0829298377588602\\
0.0674849271209098	0.982415880306125	-0.0180213627134236\\
0.128903075544697	1.01730880235047	0.0530535798275169\\
0.190907749431681	1.04886893016138	0.121320853201782\\
0.252379156510826	1.08621983747133	0.193804436751609\\
0.315139499419469	1.12452651095244	0.26797162831777\\
0.378953618905509	1.15149262954047	0.340684298480034\\
0.442835878587877	1.18590449879145	0.416311108173326\\
0.505513346867512	1.2138013079254	0.484497381543919\\
0.566919430330379	1.24261920680413	0.555585856389909\\
0.631971287720878	1.27395118423471	0.631424174361061\\
0.693379736982473	1.30330890834518	0.706850974285168\\
0.753057309240758	1.33605743490273	0.779416091847091\\
0.816047411858848	1.36629210562833	0.853668317339531\\
0.884083930531003	1.40540869704547	0.926000431825431\\
0.947072681365749	1.43618280163544	1.00001698100536\\
1.00663420203886	1.47123221470779	1.07640235977588\\
1.0691447990303	1.5009622286756	1.15093479724517\\
1.12606186973462	1.5446864200095	1.22701164262742\\
1.17974472675541	1.58769448825149	1.30355404511283\\
1.2329264835621	1.62665571917759	1.37577149928208\\
1.28210258936641	1.66271999651647	1.44977142231725\\
1.33055578649617	1.7028061616776	1.52665462199228\\
1.37903574812156	1.74629378364962	1.60168294795199\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00068039801429	0.240653644756187	-0.999024335894011\\
-0.937253295640987	0.300747056284595	-0.948466637951207\\
-0.873652877040978	0.338650004030541	-0.895336306301265\\
-0.808113604720478	0.388253193978652	-0.841404607716261\\
-0.743978307833414	0.436430858469606	-0.788134022778441\\
-0.682478371160331	0.490718587451654	-0.737315538042155\\
-0.620992286937752	0.5365139577963	-0.68702622812266\\
-0.559126266454237	0.586339083846549	-0.638445314630722\\
-0.494960379644859	0.633528757751934	-0.589898566209941\\
-0.428543946918859	0.683150244550394	-0.542683692201893\\
-0.362373878711569	0.73042517132893	-0.492837526232333\\
-0.292264814548535	0.778709195805616	-0.443338481202199\\
-0.222913209015542	0.818688459852304	-0.39347693392683\\
-0.151905178353261	0.855789346155398	-0.347375085952224\\
-0.0786397332109598	0.893602641023956	-0.298894449829859\\
-0.0083435986758045	0.933263829790044	-0.255519614643458\\
0.0692654400206779	0.972730838622875	-0.207740520051098\\
0.143898911173719	1.00587304301728	-0.157196654923438\\
0.224904696508977	1.03794175311786	-0.110746295232362\\
0.308109665172005	1.07450635599904	-0.0650790587178632\\
0.391693928912089	1.10759844889851	-0.016851449573118\\
0.475247228923485	1.14339743846377	0.0330466799342419\\
0.558987369576932	1.1779462152993	0.0877520837481897\\
0.641236597108186	1.21279989619249	0.139539230690144\\
0.730327880690867	1.24736327756213	0.196787522417735\\
0.818403581360737	1.27869592800771	0.254486754886065\\
0.911133894349329	1.32304172617135	0.311510344469394\\
1.00196265849277	1.36857489729479	0.363292126884496\\
1.08499303940429	1.41039054155304	0.416193982274278\\
1.17357355895132	1.45437433853469	0.465193744115268\\
1.27108916573045	1.49585615817136	0.511198188920007\\
1.36738815203217	1.5288777946603	0.559249988865571\\
1.46459792584918	1.57099099022238	0.60704842066653\\
1.56212782255143	1.61255482846046	0.657140249559243\\
1.65101905229456	1.64009040659743	0.697355172143784\\
1.73689753157938	1.68738904946681	0.743162119241309\\
1.83612693015357	1.72298066468903	0.788077066694301\\
1.93577383028603	1.7571649821941	0.834936806521095\\
2.03580061539425	1.79740284902888	0.871827160397645\\
2.14640774918638	1.82927946907133	0.91891253168607\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00078365475287	0.23992355535741	-0.999728671012028\\
-0.935891642953166	0.300091825089731	-0.951474389462341\\
-0.87418466838095	0.346093476197099	-0.909218351198902\\
-0.812655596659914	0.38997905399921	-0.866003938379414\\
-0.752169420156563	0.43787424959484	-0.822649289058851\\
-0.693160374216775	0.485257210769055	-0.783997105360234\\
-0.633899961413753	0.536927934143049	-0.750349007416267\\
-0.578063148420872	0.585347426857786	-0.713390213594638\\
-0.522336889168724	0.633788617358528	-0.680267083935142\\
-0.466170272683795	0.679281679845899	-0.648519521131764\\
-0.413201259798065	0.729604239953143	-0.61380063664545\\
-0.356193498793296	0.777507316190032	-0.577618642803768\\
-0.300237980555567	0.824550367130647	-0.539948180551264\\
-0.239572284860228	0.872342499049926	-0.501372323047942\\
-0.180259819052109	0.922921441578816	-0.462921887665123\\
-0.121082899804986	0.974075155469182	-0.427164662472606\\
-0.0596028969316553	1.02779599155048	-0.389515978863963\\
0.00501546932763867	1.07894707697658	-0.348259722788119\\
0.0710579821881429	1.13287548301642	-0.309723734836253\\
0.14031608034427	1.18204009515857	-0.272939079172506\\
0.201524037587837	1.22856440719882	-0.238853614006538\\
0.263305609475994	1.2749900556921	-0.205138519084251\\
0.32685918959988	1.32175041691463	-0.173873034309376\\
0.391412762787077	1.3758752709622	-0.14299065739635\\
0.452820392377637	1.42970299149503	-0.115271006907894\\
0.517680455999868	1.47537224732817	-0.0883101602986723\\
0.579419045623243	1.53030767951344	-0.0581559539972585\\
0.637925300760748	1.5806756508248	-0.0350750467162361\\
0.695185422632207	1.63571118302487	-0.00440397548219863\\
0.756929900314464	1.69009717857704	0.0185571639265925\\
0.815811620634022	1.75058499785149	0.042499890303336\\
0.870765183520883	1.80180156512811	0.064911783031098\\
0.928885152338001	1.84612847431331	0.0876981845852584\\
0.989320626855028	1.90289284182915	0.104575673815243\\
1.04275871276515	1.96252053390895	0.120934328141935\\
1.09530686760527	2.02619255868345	0.1387665029957\\
1.15094350015327	2.09891026242926	0.154727215184451\\
1.20222732319365	2.16430494030975	0.169206799873526\\
1.2573556028871	2.22674555926012	0.181193062032712\\
1.31218258441105	2.28963419120086	0.191422453652016\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997765059396343	0.239368119619885	-0.998632467358541\\
-0.93937373323242	0.30214329108609	-0.949185409875145\\
-0.875430882826985	0.348818635030752	-0.899319098786669\\
-0.814920588751239	0.390444458877849	-0.849219374066013\\
-0.756449272533883	0.434456193704606	-0.804731821703027\\
-0.697587230861426	0.479936607372494	-0.758398834170475\\
-0.639413273211574	0.532570180522667	-0.716201607484398\\
-0.583250669876915	0.580930796622951	-0.66750582265269\\
-0.527361234888502	0.625535916742555	-0.619366080362518\\
-0.473860540054439	0.675138429741735	-0.573455403431676\\
-0.416842602137691	0.718787849718638	-0.526531922360328\\
-0.355517228729186	0.761941008670046	-0.481906741047513\\
-0.29924429795684	0.797860286506303	-0.43411365788437\\
-0.241579316760711	0.842665495279437	-0.38576965554492\\
-0.186214436407172	0.884510695935943	-0.33955466820198\\
-0.131472460259029	0.922322507515103	-0.291391040471825\\
-0.0818283018778097	0.965781306244273	-0.243710623772155\\
-0.0289450444715565	1.01362678155263	-0.196341134494746\\
0.0192766868295891	1.06065271318524	-0.147124525310489\\
0.0663651930763715	1.10930768509397	-0.095297947451749\\
0.117825522326872	1.15754189666042	-0.0483557043478084\\
0.164682153080368	1.20379487712617	-0.00279573383468452\\
0.211010479540805	1.25258364544966	0.0411455465734933\\
0.255594040030545	1.30692149575259	0.0922078762991131\\
0.298254564870538	1.35645848800623	0.142000608966418\\
0.342873876235389	1.40253907038574	0.189173183692991\\
0.392926276047407	1.4486794048328	0.23175092839643\\
0.43680424289492	1.48816583448801	0.276156170773253\\
0.4807378215762	1.53137364047456	0.322775513737631\\
0.526620198531542	1.56920228882126	0.359127831373691\\
0.56591489672637	1.61693229148691	0.404238742203233\\
0.610099917813616	1.65270722008485	0.447338321696072\\
0.652502599965383	1.69384746474384	0.485782584780267\\
0.700410178129929	1.73198556856864	0.52402903078929\\
0.752113576201318	1.76889797773974	0.565405797293733\\
0.801923949775538	1.80660358681109	0.605765402145737\\
0.857822291965766	1.84933557779032	0.644559486875519\\
0.914588074077971	1.88384810618892	0.689810740450099\\
0.961631798383387	1.92606158107412	0.731858711330456\\
1.0148826543844	1.96115444333319	0.774784027441618\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00124092589185	0.239816003778784	-0.998979463466204\\
-0.937288483883964	0.298652216485728	-0.947305080414681\\
-0.874324015956683	0.346679988346124	-0.895911654551714\\
-0.813086423541777	0.396488056541292	-0.843166313898894\\
-0.751010436713365	0.446269804704144	-0.78817970307042\\
-0.682882612520197	0.493528138625298	-0.736862023324279\\
-0.613861780293297	0.545395910931668	-0.682527468420955\\
-0.538838020915168	0.590867343909261	-0.625300948241179\\
-0.466039239828263	0.641714009902162	-0.569903590745812\\
-0.398667635275314	0.69222350235383	-0.520227774555629\\
-0.330008627457289	0.747162137589701	-0.46170774691253\\
-0.260499094905648	0.801375354698887	-0.40616405740866\\
-0.186767739138402	0.856294633077699	-0.351163497386381\\
-0.111019062347564	0.908056769338158	-0.294500064696019\\
-0.0350835522365496	0.958857705356086	-0.240772170645303\\
0.0426463628396927	1.0186034213848	-0.190925113936523\\
0.11791103936777	1.0705704139845	-0.141053473742598\\
0.197839296599261	1.12843363279935	-0.0872794812274623\\
0.277347790307844	1.1823768445215	-0.0310909748515738\\
0.360988620334964	1.23250037248435	0.026051780568783\\
0.438124102287111	1.27967137325163	0.0790201668357556\\
0.515206366190743	1.33008348979629	0.129780283140996\\
0.599816880653003	1.38299679982594	0.182631115781806\\
0.678888828794389	1.43166401753439	0.234165040762675\\
0.758029893448463	1.48160154547055	0.286636606059209\\
0.841015536434754	1.52993908396869	0.336523085378486\\
0.924889234355651	1.581273031991	0.381659253479001\\
1.00387249973436	1.62711092001131	0.425831594133192\\
1.08168968192146	1.67569786099973	0.463410534659372\\
1.16164203108494	1.72351386188058	0.504984800696315\\
1.23737000582405	1.77232198652142	0.549479689877577\\
1.31104377052331	1.82690193330057	0.595304293111153\\
1.38668724076	1.87766090010812	0.632646767553519\\
1.46437653667485	1.92354642765666	0.674047007503459\\
1.54456738776447	1.97765707938978	0.710337580898264\\
1.62013027426845	2.02878200653533	0.745168892467828\\
1.70279727725444	2.08362349291647	0.787683450570283\\
1.78568175922823	2.13599486884661	0.819525740697244\\
1.87154876593784	2.19139625223957	0.863728576209412\\
1.94806169574255	2.24685221306749	0.907639684684533\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99935194721902	0.238681935338578	-0.998614880487704\\
-0.940335836971935	0.294976492649077	-0.948870499024057\\
-0.874908791475569	0.341477802018139	-0.896921152791689\\
-0.812388641867099	0.385690279888144	-0.844281874115211\\
-0.750864214281315	0.429173650735838	-0.792088891824479\\
-0.690905511463685	0.464874821347287	-0.740351533534099\\
-0.631977740516516	0.503337534656834	-0.685425691263554\\
-0.571132209431751	0.54134772890941	-0.631745062895502\\
-0.507316451248349	0.579404089114587	-0.579542816811058\\
-0.441180989267618	0.615904911165074	-0.528489391519457\\
-0.372345206888199	0.650356337398777	-0.47468554690201\\
-0.3042245244206	0.688509812480207	-0.425825793298077\\
-0.234662626611892	0.72125536451384	-0.375200019770466\\
-0.163090084788497	0.760131401500791	-0.326837971516642\\
-0.0893268737884853	0.791805202790887	-0.279677400815967\\
-0.0183310397317188	0.838870042194565	-0.230546207273301\\
0.0587946373017586	0.879888778294201	-0.187346580087519\\
0.129542188948448	0.928790274326802	-0.146944594367335\\
0.19870398092916	0.97008979090525	-0.106744648497142\\
0.268992986614762	1.00845715728851	-0.0587876227145755\\
0.342444831359641	1.05597310529209	-0.016633186444905\\
0.416066471449191	1.1013404563555	0.0303418665508237\\
0.493292186449519	1.14913228388169	0.0724549004087658\\
0.565144821047364	1.19875654035141	0.120335642148666\\
0.631988359088721	1.24445046761545	0.164866528774112\\
0.699383810166387	1.29010785268828	0.207833740504836\\
0.766648989026749	1.34489441145531	0.248559227784297\\
0.833580294365854	1.39385174978063	0.297406458174374\\
0.901497318434043	1.43850835907576	0.346483250157958\\
0.966442046604626	1.48763067637605	0.392314535904749\\
1.03047451970741	1.53159672115588	0.440687899918605\\
1.09051333003387	1.57761600039227	0.485585283586414\\
1.15272401877982	1.61953124886624	0.534540816773247\\
1.21364671499112	1.66189468245294	0.57786534400908\\
1.27806458218462	1.71141740171944	0.618109534977801\\
1.33858492863642	1.75846661187408	0.665612352640433\\
1.40684406280712	1.80841245433489	0.704197487856624\\
1.47287973581568	1.85293521433314	0.749909007172522\\
1.5436681275598	1.89714042979675	0.793034464721989\\
1.61550488564297	1.94724852083146	0.834530127630623\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999634859621356	0.239271779481475	-0.998679462684257\\
-0.936111764381054	0.296283614453489	-0.94831683958489\\
-0.879129763640786	0.344920328813215	-0.89736794283437\\
-0.820567957889284	0.392716186502721	-0.844863550836345\\
-0.765485602045061	0.443495726580834	-0.789972709196182\\
-0.71005856716443	0.497655503148952	-0.732126627113771\\
-0.659365634265378	0.550808457412839	-0.676819882311723\\
-0.604592497605471	0.606490147647145	-0.621946983750836\\
-0.55054846969073	0.651072972043645	-0.564630384875968\\
-0.499489541386082	0.699347844936272	-0.507702707992726\\
-0.446330041569933	0.7502738321523	-0.450930613005345\\
-0.396044907406805	0.798113391378133	-0.391029921300544\\
-0.338611297900659	0.849822383643951	-0.331618714582251\\
-0.280690737471354	0.894578984122785	-0.270568912008518\\
-0.224711941751689	0.93849644601338	-0.209683058849851\\
-0.16892685369019	0.986275482886221	-0.155018792153008\\
-0.111134990825546	1.02559974484507	-0.100499468719658\\
-0.0549752908328018	1.06320527674927	-0.0456769296444546\\
-0.000977872683983087	1.09666252849073	0.010302887012338\\
0.0557587964780432	1.13781354447212	0.0607750484519258\\
0.116110577061856	1.17545485565356	0.115959218816399\\
0.175691679666404	1.20992923955523	0.161901311504316\\
0.232748765770166	1.24716034135514	0.210486992358668\\
0.292881897898659	1.28045142232902	0.257209720815239\\
0.351400916583728	1.31226386929515	0.305560539142629\\
0.407759025047308	1.34674089736457	0.353242150936268\\
0.464362193982513	1.38289946352213	0.40354352753329\\
0.519806515232579	1.41766533333554	0.450756754805817\\
0.579791581474152	1.45298806998336	0.49982899465621\\
0.630330461225914	1.48939798469553	0.548791834620117\\
0.680207559994775	1.52433116639941	0.590702092131388\\
0.732210593375266	1.56916542552337	0.64101786961329\\
0.782830371440488	1.60933724902005	0.688040626190246\\
0.835222882756387	1.64714827145702	0.742395842277165\\
0.879167065106617	1.6908307056549	0.787836221186975\\
0.922554779812626	1.73442902138144	0.835343280017121\\
0.968229202375749	1.7800803062225	0.875578095160023\\
1.00468409432214	1.82122244587443	0.920233266083355\\
1.04954752099087	1.86385882139071	0.972889979690468\\
1.09424933934566	1.90572203463849	1.01571907640299\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998820335376772	0.238921318243581	-0.996969581059155\\
-0.937071634582295	0.295140179291052	-0.943756993473794\\
-0.876139596659584	0.344939806167525	-0.897342204977664\\
-0.813721266783148	0.397691538934039	-0.841597462365402\\
-0.748021699902443	0.445484609128519	-0.78301767507068\\
-0.685043459105533	0.499721975901537	-0.73103355466423\\
-0.618842846105844	0.547120151214652	-0.677477946235264\\
-0.546844142562826	0.587095564076127	-0.623561101067313\\
-0.46823195206458	0.632124148862021	-0.571199447699018\\
-0.395515238202973	0.675072970046032	-0.520880772337115\\
-0.319938529664889	0.713615139425768	-0.465927183386198\\
-0.243211956264313	0.752923796959993	-0.410387217377009\\
-0.168155245938329	0.790597964672429	-0.354645879879868\\
-0.0958117218807896	0.829815104746962	-0.301180641105088\\
-0.0259715780474841	0.860550878588039	-0.246873953464595\\
0.0421023788172709	0.904274596508869	-0.195717790601222\\
0.113715180511701	0.951859870071415	-0.141406863864737\\
0.184706948439921	0.997536369595875	-0.091462727889696\\
0.249250946848064	1.04057469957017	-0.0424766261122953\\
0.320079487574856	1.08890931768402	0.0106434234306132\\
0.392174896817315	1.13407108515269	0.0610073539818095\\
0.457136971874876	1.17454222116694	0.112058158005418\\
0.519428042632615	1.22245260767292	0.160549911540699\\
0.584663574066972	1.2627042345698	0.209544686831594\\
0.649822494004643	1.32118306801154	0.26012615385116\\
0.719907162719835	1.36934072698426	0.307409175359373\\
0.78338103065916	1.41597416906786	0.356188806277736\\
0.847678004201852	1.46567996380167	0.406173497391645\\
0.913221152014442	1.5151702694116	0.460843008360163\\
0.98030984083085	1.55695937707148	0.517205072955565\\
1.03952857790341	1.60332881896411	0.571317714147402\\
1.09798755174183	1.65011344344005	0.625106222583626\\
1.1643635454599	1.69280340409992	0.676078149923056\\
1.22877548910632	1.7465278474927	0.734725491744017\\
1.29305008212906	1.79291020122233	0.784666086452308\\
1.36131578464863	1.85129472235578	0.837823693033084\\
1.42229886754359	1.90412508397255	0.884608592598434\\
1.49063846924171	1.9581272450955	0.931869184869564\\
1.56626535556546	2.02545736600662	0.976794527451747\\
1.63564991973717	2.07397037829095	1.02263920234139\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998141641676941	0.240967974914197	-1.00104573129492\\
-0.940289965417701	0.296436333508483	-0.951756290257576\\
-0.880642106735884	0.346193713113848	-0.90194032523838\\
-0.823903869886611	0.394281991098614	-0.848688414968544\\
-0.774515055117073	0.44663042020815	-0.795615391257305\\
-0.718953555876818	0.493396837258269	-0.743592861836015\\
-0.663014760487011	0.540758853407822	-0.691942101793505\\
-0.604643703120425	0.584821925667062	-0.643936819934352\\
-0.551142793187199	0.635150151318448	-0.599578378844916\\
-0.493137791939963	0.678849867648144	-0.552117599593888\\
-0.438176982506915	0.724377433661882	-0.502596057358096\\
-0.381608546230655	0.766878362948332	-0.449712819452601\\
-0.324235174831834	0.806449695532166	-0.399555125349189\\
-0.264110604083804	0.850979232727021	-0.350140378946814\\
-0.206512661124915	0.894379517090073	-0.301081461622054\\
-0.154237726861326	0.941430839990925	-0.250857608285135\\
-0.10086694970637	0.98442856337781	-0.201758719189176\\
-0.0459965825642973	1.03030334795318	-0.152779607595599\\
0.0108273687164005	1.07162883151285	-0.108031767186483\\
0.0630459839546758	1.12172448432462	-0.0640373791277421\\
0.114140364546358	1.16516459074779	-0.0185712643445556\\
0.167483057058572	1.21027796183965	0.0260149100624995\\
0.22499017885151	1.26023140779112	0.0689347587561598\\
0.275815418455338	1.30780796524357	0.112388677324613\\
0.329024379692852	1.35324196944629	0.15361027360572\\
0.38405613968104	1.39732267347827	0.192652958101126\\
0.440666272778179	1.44568166461066	0.23004812488495\\
0.497406879657085	1.49283470924521	0.275313496475246\\
0.559461237584241	1.5377608107421	0.31895704973692\\
0.623380174570776	1.58877975853588	0.360598797189408\\
0.693562409807554	1.62522930427611	0.403593824844869\\
0.765342611122525	1.66695834452229	0.44944560983481\\
0.83752062084654	1.71001844620491	0.494724077995049\\
0.908406001396094	1.75106936413118	0.55064618493569\\
0.983922390329083	1.78547007538123	0.597413206791784\\
1.05826693551764	1.82043870407701	0.655931597015267\\
1.13113499572271	1.85605619904299	0.708403706593457\\
1.20619129348005	1.88540233292976	0.755280510916421\\
1.28143016981168	1.91792636176267	0.811799247013876\\
1.3578558127962	1.94481149689388	0.868215907014479\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999379532098069	0.241223723327276	-0.999920084408998\\
-0.93492165331174	0.295914305409757	-0.946124244297636\\
-0.874994082955451	0.343031763381411	-0.894850305142999\\
-0.809094593462341	0.385981203187363	-0.841311767072062\\
-0.750513715131491	0.435396407421481	-0.789834135005093\\
-0.687586902390309	0.480360499957345	-0.736112328938023\\
-0.632691069686544	0.526903928045293	-0.681665340098762\\
-0.577944258981679	0.572691468807821	-0.626757505663241\\
-0.525543804283991	0.618660045578255	-0.57429801599278\\
-0.473354545274657	0.664572066760024	-0.518335892726232\\
-0.416061773757111	0.71889625048144	-0.461207246992515\\
-0.357857832172204	0.765455440821941	-0.3978378972767\\
-0.302274939986316	0.816627044511738	-0.335877313033306\\
-0.247947521476374	0.862266087482545	-0.275042145613876\\
-0.199879405995406	0.904374457595352	-0.216176381583011\\
-0.156466604454471	0.945687096831013	-0.154985257768373\\
-0.112194634728078	0.992549864846286	-0.0905928258134019\\
-0.0691812259949483	1.03655867008954	-0.0319964039603638\\
-0.0231554325911002	1.07949726980244	0.0243611132704072\\
0.025900862016675	1.12645333379324	0.0791319056483098\\
0.0718501885869285	1.16993008852809	0.136942515132676\\
0.119671273213875	1.21654756500959	0.19367263401488\\
0.168020561329555	1.25850470482246	0.244341762240554\\
0.21802461144304	1.30164387328126	0.304327430250959\\
0.270951950541524	1.34508155835582	0.357294114281204\\
0.321030143896179	1.39422266287677	0.409521576158534\\
0.377994998122363	1.43741189245949	0.461461115991604\\
0.435859567248624	1.48389534083306	0.514845197059223\\
0.496265467782873	1.53040445464621	0.565186714389318\\
0.556299039976345	1.58255010062908	0.615363436602804\\
0.617047681951464	1.63552058297951	0.669227994220004\\
0.680907093515907	1.6872794052462	0.719695355352909\\
0.742044735390273	1.7413481484156	0.76984166661847\\
0.802018594842547	1.79214191244091	0.820403165860948\\
0.859282127973218	1.84274059100774	0.872457664819439\\
0.916853818852517	1.89879759749512	0.931304340332778\\
0.975616134558948	1.9593164400295	0.987942311220517\\
1.02881600198417	2.02219584921213	1.04481651384734\\
1.0832693049385	2.08176642178776	1.09728417561781\\
1.13277286916824	2.14841003268375	1.15596800117175\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999692310620872	0.239927674033235	-0.999472432615463\\
-0.933209819728707	0.294748472255955	-0.952261281905421\\
-0.868577711023995	0.335765656725296	-0.904340802739909\\
-0.799092069724105	0.377827820415651	-0.853678993657259\\
-0.727332144761213	0.422970624041353	-0.807275525685005\\
-0.655851728054118	0.473916580110526	-0.75888187800323\\
-0.587001768519097	0.520084917967592	-0.707430624155749\\
-0.515955211025173	0.567453846966708	-0.656195506366815\\
-0.446198405426685	0.612821995961846	-0.605449946997307\\
-0.373250218732531	0.65216923049297	-0.554816287316858\\
-0.299296176120974	0.690687677149231	-0.501713936178241\\
-0.223971979258598	0.729535119464636	-0.449265513717634\\
-0.152145543292195	0.762859695512808	-0.393640208907787\\
-0.077939023765532	0.792386590549032	-0.334102158390686\\
-0.00772147692959863	0.820768415406884	-0.276871959717681\\
0.0610432880036605	0.845364995915679	-0.214686061882883\\
0.129184138865217	0.869133626882791	-0.159136365829675\\
0.197104110175878	0.898505083067777	-0.105594134850437\\
0.263868304657298	0.92054046392094	-0.0480516806394047\\
0.333409676023692	0.947021412351271	0.00319140706745683\\
0.403062971142568	0.970883716135543	0.0584373869445038\\
0.475682004816493	0.995920020940746	0.11412895053286\\
0.5449443372319	1.01752848431982	0.163525375301499\\
0.610392438290691	1.03998945592692	0.216423960829373\\
0.674330360522012	1.06938989168373	0.271322847711803\\
0.738445814596909	1.09437680542196	0.328401356808452\\
0.801823353084034	1.11926185706369	0.381847195154675\\
0.864314845733103	1.14190470530954	0.438691398473727\\
0.920222809590428	1.16666620393811	0.485574912785679\\
0.977558104172646	1.19310145446199	0.534438156242062\\
1.03463157503337	1.21726284661055	0.580998946992507\\
1.08685230105948	1.23856160545643	0.627852252630681\\
1.13793081805297	1.2593147644309	0.677243817230983\\
1.19545577295665	1.27798699002787	0.728361159733363\\
1.24754004030227	1.30250091317863	0.776440145446456\\
1.30191549833444	1.31824391475217	0.821097606228413\\
1.3575995649498	1.34538921661929	0.86869134821583\\
1.40889647097055	1.37273800670513	0.914263774778509\\
1.46259078616865	1.39435947213133	0.958178684058967\\
1.5196290196583	1.41998842495514	0.99970630630871\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.0008872540537	0.241432926064298	-0.996633556315726\\
-0.937172206737194	0.303169074359908	-0.953146360197932\\
-0.877023053451693	0.345234437205845	-0.905475789191137\\
-0.811349230914318	0.393087850027326	-0.857675931327085\\
-0.748557536889076	0.43950763832727	-0.807468564276365\\
-0.690821605453801	0.49064589322845	-0.757118489027448\\
-0.631296132199868	0.538810205812094	-0.707828558577903\\
-0.571461507142488	0.585759839128613	-0.661269483166922\\
-0.513408007728163	0.6381450439303	-0.610789885088859\\
-0.455146235541629	0.688970344751322	-0.55923029660364\\
-0.401220864936343	0.745194904194207	-0.512607935279978\\
-0.342709330464797	0.798349645315461	-0.463116163216725\\
-0.282164833815141	0.856037033053808	-0.41532914635638\\
-0.222468242143816	0.917796548686238	-0.361975760192633\\
-0.165045956534996	0.981677973042248	-0.309740304771138\\
-0.108364342811272	1.04652973304131	-0.257534753134524\\
-0.0587552517817292	1.11217382389008	-0.206808854252477\\
-0.00200931185334325	1.17737973156386	-0.155243031753258\\
0.0562196644555416	1.24351072637553	-0.100664547768488\\
0.114940699105903	1.30766965566372	-0.0488840862162478\\
0.170919506281538	1.37229158082352	0.00453343930163976\\
0.226041481777202	1.44372672196622	0.0567280100758777\\
0.282446284908058	1.50867484967037	0.110299882473515\\
0.340083934919905	1.57077561906573	0.161165948861961\\
0.390407734954244	1.64136285524902	0.206372763361386\\
0.445499308068681	1.71892544365508	0.255642234222136\\
0.498051206182195	1.79675195542776	0.306691133636599\\
0.551553624648943	1.87939959894694	0.353772234579832\\
0.601596043468437	1.95851317361973	0.403985923034679\\
0.65806362583231	2.04401454564946	0.452116753343756\\
0.709241154377718	2.12176029890201	0.506249261000002\\
0.755720320081895	2.20270713280254	0.554394415598567\\
0.800217191516422	2.29846251561385	0.602512599047508\\
0.852456529453143	2.37994727284175	0.654591488133874\\
0.894773629436084	2.45194429646527	0.712713921456089\\
0.940881650942463	2.5302859323334	0.758885602116381\\
0.985561789341494	2.60697507286057	0.807825988608978\\
1.02382142933863	2.67772575072283	0.853294196716483\\
1.06953942346816	2.75370739644224	0.901880082748034\\
1.12365698166703	2.83573277421499	0.944352229336189\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00082743567633	0.238885170251025	-0.996206865027175\\
-0.940817417922833	0.296881056563082	-0.948557069637876\\
-0.881878366995346	0.35101660361673	-0.897637455255167\\
-0.819402456815038	0.400725296794156	-0.842970874700834\\
-0.758599621810355	0.455218953359551	-0.782301494425766\\
-0.698250709671254	0.516697996269605	-0.724683641260743\\
-0.642195280607129	0.574935395397737	-0.660382756763835\\
-0.591977079946194	0.635209516502012	-0.596605906885547\\
-0.540601864243441	0.701893624195876	-0.534844301705328\\
-0.48334891784124	0.764034702508068	-0.471390740652786\\
-0.429295032459792	0.827783704820473	-0.407844601893901\\
-0.373027477484754	0.899178055716306	-0.347857776586655\\
-0.319733916661838	0.966387419444043	-0.285557069314635\\
-0.268251566022367	1.02707986125062	-0.22193314363696\\
-0.221575564879888	1.09072701171127	-0.160646300653345\\
-0.167831926242652	1.14869201584876	-0.0979971288513163\\
-0.114306874366952	1.21188288584621	-0.039256381790911\\
-0.0568484378683423	1.27135149170009	0.0208765077156277\\
-0.00269477784702398	1.33240485248897	0.0767110264607232\\
0.0553665454390656	1.39401571314772	0.130330605519855\\
0.102977587419805	1.44898789224728	0.183197551203754\\
0.15567900311223	1.50842486891107	0.235722722361896\\
0.207823061891058	1.56571513228968	0.28555200706942\\
0.255135614146583	1.61638481097362	0.337960088325288\\
0.304790259240445	1.67414838607076	0.384614022381312\\
0.355903086354957	1.73159358461473	0.439592646541742\\
0.406634016269651	1.7868743930437	0.491809721004599\\
0.460914263153398	1.8343807011135	0.543374422784016\\
0.511542861930725	1.88494950697514	0.592598079622089\\
0.565263290721416	1.93961102731021	0.646332373128015\\
0.616981555691952	1.99077201622695	0.702819101503462\\
0.671197567301063	2.04015319134609	0.760803284275124\\
0.726075240116637	2.10650310794462	0.81718418991772\\
0.783255221024317	2.16623585687345	0.865259934274922\\
0.853000676037957	2.22763775186827	0.917531008264735\\
0.913478824212786	2.29682918743265	0.966696296980674\\
0.969452970558019	2.36517560733474	1.02015598397779\\
1.02946830395265	2.4281140161147	1.0748752797848\\
1.09250649588298	2.49312186411354	1.13649164958425\\
1.14801020465013	2.55986789988781	1.19054503258881\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00008317066648	0.242834635470484	-0.999899041095014\\
-0.939346175301803	0.296314821407122	-0.949410557679027\\
-0.880099002568571	0.343752438190296	-0.906356273050507\\
-0.824651746555369	0.391426348091208	-0.859385172836208\\
-0.771442787411484	0.437491768170075	-0.813425413378958\\
-0.714945218902297	0.485506554465226	-0.766641089437531\\
-0.662834128060215	0.534399092098705	-0.716416013327529\\
-0.608251504078102	0.584689137110478	-0.662707721076069\\
-0.554193738412495	0.631881020127409	-0.610628535553922\\
-0.500856522659415	0.673592449757168	-0.557450907962817\\
-0.446866294993415	0.723393243569409	-0.508738522550848\\
-0.392892391536904	0.770496439283146	-0.464306520964812\\
-0.333205082199676	0.82227573006045	-0.41442530380006\\
-0.276525099730795	0.873340341902548	-0.362061970649051\\
-0.223084849807473	0.92940436471091	-0.311476610522187\\
-0.168194829036812	0.98411040994248	-0.256843284268853\\
-0.107695320415129	1.04428466753511	-0.203963361014592\\
-0.0511222109411478	1.1030549491784	-0.157362670295097\\
0.00767296756030962	1.15454670598118	-0.108365094141501\\
0.0652733523734312	1.20667399690555	-0.0580264467290626\\
0.124304356030193	1.25576257928068	-0.00255882061443522\\
0.184480909991661	1.30970698496415	0.0576169470209865\\
0.248308933665813	1.35810446897833	0.119255205753347\\
0.312381494076611	1.41291239064518	0.184709998448736\\
0.375793362004162	1.45854951669542	0.249077833742865\\
0.436653862834686	1.50533424380876	0.309392810111666\\
0.502277859071436	1.55091135955666	0.373128960529219\\
0.571816446990701	1.60072996369009	0.437708227074967\\
0.640634339259514	1.64180824132921	0.503741223253932\\
0.702863475564713	1.6938980380019	0.569547105290018\\
0.767703523237002	1.74477144201522	0.640765705504502\\
0.838987846409415	1.80057861810469	0.716908063729262\\
0.905544002759294	1.8570284413532	0.787790908144922\\
0.975474719821674	1.91674420466195	0.86644919650893\\
1.04026145249735	1.96817372844567	0.940443625728088\\
1.10619586999997	2.02246670642592	1.00891639137243\\
1.16765686988811	2.06939376269636	1.07931471959946\\
1.23573994474283	2.12443111378121	1.14497919445465\\
1.30158775659136	2.17076864519567	1.20471193671836\\
1.3671983888644	2.21714675790961	1.25959274581551\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00020775695172	0.241752468326017	-0.998207411825569\\
-0.935412660457032	0.293829513775434	-0.945800936610767\\
-0.871239674859816	0.336606502333263	-0.896456181201684\\
-0.808541806413232	0.383791459409964	-0.843740034979626\\
-0.747295722993108	0.428188110837707	-0.787160495564368\\
-0.685957354453649	0.471724817867047	-0.728515526449395\\
-0.624326120910088	0.517746242483975	-0.671694126636045\\
-0.565079026375145	0.5647115272411	-0.616493908649543\\
-0.506665091639353	0.612639196436584	-0.562975793784745\\
-0.450662943200388	0.666281371968875	-0.514734149996427\\
-0.390564184894974	0.713579958084468	-0.4687636267017\\
-0.332438751806191	0.765269474638649	-0.424816335969826\\
-0.271536519170302	0.817951094590046	-0.383183921346484\\
-0.209292031525921	0.870531366154017	-0.339336111957847\\
-0.146875008068577	0.920883730011517	-0.292182145126404\\
-0.0830619297188933	0.967117923257754	-0.24622403560658\\
-0.0190025917659913	1.01543061657803	-0.197558077179422\\
0.0463146252773338	1.0665823738543	-0.147657825204193\\
0.107590326974069	1.11861402453776	-0.0985198091543596\\
0.172196688471171	1.17227969641039	-0.05130621956541\\
0.237663158652785	1.22669549039476	-0.00404275707666333\\
0.307380372152273	1.28342599295708	0.0408935012984167\\
0.3796894396644	1.33444743074769	0.0868261666490223\\
0.454845401889092	1.38895559911942	0.132489653079162\\
0.531622067764118	1.44535519983395	0.176263967132718\\
0.601800283013693	1.49885816783364	0.222326432057736\\
0.676908940749516	1.55113522791756	0.268860502759302\\
0.748302461751008	1.60708930892292	0.312574123220425\\
0.817069811649118	1.65967719847086	0.356537006104763\\
0.886239338921974	1.71254464257122	0.407946342020007\\
0.957336911433076	1.75698937713088	0.451327092603668\\
1.030913206791	1.79956243382572	0.495754502256299\\
1.1073219333597	1.8619595214226	0.549421259363623\\
1.18463833455541	1.90987749375411	0.603452648070007\\
1.25684062884056	1.96240220296043	0.65338077251216\\
1.32739545930923	2.02083954535988	0.703923561802601\\
1.39664955208251	2.07153467299757	0.755171261002132\\
1.4642169515537	2.13032785613182	0.807560154139646\\
1.54029054503522	2.18966417491797	0.862873472463479\\
1.60160131632678	2.23871556754639	0.910406606830474\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997497770797953	0.241338622250135	-0.997689821932872\\
-0.935305408722999	0.297768099946843	-0.949867904844403\\
-0.875335708765558	0.342110242819317	-0.901852183933097\\
-0.815849241962318	0.393494416689344	-0.8581953643271\\
-0.757742463920341	0.434221336330512	-0.814672587605776\\
-0.699074320449531	0.477099486565259	-0.772991064002535\\
-0.640336141124177	0.512716515695571	-0.727457110946281\\
-0.575840145144716	0.548120828302769	-0.681013638705464\\
-0.518686074606721	0.587661264146064	-0.632144825901329\\
-0.460136356239959	0.622039593487913	-0.585035216907204\\
-0.405973766081343	0.659569930648631	-0.535321942193913\\
-0.351197114697678	0.69908797156257	-0.485978198919754\\
-0.296672365262517	0.734122246153381	-0.438880075596537\\
-0.242053822006569	0.765820407948098	-0.388312838826704\\
-0.186553322901428	0.797359101361913	-0.337177588026869\\
-0.132205049122026	0.834877891222277	-0.287265621766334\\
-0.0820790894718472	0.872534512104874	-0.236114342486902\\
-0.0360199003929473	0.902788813015577	-0.184077630742093\\
0.014504698540903	0.942014452743439	-0.126699027959907\\
0.0580565922504901	0.97575901111624	-0.0709197961710588\\
0.108704760710776	1.01065614913078	-0.0158575813236208\\
0.162441128017141	1.04281582328382	0.0350139541656995\\
0.211868799919124	1.07835584954129	0.0895762618026884\\
0.267614654424767	1.11508846064413	0.145417667938227\\
0.321295401555564	1.14590299024124	0.196990341840391\\
0.376017110984062	1.17830678585824	0.251811820578513\\
0.424864898874264	1.21009749242554	0.306463046234224\\
0.474134593098504	1.24102549811481	0.36185673587438\\
0.526208333874866	1.27205964880837	0.416768847238454\\
0.575730902605529	1.3043520829736	0.468890479567695\\
0.63048359626773	1.34259998022593	0.52301232229123\\
0.681910995817487	1.37421245082713	0.579085006821283\\
0.733135676836192	1.40693314636095	0.636641263658516\\
0.776524622534419	1.44108002332212	0.686512503131546\\
0.8293758470028	1.47087445357308	0.75200471300118\\
0.878038599561469	1.49615492704504	0.809110371381686\\
0.929546584371171	1.5283081672303	0.870945893273693\\
0.979460470974572	1.56142999572212	0.933079533889153\\
1.0321669016887	1.58884239567125	0.998263790334524\\
1.08094257537962	1.62718464447431	1.05514064333366\\
};
\label{pgf:realized-trajectories}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
